Iterative label cleaning for transductive and semi-supervised few-shot learning

Few-shot learning amounts to learning representations and acquiring knowledge such that novel tasks may be solved with both supervision and data being limited. Improved performance is possible by transductive inference, where the entire test set is available concurrently, and semi-supervised learning, where more unlabeled data is available. Focusing on these two settings, we introduce a new algorithm that leverages the manifold structure of the labeled and unlabeled data distribution to predict pseudo-labels, while balancing over classes and using the loss value distribution of a limited-capacity classifier to select the cleanest labels, iteratively improving the quality of pseudo-labels. Our solution surpasses or matches the state of the art results on four benchmark datasets, namely miniImageNet, tieredImageNet, CUB and CIFAR-FS, while being robust over feature space pre-processing and the quantity of available data. The publicly available source code can be found in https://github.com/MichalisLazarou/iLPC.

==> fig/hist/histbal.tex <==
\begin{tabular}{cc}
\small
\centering
\setlength\tabcolsep{0pt}

\extfig{histograms-before}
{
\begin{tikzpicture}
\begin{axis}[
	width=2\linewidth,
	height=0.5\linewidth,
	font=\small,
	ybar,
	xmin=-1,
	xmax=75,
	ymin=0,
	ymax = 1.5,
	%xlabel={query ID},
	ylabel={correct},
	yticklabels={,,},
	xtick style={draw=none},
	ytick style={draw=none},
	% xtick pos=bottom,
	% ytick pos=left,
	grid=none,
		bar/.style={thin,fill opacity=0.5,bar width=1},
]
\addplot[red, fill=red, bar] table[x=x,y=before] \labelhistograms; \leg{before}
%\addplot[blue,fill=blue,bar] table[x=x,y=uniform]  \labelhistograms; \leg{uniform}
%\addplot[green,fill=green,bar] table[x=x,y=entropy]  \labelhistograms; \leg{entropy}
\end{axis}
\end{tikzpicture}
}
& 
\\
\extfig{histograms-uniform}
{
\begin{tikzpicture}
\begin{axis}[
	width=2\linewidth,
	height=0.5\linewidth,
	font=\small,
	ybar,
	xmin=-1,
	xmax=75,
	ymin=0,
	ymax = 1.5,
	%xlabel={query ID},
	ylabel={correct},
	yticklabels={,,},
	xtick style={draw=none},
	ytick style={draw=none},
	% xtick pos=bottom,
		% ytick pos=left,
	grid=none,
	bar/.style={thin,fill opacity=0.5,bar width=1},
]
%\addplot[red, fill=red, bar] table[x=x,y=before] \labelhistograms; \leg{before}
\addplot[blue,fill=blue,bar] table[x=x,y=uniform]  \labelhistograms; \leg{uniform}
%\addplot[green,fill=green,bar] table[x=x,y=entropy]  \labelhistograms; \leg{entropy}


\end{axis}
\end{tikzpicture}
}
&
\\

\extfig{hist-entropy}
{
\begin{tikzpicture}
\begin{axis}[
	width=2\linewidth,
	height=0.5\linewidth,
	font=\small,
	ybar,
	xmin=-1,
	xmax=75,
	ymin=0,
	ymax = 1.5,
	xlabel={query ID},
	ylabel={correct},
	yticklabels={,,},
	xtick style={draw=none},
	% xtick pos=bottom,
	% ytick pos=left,
	grid=none,
	bar/.style={thin,fill opacity=0.5,bar width=1},
]
%\addplot[red, fill=red, bar] table[x=x,y=before] \labelhistograms; \leg{before}
%\addplot[blue,fill=blue,bar] table[x=x,y=uniform]  \labelhistograms; \leg{uniform}
\addplot[green,fill=green,bar] table[x=x,y=entropy]  \labelhistograms; \leg{entropy}


\end{axis}
\end{tikzpicture}
}
\end{tabular}

==> presentation/iccv/tfh/tfh.tex <==
%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Motivation}

\begin{itemize}
	\item What is few-shot learning?
\end{itemize}

\fig{why_fsl}


\end{frame}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Contributions}
\structure{Previous state of the art}
\begin{itemize}
	\item Meta-learning
	\item Transfer learning
	\item Domain adaptation
	\item Synthetic data generation
\end{itemize}
\uncover<2->{
\structure{Contributions}
\begin{itemize}
	\item  Novel algorithm that consists of three modules:
	\begin{itemize}
        \item Label propagation
        \item Class balancing
        \item Label cleaning
    \end{itemize}
\end{itemize}
}
\end{frame}
%------------------------------------------------------------------------------



%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Problem formulation and definitions}

\structure{Pre-training}
\begin{itemize}
    \item We use publicly available pre-trained networks from published works
	\item Base class dataset: $D_{\base} \defn \{(x_i, y_i)\}_{i=1}^I$ where $y_i \in C_{\base}$
	\item Embedding network $f_\theta: \cX \to \real^{d}$ is trained on $D_{\base}$
	%\item $\bar{f}_\theta: \cX \to \real^d$ denotes $f_\theta$ followed by global average pooling (GAP)
\end{itemize}

\vspace{1em}

\uncover<2->{
\structure{Inference stage}
\begin{itemize}
    \item We focus on transductive and semi-supervised few-shot learning
	\item Novel class dataset $D_{\novel}$ with $C_{\novel}$ disjoint from $C_{\base}$
	\item Assume access to $f_{\theta}$, a support set, $S$, a query set, $Q$ and in the semi-supervised setting also an unlabelled set, $U$

% 	\item Sample a support set $S$ and a query set $Q$ from $D_{\novel}$
% 	\item $S$ consists of $N$ classes with $K$ labeled examples per class
% 	\item In the transductive setting we assume access to the full query set, $Q$
% 	\item In the semi-supervised setting we do not have access to the query set, $Q$ but we have access to an unlabelled set $U$ consisting of the same classes
% 	\item Given $S$ and $f_\theta$, classify examples from $Q$
\end{itemize}
}

\end{frame}
%------------------------------------------------------------------------------


% \begin{frame}
% \frametitle{Problem formulation and definitions}

% \structure{Transductive few-shot learning}
% \begin{itemize}

%     \item Assume access to $f_{\theta}$, a support set,$S$ , and a query set, $Q$
%     \item $S$ consists of $N$ classes with $K$ labeled examples per class
%     \item Exploit $S$ and $Q$ to optimize accuracy predictions for $Q$
% \end{itemize}
% \uncover<2->{
% \structure{Inductive semi-supervised few-shot learning}
% \begin{itemize}

%     \item Assume access to $f_{theta}$, a support set,$S$ , an unlabelled set, $U$ but no access to the query set, $Q$
%     \item $S$ consists of $N$ classes with $K$ labeled examples per class
%     \item Exploit $S$ and $U$ to optimize accuracy predictions for $Q$
% \end{itemize}
% }

% \end{frame}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
% \begin{frame}
% \frametitle{Problem formulation and definitions}

% \structure{Representation learning}
% \begin{itemize}
% 	\item Base class data: $D_{\base} \defn \{(x_i, y_i)\}_{i=1}^I$ where $y_i \in C_{\base}$
% 	\item Train embedding network $f_\theta: \cX \to \real^{d \times h \times w}$ on $D_{\base}$
% 	\item $\bar{f}_\theta: \cX \to \real^d$ denotes $f_\theta$ followed by global average pooling (GAP)
% \end{itemize}

% \vspace{1em}

% \uncover<2->{
% \structure{Inference stage}
% \begin{itemize}
% 	\item Novel class data $D_{\novel}$ with $C_{\novel}$ disjoint from $C_{\base}$
% 	\item Sample a support set $S$ and a query set $Q$ from $D_{\novel}$
% 	\item $S$ consists of $N$ classes with $K$ labeled examples per class
% 	\item Given $S$ and $f_\theta$, classify examples from $Q$
% \end{itemize}
% }

% \end{frame}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
% \begin{frame}
% \frametitle{Representation learning}

% \begin{itemize}
% 	\item \alert{1st stage}: train the backbone network using standard cross-entropy
% 	\begin{equation*}
% 		L(D_{\base}; \theta, \phi) \defn
% 			\sum_{i=1}^I L_{\CE}(c_{\phi}(\bar{f}_\theta(x_i)), y_i) + R(\phi)
% 	\end{equation*}
% 	\item<2-> \alert{2nd stage}: adopt a self-distillation process
% 	\begin{equation*}
% 		L_{\KD}(D_{\base}; \theta', \phi') \defn
% 			\alpha L(D_{\base}; \theta', \phi') +
% 			\beta \KL(c_{\phi'}(\bar{f}_{\theta'}(x_i)), c_\phi(\bar{f}_{\theta}(x_i)))
% 	\end{equation*}
% \end{itemize}

% \end{frame}
%------------------------------------------------------------------------------


%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Iterative label cleaning: Nearest-neighbour graph}
%\fig{iLPC1}
\centering
\includegraphics[scale=1]{\pwd fig/ilpc1_theta.pdf}
% \begin{itemize}
% 	\item Meta-training stage: sample episodes of $S$ from $D_{\base}$
% 	\item Pre-trained network $f_\theta: \cX \to \real^{d \times h \times w}$ maps images to tensors
% 	\item \alert{Class prototype} tensors:
% 	\begin{equation*}
% 		p_j \defn \frac{1}{K} \sum_{i=1}^{K} f_{\theta'}(x_i^j)
% 	\end{equation*}
% 	\item<2-> \alert{Conditioner} $h$ maps prototypes to class-conditional vectors $s_j \defn h(p_j) \in \real^{d'}$
% 	\item<2-> \alert{Generator} maps to $g(z; s_j) \in \real^{d \times h \times w}$ where $z \sim \normal(\vzero,I_k)$
% 	\item<3-> Jointly trained by:
% 	\begin{equation*}
% 		L_{\hal}(X; h, g) = \frac{1}{MN} \sum_{j=1}^N \sum_{m=1}^M \norm{g(z_m; h(p_j)) - p_j}^2
% 	\end{equation*}

% \end{itemize}

\end{frame}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Iterative label cleaning: Label propagation}
%\fig{iLPC2}
\centering
\includegraphics[scale=1]{\pwd fig/iLPC2.pdf}

% \begin{itemize}
% 	\item Meta-training stage: sample episodes of $S$ from $D_{\base}$
% 	\item Pre-trained network $f_\theta: \cX \to \real^{d \times h \times w}$ maps images to tensors
% 	\item \alert{Class prototype} tensors:
% 	\begin{equation*}
% 		p_j \defn \frac{1}{K} \sum_{i=1}^{K} f_{\theta'}(x_i^j)
% 	\end{equation*}
% 	\item<2-> \alert{Conditioner} $h$ maps prototypes to class-conditional vectors $s_j \defn h(p_j) \in \real^{d'}$
% 	\item<2-> \alert{Generator} maps to $g(z; s_j) \in \real^{d \times h \times w}$ where $z \sim \normal(\vzero,I_k)$
% 	\item<3-> Jointly trained by:
% 	\begin{equation*}
% 		L_{\hal}(X; h, g) = \frac{1}{MN} \sum_{j=1}^N \sum_{m=1}^M \norm{g(z_m; h(p_j)) - p_j}^2
% 	\end{equation*}

% \end{itemize}

\end{frame}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Iterative label cleaning: Class balancing}
%\fig{iLPC3}
\centering
\includegraphics[scale=1]{\pwd fig/ilpc3.pdf}
% \begin{itemize}
% 	\item Meta-training stage: sample episodes of $S$ from $D_{\base}$
% 	\item Pre-trained network $f_\theta: \cX \to \real^{d \times h \times w}$ maps images to tensors
% 	\item \alert{Class prototype} tensors:
% 	\begin{equation*}
% 		p_j \defn \frac{1}{K} \sum_{i=1}^{K} f_{\theta'}(x_i^j)
% 	\end{equation*}
% 	\item<2-> \alert{Conditioner} $h$ maps prototypes to class-conditional vectors $s_j \defn h(p_j) \in \real^{d'}$
% 	\item<2-> \alert{Generator} maps to $g(z; s_j) \in \real^{d \times h \times w}$ where $z \sim \normal(\vzero,I_k)$
% 	\item<3-> Jointly trained by:
% 	\begin{equation*}
% 		L_{\hal}(X; h, g) = \frac{1}{MN} \sum_{j=1}^N \sum_{m=1}^M \norm{g(z_m; h(p_j)) - p_j}^2
% 	\end{equation*}

% \end{itemize}

\end{frame}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Iterative label cleaning: Label cleaning}
\centering
\includegraphics[scale=1]{\pwd fig/ilpc4.pdf}
%\fig{iLPC4}

% \begin{itemize}
% 	\item Meta-training stage: sample episodes of $S$ from $D_{\base}$
% 	\item Pre-trained network $f_\theta: \cX \to \real^{d \times h \times w}$ maps images to tensors
% 	\item \alert{Class prototype} tensors:
% 	\begin{equation*}
% 		p_j \defn \frac{1}{K} \sum_{i=1}^{K} f_{\theta'}(x_i^j)
% 	\end{equation*}
% 	\item<2-> \alert{Conditioner} $h$ maps prototypes to class-conditional vectors $s_j \defn h(p_j) \in \real^{d'}$
% 	\item<2-> \alert{Generator} maps to $g(z; s_j) \in \real^{d \times h \times w}$ where $z \sim \normal(\vzero,I_k)$
% 	\item<3-> Jointly trained by:
% 	\begin{equation*}
% 		L_{\hal}(X; h, g) = \frac{1}{MN} \sum_{j=1}^N \sum_{m=1}^M \norm{g(z_m; h(p_j)) - p_j}^2
% 	\end{equation*}

% \end{itemize}

\end{frame}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Iterative label cleaning: Iterative inference}
%\fig{iLPC5}
\centering
\includegraphics[scale=1]{\pwd fig/ilpc5.pdf}
%\begin{figure}[h]
%\centering
%\includegraphics[scale=1]{\pwd fig/iLPC5.pdf}
%\end{figure}
% \begin{itemize}
% 	\item Meta-training stage: sample episodes of $S$ from $D_{\base}$
% 	\item Pre-trained network $f_\theta: \cX \to \real^{d \times h \times w}$ maps images to tensors
% 	\item \alert{Class prototype} tensors:
% 	\begin{equation*}
% 		p_j \defn \frac{1}{K} \sum_{i=1}^{K} f_{\theta'}(x_i^j)
% 	\end{equation*}
% 	\item<2-> \alert{Conditioner} $h$ maps prototypes to class-conditional vectors $s_j \defn h(p_j) \in \real^{d'}$
% 	\item<2-> \alert{Generator} maps to $g(z; s_j) \in \real^{d \times h \times w}$ where $z \sim \normal(\vzero,I_k)$
% 	\item<3-> Jointly trained by:
% 	\begin{equation*}
% 		L_{\hal}(X; h, g) = \frac{1}{MN} \sum_{j=1}^N \sum_{m=1}^M \norm{g(z_m; h(p_j)) - p_j}^2
% 	\end{equation*}

% \end{itemize}

\end{frame}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
% \begin{frame}
% \frametitle{Meta-training tensor hallucinator}

% \begin{itemize}
% 	\item Meta-training stage: sample episodes of $S$ from $D_{\base}$
% 	\item Pre-trained network $f_\theta: \cX \to \real^{d \times h \times w}$ maps images to tensors
% 	\item \alert{Class prototype} tensors:
% 	\begin{equation*}
% 		p_j \defn \frac{1}{K} \sum_{i=1}^{K} f_{\theta'}(x_i^j)
% 	\end{equation*}
% 	\item<2-> \alert{Conditioner} $h$ maps prototypes to class-conditional vectors $s_j \defn h(p_j) \in \real^{d'}$
% 	\item<2-> \alert{Generator} maps to $g(z; s_j) \in \real^{d \times h \times w}$ where $z \sim \normal(\vzero,I_k)$
% 	\item<3-> Jointly trained by:
% 	\begin{equation*}
% 		L_{\hal}(X; h, g) = \frac{1}{MN} \sum_{j=1}^N \sum_{m=1}^M \norm{g(z_m; h(p_j)) - p_j}^2
% 	\end{equation*}

% \end{itemize}

% \end{frame}
%------------------------------------------------------------------------------

% %------------------------------------------------------------------------------
% \begin{frame}
% \frametitle{
% \only<1-3>{Tensor hallucinator: inference}
% \only<4>{Tensor hallucinator: inference}
% }

% \fig<1>[1]{hallucinator_slides1}%
% \fig<2>[1]{hallucinator_slides2}%
% \fig<3>[1]{hallucinator_slides3}%
% \fig<4>[1]{hallucinator_slides4}%

% \end{frame}
% %------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\renewcommand{\tb}[1]{\alert{\textbf{#1}}}
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Ablation Study}
\structure{Label propagation}
%\begin{figure}
%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{tabular}{lccccc}
\toprule
\Th{Inference}            & \mc{2}{\Th{ResNet-12A}}                   & \mc{2}{\Th{WRN-28-10}}                    \\
                        &1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
Inductive classifier        & 56.30\ci{0.62}      & \textbf{75.59}\ci{0.47}      & 68.17\ci{0.60}      & \textbf{84.33}\ci{0.43}      \\
\textbf{Label Propagation}         & \textbf{61.09}\ci{0.70}      & 75.32\ci{0.50}      & \textbf{74.24}\ci{0.68}      & 84.09\ci{0.42}      \\
\bottomrule
\end{tabular}
\vspace{6pt}
\end{table}
\begin{itemize}
    \item Exploit the manifold structure of the data
\end{itemize}
\end{frame}

%------------------------------------------------------------------------------

\begin{frame}
\frametitle{Ablation Study}
% \raggedright
% \uncover<2->{
\structure{Class balancing}
%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lccccc}
\toprule
\Th{Balancing} & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}                        \\
               &              & 1-shot              & 5-shot              & 1-shot              & 5-shot \\ \midrule
None           & WRN-28-10    & 78.06\ci{0.82}      & 87.80\ci{0.42}      & 86.04\ci{0.73}      & 90.74\ci{0.46}         \\
\textbf{True}      & WRN-28-10    & \textbf{82.68}\ci{0.82} & \textbf{89.07}\ci{0.41} & \textbf{89.17}\ci{0.70} & \textbf{92.67}\ci{0.44} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\end{table}
\begin{itemize}
    \item Incorporate prior information and search for a transport plan
\end{itemize}
%}



\end{frame}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\begin{frame}
\frametitle{Ablation Study}
\structure{Label cleaning}
%\begin{figure}
\begin{tabular}{cc}
    \centering
		\includegraphics[width=0.44\linewidth, height=0.30\linewidth]{\pwd fig/query-1.pdf}
		&
		\includegraphics[width=0.44\linewidth, height=0.30\linewidth]{\pwd fig/query-2.pdf} \\
\end{tabular}
\end{frame}

%\end{figure}
% \centering
% \includegraphics[width = 0.8\textwidth, height =0.3\textheight]{\pwd fig/cleaning_loss.png}

% \raggedright
% \uncover<2->{
\begin{frame}
\frametitle{Ablation Study}
\structure{Iterative procedure}
%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{tabular}{lccccc}
\toprule
\Th{Inference}          & \mc{2}{\Th{ResNet-12A}}                   & \mc{2}{\Th{WRN-28-10}}                    \\
                        &  1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
Non-iterative         & 65.04\ci{0.75}      & 76.82\ci{0.50}      & 79.42\ci{0.69}      & 85.34\ci{0.43}      \\
\textbf{iterative (\ours)}     & \textbf{69.79}\ci{0.99} & \textbf{79.82}\ci{0.55}      & \textbf{83.05}\ci{0.79} & \textbf{88.82}\ci{0.42} \\
\bottomrule
\end{tabular}
\vspace{6pt}
\end{table}

\begin{itemize}
    \item Iterative selection of the most likely correctly classified queries
\end{itemize}
%------------------------------------------------------------------------------
%}



\end{frame}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\begin{frame}[fragile]
\frametitle{Experimental results}


\structure{Transductive experiments}

%{
\small
\centering
\setlength\tabcolsep{4pt}
%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{tabular}{lccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}                         \\
                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot                               \\ \midrule
LR+ICI [63]   & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      \\
\textbf{\ours (ours)}       & ResNet-12A   & \textbf{69.79}\ci{0.99} & \textbf{79.82}\ci{0.55} & \textbf{83.49}\ci{0.88} & \textbf{89.48}\ci{0.47} \\ \midrule
PT+MAP [19]   & WRN-28-10    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40} \\
LR+ICI [63]   & WRN-28-10    & 80.61\ci{0.80}      & 87.93\ci{0.44}      & 86.79\ci{0.76}      & 91.73\ci{0.40} \\
\textbf{\ours (ours)}       & WRN-28-10    & \textbf{83.05}\ci{0.79} & \textbf{88.82}\ci{0.42} & \textbf{88.50}\ci{0.75} & \textbf{92.46}\ci{0.42}\\ \bottomrule
\end{tabular}
\vspace{6pt}
\label{tab:trans-pre}
\end{table}

\begin{itemize}
    \item State of the art results
\end{itemize}
\end{frame}
%------------------------------------------------------------------------------
%}
% \uncover<2->{
\begin{frame}[fragile]
\frametitle{Experimental results}
\structure{Transductive experiments with more unlabeled queries}
%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{lccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}                \\
                        &              & 1-shot              & 5-shot     & 1-shot              & 5-shot          \\ \midrule
LR+ICI [63]    & WRN-28-10    & 82.38\ci{0.86}      & 88.78\ci{0.39}      & 88.59\ci{0.74}      & 92.11\ci{0.39}     \\
PT+MAP [19]  & WRN-28-10    & 83.79\ci{0.71}      & 88.94\ci{0.33}      & 88.87\ci{0.64}      & 92.01\ci{0.36} \\
\textbf{\ours (ours)}       & WRN-28-10    & \textbf{85.98}\ci{0.74} & \textbf{90.54}\ci{0.31} & \textbf{90.02}\ci{0.70} &\textbf{92.94}\ci{0.37}\\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{6pt}
\end{table}
% }
\begin{itemize}
    \item The performance gap from the other methods increases significantly because our method exploits the manifold structure of the data
\end{itemize}
\end{frame}

\begin{frame}[fragile]
\frametitle{Experimental results}

\structure{Semi-supervised experiments}
%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{adjustbox}{width=1\textwidth}
\setlength\tabcolsep{4.5pt}
\begin{tabular}{lcccccc}
\toprule
\Th{Method}                    & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}} \\
                               &              &            & 1-shot              & 5-shot              & 1-shot              & 5-shot     \\ \midrule
LR+ICI [63]           & ResNet-12A   & 30/50      & 67.57\ci{0.97}      & 79.07\ci{0.56}      & 83.32\ci{0.87}      & 89.06\ci{0.51} \\
\textbf{\ours (ours)}              & ResNet-12A   & 30/50      & \textbf{70.99}\ci{0.91} & \textbf{81.06}\ci{0.49} & \textbf{85.04}\ci{0.79} & \textbf{89.63}\ci{0.47} \\ \midrule
LR+ICI [63]         & WRN-28-10    & 30/50      & 81.31\ci{0.84}      & 88.53\ci{0.43}      & 88.48\ci{0.67}      & 92.03\ci{0.43}         \\
PT+MAP [19] & WRN-28-10    & 30/50      & 83.14\ci{0.72}      & 88.95\ci{0.38}      & 89.16\ci{0.61}      & 92.30\ci{0.39}      \\
\textbf{\ours (ours)}             & WRN-28-10    & 30/50      & \textbf{83.58}\ci{0.79} & \textbf{89.68}\ci{0.37} & \textbf{89.35}\ci{0.68} & \textbf{92.61}\ci{0.39}   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{6pt}
\label{tab:semi_pre}
\end{table}
%------------------------------------------------------------------------------
\begin{itemize}
    \item State of the art results
\end{itemize}
\end{frame}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
% \begin{frame}
% \frametitle{Conclusion}

% \begin{itemize}
%     \item Proposed a novel algorithm based on three distinct modules effectively exploiting the use of available unlabeled data
%     \item Our algorithm achieves state-of-the-art results in four benchmark datasets
% \end{itemize}

% \end{frame}
%------------------------------------------------------------------------------



==> presentation/main/defn.tex <==
\newcommand{\base}{\mathrm{base}}
\newcommand{\novel}{\mathrm{novel}}
\newcommand{\CE}{\mathrm{CE}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\KD}{\mathrm{KD}}
\newcommand{\hal}{\mathrm{hal}}

\newcommand{\ours}{iLPC\xspace}
\newcommand{\lp}{LP\xspace}
\newcommand{\bal}{Balance\xspace}
\newcommand{\ilc}{iLC\xspace}
\newcommand{\cp}{Class\xspace}
\newcommand{\iprob}{iProb\xspace}
\newcommand{\pt}{PT\xspace}


==> presentation/main/defn_exp.tex <==
\newcommand{\ro}{$\mathcal{R}$Oxf}
\newcommand{\rp}{$\mathcal{R}$Par}
\newcommand{\roxf}{$\mathcal{R}$Oxford5k\xspace}
\newcommand{\rpar}{$\mathcal{R}$Paris6k\xspace}
\newcommand{\mln}{$\mathcal{R}$1M\xspace}

\newcommand{\dm}{+$\mathcal{R}$1M}

\newcommand{\vgg}{VGG16}
\newcommand{\res}{ResNet101}

\newcommand{\lcontrp}{Contr$^+$\xspace}
\newcommand{\lcontr}{Contr\xspace}
\newcommand{\ltripl}{Triplet\xspace}
\newcommand{\lms}{MS\xspace}
\newcommand{\lreg}{Reg\xspace}
\newcommand{\lrkd}{RKD\xspace}
\newcommand{\lrank}{DR\xspace}




==> presentation/main/tex/abbrev.tex <==
% symbol abbreviations

\newcommand{\eval}[1]{\the\numexpr#1\relax}
\newcommand{\head}[1]{{\smallskip\noindent\bf #1}}
\newcommand{\eq}[1]{(\ref{eq:#1})}

\newcommand{\Th}[1]{\textsc{#1}}
\newcommand{\mr}[2]{\multirow{#1}{*}{#2}}
\newcommand{\mc}[2]{\multicolumn{#1}{c}{#2}}
\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\al}[1]{\alert{#1}}

\newcommand<>{\white}  [2][100]{{\color#3  {white!#1}{#2}}}
\newcommand<>{\red}    [2][100]{{\color#3    {red!#1}{#2}}}
\newcommand<>{\blue}   [2][100]{{\color#3   {blue!#1}{#2}}}
\newcommand<>{\green}  [2][100]{{\color#3  {green!#1}{#2}}}
\newcommand<>{\cyan}   [2][100]{{\color#3   {cyan!#1}{#2}}}
\newcommand<>{\yellow} [2][100]{{\color#3 {yellow!#1}{#2}}}
\newcommand<>{\magenta}[2][100]{{\color#3{magenta!#1}{#2}}}
\newcommand<>{\orange} [2][100]{{\color#3 {orange!#1}{#2}}}
\newcommand<>{\gray}   [2][100]{{\color#3   {gray!#1}{#2}}}

\newcommand<>{\dwhite}  [2][100]{{\color#3  {white!#1!black}{#2}}}
\newcommand<>{\dred}    [2][100]{{\color#3    {red!#1!black}{#2}}}
\newcommand<>{\dblue}   [2][100]{{\color#3   {blue!#1!black}{#2}}}
\newcommand<>{\dgreen}  [2][100]{{\color#3  {green!#1!black}{#2}}}
\newcommand<>{\dcyan}   [2][100]{{\color#3   {cyan!#1!black}{#2}}}
\newcommand<>{\dyellow} [2][100]{{\color#3 {yellow!#1!black}{#2}}}
\newcommand<>{\dmagenta}[2][100]{{\color#3{magenta!#1!black}{#2}}}
\newcommand<>{\dorange} [2][100]{{\color#3 {orange!#1!black}{#2}}}
\newcommand<>{\dgray}   [2][100]{{\color#3   {gray!#1!black}{#2}}}

\newcommand{\tta}[1]{\texttt{\alert{#1}}}
\newcommand{\qu}[1]{\textrm{\textbf{\Large{\alert{#1}}}}}
\newcommand{\quot}[1]{\qu{``}\texttt{#1}\qu{''}}
\newcommand{\inde}[1]{\begin{itemize}\item[]{#1}\end{itemize}}

\newcommand{\refc}[1]{\gray{#1}}

%--------------------------------------------------------------------

\newcommand{\tran}{^\top}
\newcommand{\mtran}{^{-\top}}
\newcommand{\zcol}{\mathbf{0}}
\newcommand{\zrow}{\zcol\tran}
\newcommand{\ch}{\checkmark}

\newcommand{\ind}{\mathbbm{1}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\zahl}{\mathbb{Z}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\proj}{\mathbb{P}}
\newcommand{\prob}{\mathbf{Pr}}
\newcommand{\normal}{\mathcal{N}}

\newcommand{\mif}{\textrm{if }}
\newcommand{\other}{\textrm{otherwise}}
\newcommand{\minimize}{\textrm{minimize }}
\newcommand{\maximize}{\textrm{maximize }}
\newcommand{\st}{\textrm{subject to }}

\newcommand{\id}{\operatorname{id}}
\newcommand{\const}{\operatorname{const}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\var}{\operatorname{Var}}
\newcommand{\mean}{\operatorname{mean}}
\newcommand{\trace}{\operatorname{tr}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\vect}{\operatorname{vec}}
\newcommand{\cov}{\operatorname{cov}}

\newcommand{\defn}{\mathrel{:=}}
\newcommand{\peq}{\mathrel{+\!=}}
\newcommand{\meq}{\mathrel{-\!=}}

\newcommand{\floor}[1]{\left\lfloor{#1}\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil{#1}\right\rceil}
\newcommand{\inner}[1]{\left\langle{#1}\right\rangle}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\frob}[1]{\norm{#1}_F}
\newcommand{\card}[1]{\left|{#1}\right|\xspace}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\der}[3][]{\frac{d^{#1}#2}{d#3^{#1}}}
\newcommand{\pder}[3][]{\frac{\partial^{#1}{#2}}{\partial{#3^{#1}}}}
\newcommand{\dder}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}

\newcommand{\wb}[1]{\overline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}

\def\spsx{\hspace{1pt}}
\def\sps{\hspace{2pt}}
\def\spm{\hspace{5pt}}
\def\spl{\hspace{10pt}}
\def\splx{\hspace{20pt}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vd}{\mathbf{d}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vh}{\mathbf{h}}
\newcommand{\vi}{\mathbf{i}}
\newcommand{\vj}{\mathbf{j}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vm}{\mathbf{m}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vo}{\mathbf{o}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vr}{\mathbf{r}}
\newcommand{\vs}{\mathbf{s}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}

\newcommand{\vA}{\mathbf{A}}
\newcommand{\vB}{\mathbf{B}}
\newcommand{\vC}{\mathbf{C}}
\newcommand{\vD}{\mathbf{D}}
\newcommand{\vE}{\mathbf{E}}
\newcommand{\vF}{\mathbf{F}}
\newcommand{\vG}{\mathbf{G}}
\newcommand{\vH}{\mathbf{H}}
\newcommand{\vI}{\mathbf{I}}
\newcommand{\vJ}{\mathbf{J}}
\newcommand{\vK}{\mathbf{K}}
\newcommand{\vL}{\mathbf{L}}
\newcommand{\vM}{\mathbf{M}}
\newcommand{\vN}{\mathbf{N}}
\newcommand{\vO}{\mathbf{O}}
\newcommand{\vP}{\mathbf{P}}
\newcommand{\vQ}{\mathbf{Q}}
\newcommand{\vR}{\mathbf{R}}
\newcommand{\vS}{\mathbf{S}}
\newcommand{\vT}{\mathbf{T}}
\newcommand{\vU}{\mathbf{U}}
\newcommand{\vV}{\mathbf{V}}
\newcommand{\vW}{\mathbf{W}}
\newcommand{\vX}{\mathbf{X}}
\newcommand{\vY}{\mathbf{Y}}
\newcommand{\vZ}{\mathbf{Z}}

\newcommand{\vone}{\mathbf{1}}
\newcommand{\vzero}{\mathbf{0}}

\newcommand{\valpha}{{\boldsymbol{\alpha}}}
\newcommand{\vbeta}{{\boldsymbol{\beta}}}
\newcommand{\vgamma}{{\boldsymbol{\gamma}}}
\newcommand{\vdelta}{{\boldsymbol{\delta}}}
\newcommand{\vepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\vzeta}{{\boldsymbol{\zeta}}}
\newcommand{\veta}{{\boldsymbol{\eta}}}
\newcommand{\vtheta}{{\boldsymbol{\theta}}}
\newcommand{\viota}{{\boldsymbol{\iota}}}
\newcommand{\vkappa}{{\boldsymbol{\kappa}}}
\newcommand{\vlambda}{{\boldsymbol{\lambda}}}
\newcommand{\vmu}{{\boldsymbol{\mu}}}
\newcommand{\vnu}{{\boldsymbol{\nu}}}
\newcommand{\vxi}{{\boldsymbol{\xi}}}
\newcommand{\vomikron}{{\boldsymbol{\omikron}}}
\newcommand{\vpi}{{\boldsymbol{\pi}}}
\newcommand{\vrho}{{\boldsymbol{\rho}}}
\newcommand{\vsigma}{{\boldsymbol{\sigma}}}
\newcommand{\vtau}{{\boldsymbol{\tau}}}
\newcommand{\vupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\vphi}{{\boldsymbol{\phi}}}
\newcommand{\vchi}{{\boldsymbol{\chi}}}
\newcommand{\vpsi}{{\boldsymbol{\psi}}}
\newcommand{\vomega}{{\boldsymbol{\omega}}}

\newcommand{\vLambda}{{\boldsymbol{\Lambda}}}
\newcommand{\vSigma}{{\boldsymbol{\Sigma}}}

\newcommand{\rLambda}{\mathrm{\Lambda}}
\newcommand{\rSigma}{\mathrm{\Sigma}}

%--------------------------------------------------------------------
% big parentesis

\makeatletter
\newcommand{\vast}[1]{\bBigg@{#1}}
\makeatother

%--------------------------------------------------------------------------------
% column width

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%--------------------------------------------------------------------------------
% add a period to the end of an abbreviation unless there's one
% already, then \xspace

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace\xspace}
%
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\Vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


==> presentation/main/tex/beam.tex <==
% macros for beamer

% replaces "<spec>" by "spec"
\newcommand{\clearbrackets}[1]{\expandafter\inside#1}\def\inside<#1>{#1}

% extends an overlay specification to all modes
\newcommand{\extendspec}[1]{#1|handout:#1|article:#1}
\newcommand{\at}[1]{#1|handout:#1|article:#1}

% clears an overlay specification from "<spec>" to "spec" and then extends to all modes
\newcommand{\onspec}[1]{\extendspec{\clearbrackets{#1}}}

% shortcuts for \includegraphics
\newcommand<>{\figure}[2][1]{\includegraphics#3[width=#1\textwidth]{#2}}
\newcommand<>{\figureh}[2][1]{\includegraphics#3[height=#1\textheight]{#2}}

% shortcuts for \includegraphics
\newcommand<>{\graph}[2][]{\includegraphics#3[#1]{\pwd fig/#2}}
\newcommand<>{\fig}[2][1]{\figure#3[#1]{\pwd fig/#2}}
\newcommand<>{\figh}[2][1]{\figureh#3[#1]{\pwd fig/#2}}
\newcommand<>{\figon}[2][1]{\fig<\onspec{#3}>[#1]{#2}}
\newcommand<>{\fighon}[2][1]{\figh<\onspec{#3}>[#1]{#2}}

\newcommand<>{\vfig}[2][1]{\visible#3{\fig[#1]{#2}}}

% extend overlay specifications of \only, \onslide and \visible
\newcommand<>{\on}{\only<\onspec{#1}>}
\newcommand<>{\ons}{\onslide<\onspec{#1}>}
\newcommand<>{\vis}{\visible<\onspec{#1}>}

% set handout style
\newcommand{\handstyle}{
  \mode<handout>{
    \usepackage{pgfpages}
    \pgfpagesuselayout{2 on 1}[a4paper,border shrink=5mm]
  }
}

% shortcuts for TOC (main, parts, sections, subsections)
\newcommand{\toc}{
	\begin{frame}
		\frametitle{outline}
		\begin{columns}
			\begin{column}{.9\textwidth}
				\tableofcontents
% 				\tableofcontents[pausesections]
			\end{column}
		\end{columns}
	\end{frame}
}

\newcommand{\partnumber}{\Rmnum{\insertpartnumber}}
\newcommand{\partheading}{outline -- part \partnumber}

\newcommand{\pagepart}{\AtBeginPart{
	\begin{frame}
	\begin{center}
		{\Large\structure{part \partnumber}} \\[24pt]
		{\Huge\structure{\insertpart}}
	\end{center}
	\end{frame}
}}

\newcommand{\tocpart}{\AtBeginPart{
	\frame{\partpage}
	\begin{frame}
		\frametitle{\partheading}
		\tableofcontents[part=\insertpartnumber]
% 		\tableofcontents[part=\insertpartnumber,pausesections]
	\end{frame}
}}

\newcommand{\tocsecpart}{\tocsec[\partheading]}
\newcommand{\tocsec}[1][outline]{\AtBeginSection[]{
	\begin{frame}<beamer>
		\frametitle{#1}
		\tableofcontents[currentsection,currentsubsection]
	\end{frame}
}}

\newcommand{\tocsubpart}{\tocsub[\partheading]}
\newcommand{\tocsub}[1][outline]{\AtBeginSubsection[]{
	\begin{frame}<beamer>
		\frametitle{#1}
		\tableofcontents[currentsection,currentsubsection]
	\end{frame}
}}

% roman numerals
\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

% color boxes for biographies
\setbeamercolor{bioupper}{fg=purple!50!blue!60!black,bg=purple!30!blue!40!white}
\setbeamercolor{biolower}{bg=purple!30!blue!20!white}
\newenvironment{bio}[2]{
	\begin{beamerboxesrounded}[upper=bioupper,lower=biolower,width=\textwidth,shadow=true]{\structure{#1}}
		\begin{columns}
		\column{.3\textwidth} {#2}
		\column{.6\textwidth}
}{
		\end{columns}
	\end{beamerboxesrounded}
}

%--------------------------------------------------------------------

% section frame
\newcommand{\fsect}[2]{%
\begin{frame}\begin{center}
{\white{.}#2\white{.}}\\[2em]{\Huge \structure{#1}}
\end{center}\end{frame}
}

% section definition
\newcommand{\tsect}[3]{%
\section{#2}
\fsect{#2}{#3}
\use{#1}{#1}
}

% section with image
\newcommand{\isect}[4][.5]{\tsect{#3}{#4}{\figh[#1]{#2}\\[1em]}}

% plain section
\newcommand{\sect}[2]{\tsect{#1}{#2}{}}


==> presentation/main/tex/plots-ext.tex <==
\usepackage{tikzextern}
\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> presentation/main/tex/plots.tex <==
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,calc,matrix,fit,backgrounds,positioning,shapes.multipart,graphs,graphs.standard,shadows,mindmap,scopes,intersections,plotmarks,shapes.geometric}
% \usepackage{pgffor}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.9}

\usepackage{chapterfolder}  % finds relative paths in nested \input's
\newcommand{\use}[2]{\cffolderinput{#1}{#2}}
\newcommand{\pwd}{\cfcurrentfolder}

%-----------------------------------------------------------------------------
% tikz styles

\tikzstyle{every picture}+=[
	remember picture,
	every text node part/.style={align=center},
	every matrix/.append style={ampersand replacement=\&},
]
\tikzstyle{tight} = [inner sep=0pt,outer sep=0pt]
\tikzstyle{txt} = [inner sep=1pt,outer sep=0pt,anchor=base]
\tikzstyle{base} = [baseline,every node/.style={inner xsep=0pt,anchor=base}]
\tikzstyle{na} = [baseline=-.5ex]
\tikzstyle{lab} = [draw=none,fill=blue!10,anchor=base,font=\footnotesize]
\tikzstyle{label} = [baseline,every node/.style={lab}]
\tikzstyle{over} = [overlay,every path/.style={->,draw=red,thick},nodes={draw}]
\tikzstyle{semi} = [draw opacity=.5]
\tikzstyle{paper} = [fill=white]
\tikzstyle{help} = [gray]
\tikzstyle{high} = [blue!70]
\tikzstyle{op} = [draw,circle,tight]
\tikzstyle{dot} = [fill,draw,circle,inner sep=1pt,outer sep=0]
\tikzstyle{pt} = [fill,draw,circle,inner sep=1.5pt,outer sep=.2pt]
\tikzstyle{circ} = [draw,circle,thick,inner sep=1.5pt,outer sep=0]
\tikzstyle{ocirc} = [draw,circle,thick,inner sep=2pt,outer sep=0]
\tikzstyle{node} = [draw,circle,tight,minimum size=12pt,anchor=center]
\tikzstyle{box} = [draw,thick,rectangle,inner sep=6pt]
\tikzstyle{group} = [high,box,opacity=.5]
\tikzstyle{maths} = [matrix of math nodes]
\tikzstyle{rsep} = [row sep={#1,between origins}]
\tikzstyle{csep} = [column sep={#1,between origins}]
\tikzstyle{short} = [shorten >=#1,shorten <=#1]
\tikzstyle{dim1} = [fill opacity=.3,text opacity=1]
\tikzstyle{dim2} = [fill opacity=.5,text opacity=1]
\tikzstyle{dim3} = [fill opacity=.7,text opacity=1]
\tikzstyle{rectc} = [tight,transform shape]
\tikzstyle{rect} = [rectc,anchor=south west]

%--------------------------------------------------------------------
% style overlays

\newcommand<>{\son}[2]{\alt#3{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={}}}}
\newcommand<>{\sunc}[2]{\alt#3{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={#2,opacity=.3}}}}
\newcommand<>{\svis}[2]{\alt#3{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={#2,opacity=0}}}}
\newcommand<>{\salt}[3]{\alt#4{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={#3}}}}
\newcommand<>{\stemp}[4]{\temporal#5{\tikzset{#1/.style={#2}}}{\tikzset{#1/.style={#3}}}{\tikzset{#1/.style={#4}}}}

%--------------------------------------------------------------------

% layers
\pgfdeclarelayer{bg4}
\pgfdeclarelayer{bg3}
\pgfdeclarelayer{bg2}
\pgfdeclarelayer{bg1}
\pgfdeclarelayer{fg1}
\pgfdeclarelayer{fg2}
\pgfdeclarelayer{fg3}
\pgfdeclarelayer{fg4}
\pgfsetlayers{bg4,bg3,bg2,bg1,main,fg1,fg2,fg3,fg4}

%--------------------------------------------------------------------

% nested equation/text inside tikz picture, to provide a labeled node
\newcommand{\nequ}[3][]{\tikz[base]{\node[#1] (#2) {$\displaystyle {#3}$};}}
\newcommand{\ntext}[3][]{\tikz[base]{\node[#1] (#2) {{#3}};}}

% apply style #1 to given text #2
\newcommand{\style}[2][]{\tikz[base]{\node[#1]{#2};}}

%--------------------------------------------------------------------

% display physical-to-logical unit ratio (how many pt per 1 logical unit)
\makeatletter
\newcommand\displogical{{%
    \pgfmathparse{1000*\pgf@xx}%
    \pgfmathprintnumber{\pgfmathresult}%
}}
\makeatother

% convert physical units to logical (dimensionless)
\newcommand{\logical}[1]{scalar(#1/28.4527)}
\newcommand{\physical}[1]{#1*28.4527pt}

%-----------------------------------------------------------------------------
% tikz-assisted positioning

% position image as character
\newcommand{\tchar}[2]{%
	\tikz{%
		\node[minimum width=#1\textwidth](a){};
		\node[tight,overlay] at(a) {\fig[#1]{#2}};
	}%
}

% lower object #1 by dimension #2 - useful as a workaround to (manually)
% center objects vertically inside overprint
\newcommand{\low}[2][0pt]{\tikz{\node(a){};\node[below=#1 of a]{#2};}}

% shift given tikz paths #2 by #1
\newcommand{\off}[2][(0pt,0pt)]{\tikz{\node[tight](a){};{[shift={#1}]{#2}}}}

% footer - place text #2 styled as #1 at the bottom left corner of slide
\newcommand{\foot}[2][]{%
	\tikz[overlay]{%
		\node[shift={(2ex,2ex)},anchor=south west,tight,#1]
		at (current page.south west)
		{\begin{varwidth}{\textwidth}{#2}\end{varwidth}};
	}%
}

% citation as footer
\newcommand{\refs}[1]{\foot[black!70]{\tiny {#1}\par}}

% cross out a rectangle specified by two nodes at the corners
% e.g. mark two nodes like \ntext{topleft}{...} and \ntext{bottomright}{...},
% then \crossout{topleft}{bottomright}
\newcommand<>{\crossout}[3][]{
\begin{tikzpicture}[overlay]
	\node[fit=(#2)(#3)](box){};
	\draw#4[red,line width=3pt,#1]
		(box.south west)--(box.north east)
		(box.north west)--(box.south east);
\end{tikzpicture}
}

%-----------------------------------------------------------------------------
% pgfplots general options

\newcommand{\data}[1]{\pwd fig/#1.txt}
\newcommand{\tabread}[2]{\pgfplotstableread{\data{#1}}#2}

\newcommand{\leg}[1]{\addlegendentry{#1}}
\newcommand{\legtext}[1]{\addlegendimage{empty legend} \addlegendentry{#1}}

%-----------------------------------------------------------------------------
% pgfplots styles

\tikzset{every mark/.append style={solid}}
\pgfplotsset{%smooth,
	grid=both, width=\columnwidth, try min ticks=5,
% 	every axis x label/.style={at={(ticklabel cs:0.5)},anchor=north},
% 	every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=south},
	every axis/.append style={font=\scriptsize},
	every axis plot/.append style={thick,mark size=1.2,tension=0.18},
	legend cell align=left, legend style={fill opacity=0.8}
}

\pgfplotsset{
	dash/.style={mark=o,dashed,opacity=0.7},
	dott/.style={mark=o,dotted,opacity=0.7},
	notick/.style={xtick=\empty,ytick=\empty,ztick=\empty},
	notic/.style={xticklabels={,,},yticklabels={,,},zticklabels={,,}},
	noxtic/.style={xticklabels={,,}},
	noytic/.style={yticklabels={,,}},
	noztic/.style={zticklabels={,,}},
	nolim/.style={enlargelimits=false},
	noxlim/.style={enlarge x limits=false},
	noylim/.style={enlarge y limits=false},
	nozlim/.style={enlarge z limits=false},
	lim/.style={enlargelimits=true},
	xlim/.style={enlarge x limits=true},
	ylim/.style={enlarge y limits=true},
	zlim/.style={enlarge z limits=true},
	ulim/.style={enlargelimits=upper},
	uxlim/.style={enlarge x limits=upper},
	uylim/.style={enlarge y limits=upper},
	uzlim/.style={enlarge z limits=upper},
% 	stealth/.style={grid=none,hide axis=true}, % alignment breaks
	stealth/.style={notick,axis line style={opacity=0}},
	plain/.style={every axis plot/.append style={},nolim,grid=none},
	comb/.style={every axis plot/.append style={ycomb,mark=*},noxlim,uylim,grid=none},
	cent/.style={axis lines=center},
	graf/.style={axis x line=bottom, axis y line=left},
	scat/.style={scatter,only marks,point meta=explicit},
	xy/.style={
		every axis x label/.style={at={(ticklabel* cs:1)},anchor=west},
		every axis y label/.style={at={(ticklabel* cs:1)},anchor=south},
	},
	xyz/.style={
		every axis x label/.style={at={(ticklabel* cs:1)},anchor=west},
		every axis y label/.style={at={(ticklabel* cs:1)},anchor=west},
		every axis z label/.style={at={(ticklabel* cs:1)},anchor=south},
	},
	z-sort/.style={z buffer=sort,unbounded coords=jump},
}

\newcommand{\igiga}[1]{\thisrowno{#1}/1000000000}
\newcommand{\imega}[1]{\thisrowno{#1}/1000000}
\newcommand{\ikilo}[1]{\thisrowno{#1}/1000}
\newcommand{\iperc}[2]{\thisrowno{#1}/#2}
\newcommand{\imap}[1]{\thisrow{#1}*100}
\newcommand{\giga}[1]{\thisrow{#1}/1000000000}
\newcommand{\mega}[1]{\thisrow{#1}/1000000}
\newcommand{\kilo}[1]{\thisrow{#1}/1000}
\newcommand{\perc}[2]{\thisrow{#1}/#2}
\newcommand{\map}[1]{\thisrow{#1}*100}

%------------------------------------------------------------------------------
% https://tex.stackexchange.com/a/355579/38641
% to use e.g. as "only=<4>{/pgf/bar width=2.8}" in axis options
\tikzset{only/.code args={<#1>#2}{\only<#1>{\pgfkeysalso{#2}}}}

%------------------------------------------------------------------------------
% python plots and plain axes

\newcommand{\pypre}{\pwd fig/data/}
\newcommand{\python}[1]{python -c "%
import math, sys; import numpy as np; import scipy.linalg as la;%
#1 np.savetxt(sys.stdout, data)%
"}
\newcommand<>{\pyplot}[3][]%
{\only#4{\addplot[#1] shell[prefix=\pypre,id=#2,] {\python{#3}};}}
\newcommand<>{\pyplott}[3][]%
{\only#4{\addplot3[z-sort,#1] shell[prefix=\pypre,id=#2,] {\python{#3}};}}
\newcommand<>{\pyload}[3][]%
{\only#4{\addplot[#1] table[x index=0,y index=#2] {\pypre #3.out};}}
\newcommand<>{\pyloadp}[3][]%
{\only#4{\addplot+[#1] table[x index=0,y index=#2] {\pypre #3.out};}}
\newcommand<>{\pyloadt}[2][]%
{\only#3{\addplot3[z-sort,#1] table {\pypre #2.out};}}
\newcommand{\pysave}[2]{
	\begin{tikzpicture}[overlay,opacity=0]
	\begin{axis} \pyplot{#1}{#2} \end{axis}
	\end{tikzpicture}
}
\newenvironment<>{axes}[3][plain]{
	\begin{onlyenv}#4
	\begin{tikzpicture}
	\begin{axis}[width=#2\textwidth,height=#3\textwidth,#1]
}{
	\end{axis}
	\end{tikzpicture}
	\end{onlyenv}
}
\newenvironment<>{xaxes}[3][plain]{
	\begin{onlyenv}#4
	\begin{tikzpicture}
	\begin{semilogxaxis}[width=#2\textwidth,height=#3\textwidth,#1]
}{
	\end{semilogxaxis}
	\end{tikzpicture}
	\end{onlyenv}
}
\newenvironment<>{xyaxes}[3][plain]{
	\begin{onlyenv}#4
	\begin{tikzpicture}
	\begin{loglogaxis}[width=#2\textwidth,height=#3\textwidth,#1]
}{
	\end{loglogaxis}
	\end{tikzpicture}
	\end{onlyenv}
}

%------------------------------------------------------------------------------
% python external plots with matplotlib & pgf

% convert unit of measure, e.g. \unit{in}{.8\textwidth}
\makeatletter
\def\unit#1#2{\strip@pt\dimexpr #2*65536/\number\dimexpr 1#1}
\makeatother

\newcommand{\pygf}[3]{python -c "%
import math, sys; import numpy as np; import scipy.linalg as la; %
import matplotlib as mpl; mpl.use('pgf'); import matplotlib.pyplot as plt; %
mpl.rcParams.update({'font.family':'serif','font.size':8}); %
fig = plt.figure(figsize=#2); #3 fig.savefig('#1', dpi=500); %
"}

\newcommand<>{\pygfplot}[4]{
	\immediate\write18{\pygf{fig/pgf/#1.pgf}{(\unit{in}{#2},\unit{in}{#3})}{#4}}
	\only#5{\input{fig/pgf/#1.pgf}}
}

%--------------------------------------------------------------------
% 2d drawing

% 2d coordinates
\def\bx[#1,#2]{#1}
\def\by[#1,#2]{#2}
\def\dx[#1,#2]{#1,0}
\def\dy[#1,#2]{0,#2}

% node coordinate system
\newcommand{\ncs}[2]{%
($(#1.south west)!\bx[#2]!(#1.south east)!\by[#2]!($(#1.north west)!\bx[#2]!(#1.north east)$)$)%
}

% rectangle in node coordinate system
\newcommand<>{\nrect}[4][]{\path#5[#1] \ncs{#2}{#3} rectangle \ncs{#2}{#4};}

% draw centered rectangle by node
\newcommand{\rectn}[4]{%
	node[draw,rectc,minimum width=#3cm,minimum height=#4cm,#1](#2){}%
}

% draw image by node
\newcommand{\rectim}[2]{%
	node[rect] {\graph[width={\bx[#1]}cm,height={\by[#1]}cm]{#2}}%
}

% draw image by node, with label
\newcommand{\rectiml}[3]{%
	node[rect](#1) {\graph[width={\bx[#2]}cm,height={\by[#2]}cm]{#3}}%
}

%------------------------------------------------------------------------------
% 3d drawing

\pgfkeys{/tikz/.cd, aspect/.store in=\aspect, aspect=3}
\pgfkeys{/tikz/.cd, depth/.store in=\depth, depth=.15}
\pgfkeys{/tikz/.cd, stepx/.store in=\step, stepx=1}

\tikzstyle{geom} = [line join=bevel,aspect=3,depth=.15,z={(\depth*\aspect,\depth)}]
\tikzstyle{wire} = [geom,draw,thick]

% 3d coordinates
\def\cx[#1,#2,#3]{#1}
\def\cy[#1,#2,#3]{#2}
\def\cz[#1,#2,#3]{#3}
\def\ex[#1,#2,#3]{#1,0,0}
\def\ey[#1,#2,#3]{0,#2,0}
\def\ez[#1,#2,#3]{0,0,#3}

% ellipses
\newcommand{\xell}[4][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect]
	(0,0) ellipse [x radius={\bx[#3]cm},y radius={\by[#3]cm},rotate=#4];
}

% lines along x, y, or z
\newcommand{\zline}[3][]{%
\path[geom,#1] #2 -- +(\cx[#3],\cy[#3]);
}
\newcommand{\yline}[3][]{%
\path[geom,#1,shift={#2},xslant=\aspect]
	(0,0) -- +(\cx[#3],\depth*\cz[#3]);
}
\newcommand{\xline}[3][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect]
	(0,0) -- +(\aspect*\depth*\cz[#3],\cy[#3]);
}

% rectangles / grids along x, y, or z
\newcommand{\zrect}[3][]{%
\path[geom,#1] #2 rectangle +(\cx[#3],\cy[#3]);
}
\newcommand{\yrect}[3][]{%
\path[geom,#1,shift={#2},xslant=\aspect]
	(0,0) rectangle +(\cx[#3],\depth*\cz[#3]);
}
\newcommand{\xrect}[3][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect]
	(0,0) rectangle +(\aspect*\depth*\cz[#3],\cy[#3]);
}
\newcommand{\xgrid}[3][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect,xstep=\aspect*\depth*\step]
	(0,0) grid +(\aspect*\depth*\cz[#3],\cy[#3]);
}

% parallepiped
\newcommand{\para}[3][]{%
\zrect[#1]{(#2)}{#3}               % front
\yrect[#1]{($(#2)+(\ey[#3])$)}{#3}   % top
\xrect[#1]{($(#2)+(\ex[#3])$)}{#3}   % right
}

\newcommand<>{\xrectim}[4][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect]
	let \n0={\aspect*\depth*\cz[#3]} in
		(0,0) node[rect] {\graph#5[width={\n0}cm,height={\cy[#3]}cm]{#4}};
}
\newcommand<>{\paraim}[4][]{\uncover#5{%
\zrect[#1]{(#2)}{#3}                         % front
\yrect[#1]{($(#2)+(\ey[#3])$)}{#3}           % top
\xrectim#5[#1]{($(#2)+(\ex[#3])$)}{#3}{#4}   % right, image
\xrect[#1]{($(#2)+(\ex[#3])$)}{#3}           % right
}}

%------------------------------------------------------------------------------
% externalize

\usepgfplotslibrary{external}
% \tikzexternalize[prefix=fig/extern/]
\newcommand{\extfig}[2]{\tikzsetnextfilename{#1}{#2}}
\newcommand{\extdata}[1]{\input{#1}}


==> presentation/main/tex/slides.tex <==
\usetheme{default}
\useinnertheme{rounded}
%\definecolor{orng}{rgb}{1,.35,0}
\definecolor{blue}{rgb}{0,0,0.75}
\usecolortheme[named=blue]{structure}
\setbeamercolor{alerted text}{fg=blue}
\usefonttheme{structurebold}
\usefonttheme[onlymath]{serif}
\setbeamercovered{transparent}
\setbeamertemplate{frametitle}[default][center]
\setbeamertemplate{itemize items}[circle]
\setbeamersize{text margin left=10pt}
\setbeamersize{text margin right=10pt}

\setbeamertemplate{navigation symbols}{%
\insertslidenavigationsymbol
\insertframenavigationsymbol
\insertsectionnavigationsymbol
\insertdocnavigationsymbol
\insertbackfindforwardnavigationsymbol
\hspace{5pt}
\raisebox{2pt}{\insertframenumber/\inserttotalframenumber}
}

%--------------------------------------------------------------------
% FIGURES: CHOOSE ONE OPTION
%
% plots:     build standalone pdfs for figures, then use them
% plots-ext: use existing pds for figures
%
\input{../main/tex/plots}
%  \input{../main/tex/plots-ext}
%--------------------------------------------------------------------

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{array}
\usepackage{xspace}
\usepackage{booktabs}       % professional-quality tables
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{array}
\usepackage{setspace}
\usepackage{bbm}
\usepackage{varwidth}
\usepackage{multimedia}
\usepackage[]{animate}

\usepackage{enumitem}
\setlist[itemize]{label=\usebeamerfont*{itemize item}%
	\usebeamercolor[fg]{itemize item}%
	\usebeamertemplate{itemize item}%
}
\setlist[enumerate]{label=\protect\usebeamerfont*{enumerate item}%
	\protect\usebeamercolor[fg]{enumerate item}%
	\insertenumlabel%
}

%--------------------------------------------------------------------

\input{../main/tex/abbrev}    % standard abbreviations
\input{../main/tex/beam}      % macros for beamer


==> presentation/main/thanks.tex <==
%--------------------------------------------------------------------
\begin{frame}
\begin{center}

% \begin{figure}[h]
%     \centering
% \begin{tabular}{cc}
%     \centering
% 		\includegraphics[width=0.25\linewidth, height=0.15\linewidth]{slides/main/fig/inria.png}
% 		&
% 		\includegraphics[width=0.25\linewidth, height=0.15\linewidth]{slides/main/fig/Imperial_logo.jpg}
% \end{tabular}
% \end{figure}
\figh[.12]{Imperial_logo.jpg}% \\[3em]
\figh[.12]{inria.png} \\[3em]



{\Huge \structure{Thank you!}} \\[2em]

{
\url{https://github.com/MichalisLazarou} \\
\url{http://www.commsp.ee.ic.ac.uk/~tania/}\\
\url{https://avrithis.net}
}

\end{center}
\end{frame}

%--------------------------------------------------------------------


==> presentation/main/title.tex <==
% \subtitle{}
\author{Michalis Lazarou$^1$, Tania Stathaki$^1$ and Yannis Avrithis$^2$}
\institute{$^1$Imperial College London, $^2$Inria, Univ Rennes, CNRS, IRISA}
%\includegraphics[scale=1]{presentation/iccv/tfh/fig/iccv_blue.png}

\titlegraphic{\figureh[.1]{../main/fig/Imperial_logo.jpg} \figureh[.1]{../main/fig/inria.png}} %{../main/fig/Imperial_logo.jpg}}
%\titlegraphic{\figureh[.1]{../main/fig/Imperial_logo.jpg}}
\date{\structure{ICCV 2021} \\[6pt] Virtual, October 2021}


==> tex/algo.tex <==
\footnotesize
\algrenewcommand\algorithmicindent{0.5em}%
    \begin{algorithmic}[1]
        \Require Access to $\{D_{base}, D_{novel}\}$ 
        \State Pre-train feature extractor, $f_\theta$, on $D_{base}$
        \State Sample a support set, $S$, and a querry set, $Q$, from $D_{novel}$
        \State extract feature embeddings, $v_i = f_{\theta}(x_i)$ for all samples, $x_i\in S \cup Q$
        \State pre-processing feature embeddings
		\For {iterate until all querries  from $Q$ are predicted}
	    	\State Graph construction, define affinity matrix, $A$, as \ref{eq:affinity}
	    	\State $W \gets A + A\tran$ %\comment{symmetric affinity}
            \State $\cW \gets D^{-1/2} W D^{-1/2}$ %\comment{symmetrically normalized affinity}
            \State Label Propagation: $Z \gets$ solve~\eq{lp} with CG
	    	\State Predict pseudolabels for querries using sinkhorn-knopp algorithm 
		    \State Label cleaning, choose the most likely example with the lowest loss
		    \State Augment support set, $S$, with selected pseudolabels
	    	\EndFor
    \end{algorithmic}


==> tex/experiments-1.tex <==
\section{Experiments}
\label{sec:experiments}

%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
%------------------------------------------------------------------------------

% We evaluate and compare our proposed method with the state-of-the-art methods in trasnductive and semi-supervised few-shot learning on the four most commonly used databases, \emph{mini}ImageNet~\cite{ravilstm, matchingNets}, \emph{tiered}ImageNet~\cite{ssmeta}, \emph{cifar-FS} and \emph{CUB}. 

%------------------------------------------------------------------------------

\subsection{Datasets}
\label{sec:data}

\paragraph{\emph{mini}ImageNet}

This is a widely used few-shot image classification dataset~\cite{matchingNets, ravilstm}. It contains 100 randomly sampled classes from ImageNet~\cite{imagenet}. These 100 classes are split into 64 training (base) classes, 16 validation (novel) classes and 20 test (novel) classes. Each class contains 600 examples (images). We follow the commonly used split proposed in~\cite{ravilstm}. All images are resized to $84 \times 84$.

\paragraph{\emph{tiered}ImageNet}

This dataset is also sampled from the ImageNet~\cite{imagenet}. However, rather than randomly sampling classes as in \emph{mini}ImageNet, it follows a hierarchical structure where the sampled classes are partitioned into 34 categories, which are organized into 20 training, 6 validation and 8 test categories, containing 351, 97 and 160 classes, respectively. This hierarchical partitioning strategy ensures that the training classes are semantically distinct from the test classes, making it a more realistic few-shot classification problem. We follow the commonly used split proposed in~\cite{sslmeta}. Again, all images are resized to $84 \times 84$.

\paragraph{CUB}

This is a fine-grained classification dataset consisting of 200 classes, each corresponding to a bird species. We follow the split defined by~\cite{closerlook, fewshotCUB}, with 100 training, 50 validation and 50 test classes. In order to have fair comparisons with state-of-the-art methods, we compare with~\cite{pt_map} \emph{without using} bounding boxes and with~\cite{lrici} \emph{using} bounding boxes, as described in~\cite{fewshotCUBbounding}.

\alert{How about all other comparisons? Do we use boxes by default or not? Yes on ResNet12A, no on WRN.}

\paragraph{CIFAR-FS}

This dataset is derived from CIFAR-100~\cite{cifar100db}, consisting of 100 classes with 600 examples per class. We follow the split provided by~\cite{closerlook}, with 64 training, 16 validation and 20 test classes. In order to have fair comparisons with state-of-the-art methods, we compare with~\cite{pt_map} by using the original image resolution of $32 \times 32$ and with~\cite{lrici} by resizing images to $84 \times 84$.

\alert{The original CIFAR resolution is $32 \times 32$, so it should the $84 \times 84$ that is resized, right? How about all other comparisons? What resolution do we use by default? 84 on ResNet12A and 32 on WRN}

%------------------------------------------------------------------------------

\subsection{Setup}
\label{sec:setup}

\paragraph{Tasks}

We consider $N$-way, $K$-shot classification tasks with $N \defn 5$ randomly sampled novel classes and $K \in \{1, 5\}$ randomly selected examples per class for support set $S$, that is, $L \defn 5K$ examples in total. For the query set $Q$, we randomly sample $15$ additional examples per class, that is, $M \defn 75$ examples in total, which is the most common choice in transductive and semi-supervised few shot learning~\cite{tpn, learning2selftrain, transmatch}. 

% In the transductive setting we have access to the query samples while on the semi-supervised setting we do not, therefore the semi-supervised setting is an inductive inference procedure.

In the semi-supervised setting, the unlabeled set $U$ contains an additional number of randomly sampled examples per novel class. This number depends on $K$. We use two settings, namely 30/50 and 100/100, where the first number (30 or 100) refers to 1-shot and the second (50 or 100) to 5-shot. Again, these are the two most common choices in semi-supervised few shot learning~\cite{learning2selftrain,lrici,mct,ssmeta,transmatch}.

\alert{How many tasks? Evaluation measures? Mean accuracy/confidence interval?}

% We experiment with different number of unlabelled examples in order to compare fairly to the different state-of-the-art methods since different works use different numbers of unlabelled examples and show the robustness of our method in every possible setting. More specifically we use 30/100 for the 1-shot setting and 50/100 for the 5-shot setting since they are the most widely used configurations for semi-supervised few-shot experiments. 

\paragraph{Networks}

We use publicly available pre-trained backbone convolutional neural networks that are trained on the base-class training set. We experiment with two popular networks, namely, the residual network ResNet-12~\cite{tadam} and the wide residual network (WRN-28-10)~\cite{LEO}. We use different settings to provide completely fair comparisons with reproduced results of three state-of-the-art methods: LR+ICI~\cite{lrici}, PT+MAP~\cite{pt_map} and MCT~\cite{mct}. 

In particular, to compare with~\cite{lrici}, we use pre-trained weights of the ResNet-12 provided by~\cite{lrici}, which we call ResNet-12A, as well as official public code\footnote{\url{https://github.com/Yikai-Wang/ICI-FSL}} for testing. To compare with~\cite{pt_map}, we use pre-trained weights of a WRN-28-10 provided by~\cite{manifoldmixup}\footnote{\url{https://github.com/nupurkmr9/S2M2_fewshot}}, which are the same used by~\cite{pt_map}, as well as official public code\footnote{\url{https://github.com/yhu01/PT-MAP}} for testing. To compare with~\cite{mct}, we use official public code\footnote{\url{https://github.com/seongmin-kye/MCT}} to train from scratch another version of ResNet-12 used by~\cite{mct}, which we call ResNet-12B, as well as the same code for testing.

% In our work we used the publicly available pre-trained models from the state-of-the-Art methods in the transductive and semi-supervised few-shot learning setting.~\cite{lrici} provided their pre-trained weights of a 12-layer resnet while~\cite{pt_map} provided the pre-trained weights of a WRN-28-10 which are the pre-trained weights provided from~\cite{manifoldmixup}. \alert{We also trained the backbones of \cite{mct} from scratch, since the backbones were not publicly available, in order to obtain fair and unbiased comparisons between our method and \cite{mct}.}

%We use the training scheme proposed in~\cite{manifoldmixup} to train the wide residual networks (WRN-28-10). In~\cite{manifoldmixup} two variations of the training method are used consisting of two different self-supervised pretext tasks. The first pretext task involves the input image to be rotated by different angles and the  model is trained  to  predict  the  amount  of  rotation  applied  to the image. In the rotation pretext task the model is trained using a standard cross-entropy loss in a similar way to standard supervised learning problems. The second pretext task, named exemplar, focuses on  training the model to learn invariant features  invariant  to  a  wide  range  of  image transformations such as: translation, scaling, rotation, contrast  and  color  shifts by creating 4 copies of every image through the aforementioned random augmentations. In the exemplar pretext task, the model is trained using the triplet loss~\cite{tripletLoss} where the positive examples are the augmentations of the query image and the negative examples are all the other images. In our work we use the rotation pretext task and then we follow the training stage training for a few more epochs using  manifold mixup

\paragraph{Implementation details}

% In order to provide a fair comparison with different state-of-the-art methods we used the two most commonly used backbones, the 12-layer resnet~\cite{tadam} and the wide residual network (WRN-28-10)~\cite{LEO}. Since we would like to have fair comparisons with the best state-of-the-Art methods, we used the publicly available pre-trained models provided by~\cite{pt_map} and~\cite{lrici}.

Our implementation is based on PyTorch~\cite{pytorch} and FAISS~\cite{faiss}. The hyperparameters $\gamma$ and $k$ used in the nearest neighbor graph~\eq{affinity}, $\alpha$ used in label propagation~\eq{lp} and $\tau$ used in balancing~\eq{balance} are all optimized on the validation set of every dataset. \alert{We set $\tau=3$.}

\alert{
Ablation on hyperparameters (see section below).

PRE-PROCESSING? (On ResNet-12A,B and WRN). Ablation below.

Training details? Optimizer, learning rate and schedule, batch size etc. used in cleaning? 

Is $\vp$ used~\eq{sink-row},\eq{sink-col},\eq{loss} or just uniform? Ablation below.
}

%------------------------------------------------------------------------------

\subsection{Loss distribution of correct and mislabelled samples}
\label{sec:hist}

In order to verify the effectiveness of our label cleansing module we carried out the following experiments: a) for 500 correctly labelled images we apply different artificial label noise levels and apply our label cleaning module to observe whether it is possible to differentiate between the average loss of correct and mislabelled data. b) Rather than use artificial noise, given the few-shot transductive setting with $q=50$, we predict the labels of all unlabelled query samples and apply our label cleaning module to observe whether it is possible to differentiate between correct mislabelled predicted data. 

It can be clearly seen in \ref{fig:artificial_distr} that the correct and mislabelled samples have different loss distributions and our cleaning module can effectively uncover and exploit it. The robustness of our module is evident since even with different \% of artificial noise our cleaning module can detect and effectively distinguish between correct and mislabelled data. This is also evident on the more challenging case shown in \ref{fig:q_distr} where the mislabelled images are actually mislabelled query samples from labelled propagation. This is quiet profound since even though label propagation cannot classify correctly the samples are cleaning module can still detect robustly which samples are misclassified.

%------------------------------------------------------------------------------

%\begin{figure}
 %\centering
%\begin{tabular}{c}
%	 \fig[.95]{hist/artificial_noises} \\
%	 (a) \\
%	 \fig[.95]{hist/query_distr} \\
%	 (b) \\
%\end{tabular}
%\caption{Distribution of correctly classified and misclassified samples. (a) Artificial noise. (b) Query predictions.}
%\label{fig:hist}
%\end{figure}
%------------------------------------------------------------------------------
\begin{figure}
\vspace{-2pt}
\input{fig/hist/distributions}
\caption{
Distribution of correctly classified and misclassified with artificial noise.
\label{fig:artificial_distr}
}
\vspace{-3pt}
\end{figure}

%------------------------------------------------------------------------------
\begin{figure}
\vspace{-2pt}
\input{fig/hist/qdistr}
\caption{
Distribution of correctly classified and misclassified predicted queries.
\label{fig:q_distr}
}
\vspace{-3pt}
\end{figure}


%------------------------------------------------------------------------------

\subsection{Comparison using the pre-trained weights released from the state-of-the-Art methods}

In order to have objective comparisons between different methods, we believe that not only the experimental settings must be identical but also the backbone features, therefore  we decided to compare against the state-of-the-art method in transductive few-shot learning, \cite{pt_map} using their publicly available pre-trained WRN-28-10 networks. In order to compare the robustness of our algorithm using a different backbone we also compared against \cite{lrici} which is one of the state-of-the art methods in transductive few-shot learning using their pre-trained resNet-12 networks . %We decided to use the backbones of these two methods since they use different backbones, \cite{pt_map} uses WRN-28-10 while \cite{lrici} uses RESNET-12 which will allow us to show the robustness of our method through the use of different backbone architectures.
In table \ref{tab:trans_pre} it can be clearly observed that at best our method is clearly superior to both \cite{lrici} and \cite{pt_map} using their pre-trained networks while at worst it provides almost the same performance in the transductive setting. 

In order to compare the robustness of our method in different transductive experiments, using the same pre-trained WRN-28-10 backbones we experiment with using more unlabelled queries and using labelled support examples. We compare our method against \cite{pt_map} on 5-way, $k \in \{1, 5\}$-shot setting using more unlabelled queries $q=50$. The superiority of our algorithm is evident as it can be clearly seen in table \ref{tab:50q}. Leveraging the underlying manifold structure of the unlabelled data queries our method can improve its performance much more in comparison to \cite{pt_map}. This is evident since using only $q=15$, our method outperformed \cite{pt_map} on average on all dataset by $0.45\%$ while using $q=15$ the difference in performance accuracy is increased to $1.02\%$ with this being more evident on the 1-shot setting. Furthermore, we investigate the two methods under the setting of more available support examples under the 10-shot setting. Evidently from table \ref{tab:10shot} our method outperforms \cite{pt_map} on all 4 datasets.

As a last robustnest test, we compare the two methods by a robustness ablation study, removing the pre-processing part and removing the balancing with the raised exponent $\tau$.

\begin{table*}
\small
\centering
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}             & \Th{Backbone} & \mc{2}{\Th{\emph{mini}Imagenet}}          & \mc{2}{\Th{\emph{tiered}Imagenet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                        &               & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
LR+ICI~\cite{lrici}     & ResNet-12a    & 66.80\cip           & 79.26\cip           & 80.79\cip           & 87.92\cip           & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
LR+ICI~\cite{lrici}*    & ResNet-12a    & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
\textbf{LCLP (ours)}                      & ResNet-12a &\tb{69.79}\ci{0.99} &\tb{79.58}\ci{0.55} &\tb{83.49}\ci{0.88} &\tb{89.48}\ci{0.47} &\tb{77.14}\ci{0.95} &\tb{85.23}\ci{0.55} &\textbf{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\ \midrule
PT+MAP~\cite{pt_map}    & WRN-28-10     & 82.92\ci{0.00}      & 88.82\ci{0.00}      & -                   & -                   & 87.69\ci{0.00}      & 90.68\ci{0.00}      & 91.55\ci{0.00}      & 93.99\ci{0.00}      \\
PT+MAP~\cite{pt_map}*   & WRN-28-10     & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
\tb{LCLP (ours)}        & WRN-28-10     & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.00} & \tb{88.50}\ci{0.00} & \tb{92.99}\ci{0.00} & 87.55\ci{0.00}      & \tb{91.26}\ci{0.00} & 91.34\ci{0.00}      & \tb{94.27}\ci{0.30} \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive Few-shot learning methods comparison with same pre-trained backbones. * represents our re-implementation based on the original code and our datasets}
\label{tab:trans_pre}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\multicolumn{1}{c}{\Th{Method}} & \multicolumn{1}{c}{\Th{Backbone}}&\multicolumn{2}{c}{\Th{\emph{mini}Imagenet}} &  \multicolumn{2}{c}{\Th{\emph{tiered}Imagenet}} & \multicolumn{2}{c}{\Th{Cifar-FS}}\\ 
                            &           & 1-shot                & 5-shot                & 1-shot                & 5-shot                & 1-shot                & 5-shot     \\ \midrule
PT+MAP~\cite{pt_map}*       & WRN-28-10 & 83.79\ci{0.71}        & 88.94\ci{0.33}        & 88.87\ci{0.64}        & 92.01\ci{0.36}        & 87.63\ci{0.66}        & 90.15\ci{0.46}      \\
\textbf{LCLP (ours)}        & WRN-28-10 & \tb{86.30}\ci{0.71}   & \tb{89.99}\ci{0.32}   & \tb{90.60}\ci{0.64}   &\tb{92.97}\ci{0.38}    & \tb{88.51}\ci{0.69}   & \tb{91.23}\ci{0.44} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\label{tab:50q}
\caption{Transductive Few-shot 50-queries comparison}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccc}
\toprule
\Th{Method} & \Th{Backbone}&\Th{\emph{mini}Imagenet} &  \Th{\emph{tiered}ImageNet} & \Th{Cifar-FS} & \Th{CUB}    \\ 
                        &           & 10-shot               & 10-shot               & 10-shot               & 10-shot        \\ \midrule
PT+MAP~\cite{pt_map}*   & WRN-28-10 & 89.97\ci{0.34}        & 93.33\ci{0.34}        & 91.30\ci{0.45}        & 94.24\ci{0.28}          \\
\textbf{LCLP (ours)}    & WRN-28-10 & \tb{90.51}\ci{0.35}   & \tb{93.61}\ci{0.38}   & \tb{91.59}\ci{0.44}   & \tb{94.75}\ci{0.26} \\ \bottomrule
\end{tabular}
\caption{Transductive Few-shot 10-shot comparison}
\label{tab:10shot}
\end{table*}

%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{c}{\Th{Method}} & \multicolumn{1}{c}{\Th{Backbone}}&\multicolumn{2}{c}{\Th{\emph{mini}Imagenet}} &  \multicolumn{2}{c}{\Th{\emph{tiered}Imagenet}} \\\midrule 
                           &            & 1-shot    & 5-shot     & 1-shot & 5-shot     \\ \midrule
MCT(instance)~\cite{mct}   & ResNet-12b & 78.55\ci{0.86}        & 86.03\ci{0.42}        & 82.32\ci{0.81}        & 87.36\ci{0.50}          \\
MCT(instance)~\cite{mct}*  & ResNet-12b & 77.10\ci{0.88}        & 86.19\ci{0.40}        & -                     & -          \\
\textbf{LCLP (ours)}       & ResNet-12b &\textbf{-}             & \textbf{-}            & -                     & \textbf{-} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transducive few-shot learning comparison with MCT ~\cite{mct} and its network}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\Th{Method} & \mc{3}{\Th{Components}}    & \mc{2}{\emph{mini}Imagenet}  & \mc{2}{\emph{tiered}Imagenet}  \\ 
                & PT    & Norm.     & Center        & 1-shot            & 5-shot            & 1-shot        & 5-shot    \\ \midrule
PT+MAP          & -     & -         & -             & 48.57\ci{0.81}    & 75.67\ci{0.82}     & 49.67\ci{0.77} & 88.32\ci{0.50}          \\ 
LCLP(ours)      &  -     & -         & -             & -          & -    &       &      \\ \midrule
PT+MAP          & \ch     & -         & -             & 44.13\ci{0.56}    & 80.58\ci{0.44}     & 21.84\ci{0.58} & 78.81\ci{1.43}          \\ 
LCLP(ours)      & \ch     & -         & -             & -          & -    &       &      \\ \midrule
PT+MAP          & \ch     & \ch         & -             & 73.41\ci{0.64}    & 84.86\ci{0.42}     & 83.88\ci{0.69} & 90.48\ci{0.42}          \\ 
LCLP(ours)      & \ch      & \ch         &              & -          & -    &       &      \\ \midrule
PT+MAP          &\ch     &         & \ch            & 80.60\ci{0.81}          & 87.42\ci{0.43}    &   86.50\ci{0.77}    &  91.11\ci{0.46}          \\ 
LCLP(ours)      &\ch       &          & \ch             & -         & -    &   -   &      \\ \midrule
\end{tabular}

\vspace{6pt}
\caption{Robustness comparison our method against \cite{pt_map} for WRN-28-10 on \emph{mini}Imagenet and \emph{tiered}Imagenet}
\label{tab:ab-comp}
\end{table*}
%------------------------------------------------------------------------------




%------------------------------------------------------------------------------
%\begin{table*}
%\small
%\centering
%\begin{tabular}{lccccccccc}
%\toprule
%\multicolumn{1}{c}{\Th{Method}} & \multicolumn{1}{c}{\Th{Backbone}}&\multicolumn{2}{c}{\Th{\emph{mini}Imagenet}} &  \multicolumn{2}{c}{\Th{\emph{tiered}Imagenet}} & \multicolumn{2}{c}{\Th{Cifar-FS}} & \multicolumn{2}{c}{\Th{CUB}}    \\ 
  %                                       &           & 1-shot           & 5-shot            & 1-shot            & 5-shot            & 1-shot            & 5-shot            & 1-shot            & 5-shot     \\ \midrule
%PT+MAP (no-pre)~\cite{pt_map}*           & WRN-28-10 & 48.57\ci{0.81}   & 75.67\ci{0.82}    & 49.67\ci{0.77}    & 88.32\ci{0.50}    & 20.16\ci{0.04}    & 20.77\ci{0.08}    & 62.99\ci{1.23}    & 85.94\ci{0.85}      \\
%\textbf{LCLP (ours, no-pre)}                     & WRN-28-10 & \tb{-}           & \tb{-}            & -                 & \tb{-}            & \tb{-}            & \tb{-}            & -                 & \tb{-} \\ \midrule
%PT+MAP (no-sink)~\cite{pt_map}*          & WRN-28-10 & 81.12\ci{0.71}   & 87.66\ci{0.40}    & 87.62\ci{0.64}    & 91.27\ci{0.40}    & 85.28\ci{0.71}    & 89.34\ci{0.47}    & 89.89\ci{0.60}    & 92.55\ci{0.31}      \\
%\textbf{LCLP (ours)}                     & WRN-28-10 &\tb{-}            & \tb{-}            & -                 & \tb{-}            & \tb{-}            & \tb{-}            & -                 & \tb{-} \\ \midrule
%PT+MAP (no-sink/no-$\tau$)~\cite{pt_map}*  & WRN-28-10 &70.09\ci{0.61}    & 83.89\ci{0.41}    & 78.48\ci{0.63}    & 89.25\ci{0.42}    & 77.27+0.63        & 87.68\ci{0.48}    & 82.97\ci{0.59}    & 91.45\ci{0.35}      \\
%\textbf{LCLP (ours, no-bal/no-$\tau$)}                     & WRN-28-10 & \tb{-}           & \tb{-}            & -                 & \tb{-}            & \tb{-}            & \tb{-}            & -                 & \tb{-} \\
%\bottomrule
%\end{tabular}
%\vspace{6pt}
%\caption{Ablation on robustness of our algorithm in comparison to the best state-of-the-Art method}
%\end{table*}
%------------------------------------------------------------------------------

\begin{table*}
\small
\centering
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\Th{Method}}  & \multicolumn{1}{c}{\Th{Backbone}}&\multicolumn{1}{c}{\Th{unlabelled}} &\multicolumn{2}{c}{\Th{\emph{mini}Imagenet}}             &  \multicolumn{2}{c}{\Th{\emph{tiered}Imagenet}} & \multicolumn{2}{c}{\Th{Cifar-FS}} &\multicolumn{2}{c}{\Th{CUB}}\\ 
                     &           & split & 1-shot               & 5-shot                & 1-shot            & 5-shot            & 1-shot            & 5-shot                & 1-shot                & 5-shot \\ \midrule
LR+ICI~\cite{lrici}  & ResNet-12 & 30/50 & 69.66                & 80.11                 & 84.01             & 89.00             & 76.51             & 84.32                 & 89.58                 & 92.48  \\
LR+ICI~\cite{lrici}* & ResNet-12 & 30/50 & 67.64\ci{0.95}       & 80.00\ci{0.55}        & 83.20\ci{0.89}    & 89.15\ci{0.48}    & 76.57\ci{0.96}    & 84.11\ci{0.60}        & 88.36\ci{0.71}        & -      \\
\textbf{LCLP (ours)} & ResNet-12 & 30/50 &\tb{70.67}\ci{0.98}   & \tb{81.48}\ci{0.53}   & 83.49\ci{0.80}    & 88.65\ci{0.45}    & 76.46\ci{0.88}               & \tb{85.06}\ci{0.56}   & \tb{89.92}\ci{0.63}   & -      \\ 
\textbf{LCLP (ours)$\dagger$} & ResNet-12 & 30/50 & -   & -   & \tb{84.34}\ci{0.77}    & \tb{89.66}\ci{0.49}    & -               & -   & -   & -      \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised inductive few-shot learning methods comparison with same pre-trained backbones. * represents our re-implementation based on the original code and our datasets, $\dagger$ represents unormalized features}
\end{table*}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
%\input{fig/hist/exp}
\subsection{Ablation study}
\label{sec:ablation}



%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lcccccccc}
\toprule
\Th{Inference} & \mc{4}{\Th{Components}}    & \mc{2}{\Th{ResNet-12}}  & \mc{2}{\Th{WRN-28-10}}  \\ 
               & \lp & \bal & \iprob & \ilc & 1-shot     & 5-shot     & 1-shot     & 5-shot     \\ \midrule
Inductive      & -   & -    & -      & -    & -          & -          & -          & -          \\ 
Transductive   & \ch & -    & -      & -    & -          & -          & 74.35\ci{0.68}      & 84.84      \\ 
Transductive   & \ch & \ch  & -      & -    & -          & -          & 79.21\ci{0.72}      & 88.00\ci{0.41}      \\ 
Transductive   & \ch & \ch  & \ch    & -    & -          & -          & 72.28\ci{0.90}      & 85.88\ci{0.46}      \\ 
Transductive   & \ch & \ch  & -      & \ch  & \tb{69.79} & \tb{79.58} & \tb{83.43} & \tb{89.10} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Ablation study of each component of our method for WRN-28-10 and ResNet-12 backbones on \emph{mini}Imagenet.}
\label{tab:ab-comp2}
\end{table*}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------

\subsection{Comparison with Inductive Semi-Supervised Few-shot learning State-of-the-Art methods}

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{\Th{Method}} & \multicolumn{1}{c}{\Th{Backbone}} &\multicolumn{1}{c}{\Th{unlabelled}} &  \multicolumn{2}{c}{\Th{\emph{mini}Imagenet}}  & \multicolumn{2}{c}{\Th{\emph{tiered}Imagenet}}   \\ 
                                        &           & split  & 1-shot & 5-shot  & 1-shot & 5-shot \\ \midrule
%TPN$_{SSL}$\cite{tpn}                  & CONV-4    &20/20   & 52.78            & 66.42                 & 55.74             & 71.01  \\
%k-means$_{masked, soft}$~\cite{ssmeta} & CONV-4    &20/20   & 50.41            & 64.39                 & -                 & -      \\
%\textbf{LCLP (ours)}                   & CONV-4    &20/20   &                  &                       &                   &        \\ \midrule
LST~\cite{learning2selftrain}           & ResNet-12 &30/50   & 70.10\ci{1.90}   & 78.70\ci{0.80}        & 77.70\ci{1.60}    & 85.20\ci{0.80} \\
LR+ICI~\cite{lrici}                     & ResNet-12 &30/50   & 69.66            & 80.11                 & 84.01             & 89.00  \\
MCT (instance)~\cite{mct}               & ResNet-12 &30/50   & 73.80\ci{0.70}   & 84.40\ci{0.50}        & 76.90\ci{0.70}    & 86.30\ci{0.50}   \\
\textbf{LCLP (ours)}                    & ResNet-12 &30/50   &                  &                       &                   &        \\ \midrule
%LR+ICI~\cite{lrici}                    & ResNet-12 &80/80   & 71.41            & 81.12                 & 85.44             & 89.12  \\
%\textbf{LCLP (ours)}                   & ResNet-12 &80/80   &                  &                       &                   &        \\ \midrule
*k-means$_{masked, soft}$~\cite{ssmeta} & WRN-28-10 &100/100 & 52.35\ci{0.89}   & 67.67\ci{0.65}        & -                 & -      \\
TransMatch~\cite{transmatch}            & WRN-28-10 &100/100 & 63.02\ci{1.07}   & 81.06\ci{0.59}        & -                 & -      \\
\textbf{LCLP (ours)}                    & WRN-28-10 &100/100 &                  & \tb{87.73}\ci{0.37}   &                   &        \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised inductive few-shot learning methods comparison. *Re-implemented~\cite{transmatch}}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{c}{\Th{Method}} & \multicolumn{1}{c}{\Th{Backbone}}&\multicolumn{2}{c}{\Th{\emph{mini}Imagenet}} &  \multicolumn{2}{c}{\Th{\emph{tiered}Imagenet}} & \multicolumn{2}{c}{\Th{Cifar-FS}} & \multicolumn{2}{c}{\Th{CUB}}    \\ 
                                          &           & 1-shot        & 5-shot        & 1-shot        & 5-shot        & 1-shot        & 5-shot        & 1-shot        & 5-shot         \\\midrule
LR+ICI~\cite{lrici}                       & ResNet-12 & 66.80         & 79.26         & 80.79         & 87.92         & 73.97         & 84.13         & 88.06         & 92.53          \\
LR+ICI~\cite{lrici}*                      & ResNet-12 & 66.85\ci{0.92}         & 78.89\ci{0.55}         & 82.40\ci{0.84}         & 88.80\ci{0.50}         & 75.36\ci{0.97}         & 84.57\ci{0.57}         & 86.53\ci{0.79}         & 92.11\ci{0.35}          \\
CAN+Top-\emph{k}~\cite{crossattention}  & ResNet-12 & 67.19\ci{0.55}         & 80.64\ci{0.35}         & 73.21\ci{0.58}         & 84.93 \ci{0.38}        & -             & -             & -             & -              \\
DPGN~\cite{DPGN}                          & ResNet-12 & 67.77\ci{0.32}         & 84.60\ci{0.43}         & 72.45\ci{0.51}         & 87.24\ci{0.39}         & 77.90\ci{0.50}         & 90.20\ci{0.40}         & 75.71\ci{0.47}             & 91.48\ci{0.33}              \\
EP~\cite{embeddingpropagation}            & ResNet-12 & 66.50\ci{0.89}         & 81.06\ci{0.60}         & 76.53\ci{0.87}         & 87.32\ci{0.64}         & -             & -             & -             & -              \\
MCT(Instance)~\cite{mct}                  & ResNet-12 & 78.55\ci{0.86}         & 86.03\ci{0.42}         & 82.32\ci{0.81}         & 87.36\ci{0.50}         & 85.61\ci{0.69}         & 90.03\ci{0.46}         & -             & -              \\
MCT(Pair)~\cite{mct}                    & ResNet-12 & 76.16\ci{0.89}         & 85.22\ci{0.42}         & 80.68\ci{0.89}         & 86.63\ci{0.89}         & 87.28\ci{0.70}         & 90.50\ci{0.43}         & -             & -              \\
\textbf{LCLP (ours)}                      & ResNet-12 &\tb{69.79}\ci{0.99} &\tb{79.58}\ci{0.55} &\tb{83.49}\ci{0.88} &\tb{89.48}\ci{0.47} &\tb{77.14}\ci{0.95} &\tb{85.23}\ci{0.55} &\textbf{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\ \midrule
PT+MAP~\cite{pt_map}                      & WRN-28-10 & 82.92\ci{0.26}         & 88.82\ci{0.13}         &    -          & -             & 87.69\ci{0.23}        &90.68\ci{0.15}          &91.55\ci{0.19}          & 93.99\ci{0.10}          \\
PT+MAP~\cite{pt_map}*                     & WRN-28-10 & 82.88\ci{0.73}         & 88.78\ci{0.40}         & 88.15\ci{0.71}         & 92.32\ci{0.40}         & 86.91\ci{0.72}         &90.50\ci{0.49}          &91.37\ci{0.61}          & 93.93\ci{0.32}          \\
Fine-tuning~\cite{baseline_ft}            & WRN-28-10 & 65.73\ci{0.68}         & 78.40\ci{0.52}         & 73.34\ci{0.71}         & 85.50\ci{0.50}         & 76.58\ci{0.68}         & 85.79\ci{0.50}         & -             & -              \\
EP~\cite{embeddingpropagation}            & WRN-28-10 & 70.74\ci{0.85}         & 84.34\ci{0.53}         & 78.50\ci{0.91}         & 88.36\ci{0.57}         & -             & -             & -             & -              \\
SIB~\cite{SIB}                            & WRN-28-10 & 70.00\ci{0.60}          & 79.20\ci{0.40}          & 72.90$\dagger$ & 82.80$\dagger$ & 80.00\ci{0.60}          & 85.3\ci{0.40}          & -             & -              \\
DPGN~\cite{DPGN}                          & WRN-28-10 & 67.24\ci{0.51}         & 83.72\ci{0.44}         & -             & -             & -             & -             & -             & -              \\
SIB+E$^3$BM~\cite{ensemblefsl}            & WRN-28-10 & 71.40\ci{0.50}          & 81.20\ci{0.4}          & 75.60\ci{0.6}          & 84.30\ci{0.4}          & -             & -             & -             & -              \\
\textbf{LCLP (ours)}                      & WRN-28-10 &\tb{83.43} &\tb{89.10} & \tb{88.50}         &\tb{92.99} &\tb{87.55} &\tb{91.26} &91.34          &\tb{94.27}  \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive few-shot learning methods comparison with all state-of-the-Art. * represents our re-implementation based on the original code and our datasets, $\dagger$ implementation carried out by \cite{ensemblefsl}}
\end{table*}
%------------------------------------------------------------------------------

==> tex/experiments-2.tex <==
\section{Experiments}
\label{sec:experiments}

%------------------------------------------------------------------------------
\extdata{fig/data/sample}
%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
%------------------------------------------------------------------------------

% We evaluate and compare our proposed method with the state-of-the-art methods in trasnductive and semi-supervised few-shot learning on the four most commonly used databases, \emph{mini}ImageNet~\cite{ravilstm, matchingNets}, \emph{tiered}ImageNet~\cite{ssmeta}, \emph{cifar-FS} and \emph{CUB}. 

%------------------------------------------------------------------------------

\subsection{Datasets}
\label{sec:data}

\paragraph{\emph{mini}ImageNet}

This is a widely used few-shot image classification dataset~\cite{matchingNets, ravilstm}. It contains 100 randomly sampled classes from ImageNet~\cite{imagenet}. These 100 classes are split into 64 training (base) classes, 16 validation (novel) classes and 20 test (novel) classes. Each class contains 600 examples (images). We follow the commonly used split proposed in~\cite{ravilstm}. All images are resized to $84 \times 84$.

\paragraph{\emph{tiered}ImageNet}

This dataset is also sampled from the ImageNet~\cite{imagenet}. However, rather than randomly sampling classes as in \emph{mini}ImageNet, it follows a hierarchical structure where the sampled classes are partitioned into 34 categories, which are organized into 20 training, 6 validation and 8 test categories, containing 351, 97 and 160 classes, respectively. This hierarchical partitioning strategy ensures that the training classes are semantically distinct from the test classes, making it a more realistic few-shot classification problem. We follow the commonly used split proposed in~\cite{sslmeta}. Again, all images are resized to $84 \times 84$.

\paragraph{CUB}

This is a fine-grained classification dataset consisting of 200 classes, each corresponding to a bird species. We follow the split defined by~\cite{closerlook, fewshotCUB}, with 100 training, 50 validation and 50 test classes. To compare fairly with competitors, we \emph{use} bounding boxes on ResNet features following~\cite{fewshotCUBbounding} to compare with~\cite{lrici} but we \emph{do not use} bounding boxes on WRN features to compare with~\cite{pt_map}.

\paragraph{CIFAR-FS}

This dataset is derived from CIFAR-100~\cite{cifar100db}, consisting of 100 classes with 600 examples per class. We follow the split provided by~\cite{closerlook}, with 64 training, 16 validation and 20 test classes. To compare fairly with competitors, we use the original image resolution of $32 \times 32$ on WRN features to compare with~\cite{pt_map} but we resize images to $84 \times 84$ on ResNet features to compare with~\cite{lrici}.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lcccccccccc}
\toprule
\Th{Inference}        & \mc{5}{\Th{Components}}            & \mc{2}{\Th{ResNet-12}}             & \mc{2}{\Th{WRN-28-10}}             \\ 
                      & \lp & \bal & \ilc & class & \iprob & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
Inductive             &     &      &      &       &        & 56.30\ci{0.62}      & 75.59\ci{0.47}      & 60.04\ci{0.64}      & 81.35\ci{0.43}      \\ 
Transductive          & \ch &      &      &       &        & 61.09\ci{0.70}      & 75.32\ci{0.50}      & 74.35\ci{0.68}      & 84.84\cim           \\ 
Transductive          & \ch & \ch  &      &       &        & 65.04\ci{0.75}      & 76.82\ci{0.50}      & 79.21\ci{0.72}      & 88.00\ci{0.41}      \\ 
Transductive          & \ch & \ch  & \ch  &       &        & \tb{69.79}\ci{0.99} & \tb{79.58}\ci{0.55} & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} \\ 
Transductive          & \ch & \ch  &      &       & \ch    & 58.27\ci{0.91}      & 74.11\ci{0.56}      & 72.28\ci{0.90}      & 85.88\ci{0.46}      \\ 
Transductive$\dagger$ &     &      & \ch  & \ch   &        & -                   & -                   & -                   & -                   \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Ablation study of each component of our method for WRN-28-10 and ResNet-12 backbones on \emph{mini}ImageNet. $\dagger$Linear classifier used for prediction instead of label propagation as in~\cite{lrici}.}
\label{tab:ab-comp}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{figure}
\input{fig/hist/distributions}
\caption{(a,b) Distributions of loss values~\eq{loss} for correctly and incorrectly labeled examples, normalized independently. Uniform label noise: (a) 20\%, (b) 40\%. Pseudo-labels predicted by label propagation and balancing~\eq{argmax} for two different tasks (c,d).}
\label{fig:hist}
\end{figure}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot       & 5-shot                     \\ \midrule
LR+ICI~\cite{lrici}     & ResNet-12A   & 66.80\cip           & 79.26\cip           & 80.79\cip           & 87.92\cip           & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
LR+ICI~\cite{lrici}*    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
\tb{\ours (ours)}       & ResNet-12A   & \tb{69.79}\ci{0.99} & \tb{79.58}\ci{0.55} & \tb{83.49}\ci{0.88} & \tb{89.48}\ci{0.47} & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\ \midrule
PT+MAP~\cite{pt_map}    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}      & -                   & -                   & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
PT+MAP~\cite{pt_map}*   & WRN-28-10    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
LR+ICI~\cite{lrici}*    & WRN-28-10    & 80.61\ci{0.80}      & 87.93\ci{0.44}      & 86.79\ci{0.76}      & 91.73\ci{0.40}      & 84.88\ci{0.79}      &  89.75\ci{0.48}     & 90.18\ci{0.65}      & 93.35\ci{0.30}      \\
\tb{\ours (ours)}       & WRN-28-10    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78} & \tb{91.26}\ci{0.46} & \tb{91.53}\ci{0.59} & \tb{94.27}\ci{0.30} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive few-shot learning methods comparison with same pre-trained backbones. *: our reproduction with official code on our datasets.}
\label{tab:trans-pre}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Setup}
\label{sec:setup}

\paragraph{Tasks}

We consider $N$-way, $K$-shot classification tasks with $N = 5$ randomly sampled novel classes and $K \in \{1, 5\}$ randomly selected examples per class for support set $S$, that is, $L = 5K$ examples in total. For the query set $Q$, we randomly sample $15$ additional examples per class, that is, $M = 75$ examples in total, which is the most common choice in transductive and semi-supervised few shot learning~\cite{tpn, learning2selftrain, transmatch}. 

In the semi-supervised setting, the unlabeled set $U$ contains an additional number of randomly sampled examples per novel class. This number depends on $K$. We use two settings, namely 30/50 and 100/100, where the first number (30 or 100) refers to 1-shot and the second (50 or 100) to 5-shot. Again, these are the two most common choices in semi-supervised few shot learning~\cite{learning2selftrain,lrici,mct,ssmeta,transmatch}.

Unless otherwise stated, we use 1000 tasks and report mean accuracy and 95\% confidence interval on the test set.

\paragraph{Competitors}

As discussed in \autoref{sec:flaws}, there are number of flaws in experimental evaluation in the bibliography, including the use of different networks, different training settings, different versions of datasets, different dimenionalities and pre-processing of features. As a result, it is impossible to provide fair comparisons with the state of the art, unless one uses public code to reproduce results under exactly the same setup.

In this work, we do provide completely fair comparisons with such reproduced results of three state-of-the-art methods: LR+ICI~\cite{lrici}, PT+MAP~\cite{pt_map} and MCT~\cite{mct}. To our knowledge, these methods outperform all other state of the art. Importantly, only~\cite{lrici} is published, while the other two are pre-prints. We compare with these methods in \autoref{sec:trans} (transductive) and \autoref{sec:semi} (semi-supervised), then with other state of the art in \autoref{sec:soa}.

\paragraph{Networks}

We use publicly available pre-trained backbone convolutional neural networks that are trained on the base-class training set. We experiment with two popular networks, namely, the residual network ResNet-12~\cite{tadam} and the wide residual network (WRN-28-10)~\cite{LEO}.

In particular, to compare with~\cite{lrici}, we use pre-trained weights of the ResNet-12 provided by~\cite{lrici}, which we call ResNet-12A, as well as official public code\footnote{\url{https://github.com/Yikai-Wang/ICI-FSL}} for testing. To compare with~\cite{pt_map}, we use pre-trained weights of a WRN-28-10 provided by~\cite{manifoldmixup}\footnote{\url{https://github.com/nupurkmr9/S2M2_fewshot}}, which are the same used by~\cite{pt_map}, as well as official public code\footnote{\url{https://github.com/yhu01/PT-MAP}} for testing. To compare with~\cite{mct}, we use official public code\footnote{\url{https://github.com/seongmin-kye/MCT}} to train from scratch another version of ResNet-12 used by~\cite{mct}, which we call ResNet-12B, as well as the same code for testing.

\paragraph{Implementation details}

Our implementation is based on PyTorch~\cite{pytorch} and FAISS~\cite{faiss}. We set hyperparameters based on the validation set, as discussed in \autoref{sec:ablation}.

\paragraph{Feature pre-processing}

Each method uses its own feature pre-processing choices. For instance, LR+ICI~\cite{lrici} uses PCA to reduce ResNet-12A to 5 dimensions. PR+MAP~\cite{pt_map} uses element-wise power transform, $\ell_2$-normalization and centering of WRN-28-10 features. MCT~\cite{mct} uses flattening of the output tensor of ResNet-12B rather than global spatial pooling, hence dimensionality is in the thousands. By default, we use the same choices as~~\cite{pt_map,mct} for WRN-28-10 and ResNet-12B but we do not use any dimensionality reduction on ResNet-12A, because it hurts performance. We ablate these options in \autoref{sec:trans}.

(On ResNet-12A,B and WRN). Ablation below.
 
In the pre-processing step we consider either using the pre-processing step that each method uses or not using it. In ~\cite{pt_map}, 

We assume that since each method uses the pre-processing step it is because it improves its performance, thus omitting it can be classed as fair comparison. In all of our transductive experiments we used the pre-processing provided by each work, while on the semi-supervised setting when comparing with ~\cite{lrici} we did not use the pre-processing step since we found that our method works better by omitting it.

\alert{
Training details? Optimizer, learning rate and schedule, batch size etc. used in cleaning?

The cleaning module is used at every iteration right after the label propagation step. We provide all the support and query examples with their labels and predicted pseudolabels respectively to the cleaning module. We do not provide any information which are the support and which are the query examples thus they are all treated as labelled examples. We initialize the cleaning module's weights by imprinting the average of the support features of each class. We train the cleaning module using a cyclic learning rate for 200 iterations where each cycle is 20 iterations. We use SGD optimizer with momentum of factor 0.9 and $L_2$ penalty of factor 0.0005.

Is $\vp$ used~\eq{sink-row},\eq{sink-col},\eq{loss} or just uniform? Ablation below.
}

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}          & \mc{2}{\Th{Cifar-FS}}                     \\ 
                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot                & 1-shot              & 5-shot              \\ \midrule
PT+MAP~\cite{pt_map}*   & WRN-28-10    & 83.79\ci{0.71}      & 88.94\ci{0.33}      & 88.87\ci{0.64}      & 92.01\ci{0.36}        & 87.63\ci{0.66}      & 90.15\ci{0.46}      \\
\tb{\ours (ours)}       & WRN-28-10    & \tb{86.30}\ci{0.71} & \tb{89.99}\ci{0.32} & \tb{90.60}\ci{0.64} &\tb{92.97}\ci{0.38}    & \tb{88.51}\ci{0.69} & \tb{91.23}\ci{0.44} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive few-shot 50-queries comparison. *: our reproduction with official code on our datasets.}
\label{tab:trans-50q}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength\tabcolsep{4pt}
\begin{tabular}{lccccc}
\toprule
\Th{Method}             & \Th{\emph{m}IN}     & \Th{\emph{t}IN}     & \Th{Cifar-FS}       & \Th{CUB}            \\ \midrule
PT+MAP~\cite{pt_map}*   & 89.97\ci{0.34}      & 93.33\ci{0.34}      & 91.30\ci{0.45}      & 94.24\ci{0.28}      \\
\tb{\ours (ours)}       & \tb{90.51}\ci{0.35} & \tb{93.61}\ci{0.38} & \tb{91.59}\ci{0.44} & \tb{94.75}\ci{0.26} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive 10-shot comparison with PT+MAP~\cite{pt_map} using WRN-28-10. \emph{m}IN: \emph{mini}ImageNet. \emph{t}IN: \emph{tiered}ImageNet. *: our reproduction with official code on our datasets.}
\label{tab:trans-10shot}
\end{table}

%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Ablation study}
\label{sec:ablation}

\paragraph{Hyperparameters}

We optimize all hyperparameters on the validation set of every dataset. This includes hyperparameters $\gamma$ and $k$ used in the nearest neighbor graph~\eq{affinity}, $\alpha$ used in label propagation~\eq{lp} and $\tau$ used in balancing~\eq{balance}.

\alert{We set $\tau=3$.}

\paragraph{Algorithmic components}

\autoref{tab:ab-comp}.

%------------------------------------------------------------------------------

\subsection{Label cleaning: loss distribution}
\label{sec:hist}

To illustrate the effectiveness of our label cleaning, we conduct two experiments with different label noise and we show the distribution of the loss value~\eq{loss} for correctly and incorrectly labeled examples. In the first experiment, shown in \autoref{fig:hist}(a,b), we collect 500 correctly labeled examples and inject label noise uniformly at random to the 20\%~(a) and 40\%~(b) of the data. The correctly and incorrectly labeled examples have very different loss distributions. Importantly, while previous work on label cleaning~\cite{ArazoOAOM19,o2u,robustonfly} attempts to detect clean examples by applying an optimal threshold on the loss value, due to the iterative nature of our algorithm we only need to find few clean examples at a time. It is clear that the examples with minimal loss value are clean.

The second experiment is on two novel \alert{5-way 5-shot} tasks in the transductive setting, as shown in \autoref{fig:hist}(c,d). We use 50 additional unlabeled novel-class queries in each task and we predict pseudo-labels using label propagation and balancing, according to~\eq{argmax}. In this case, label cleaning is more challenging because the distibutions of correctly and incorrectly labeled examples are more overlapping. This is natural because predictions are more informed than uniform, even if incorrect. Still, a large proportion of clean examples have less loss than the minimal value of noisy ones.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\Th{Method}             & \mc{3}{\Th{Components}}  & \mc{2}{\emph{mini}ImageNet}               & \mc{2}{\emph{tiered}ImageNet}             \\ 
                        & PT     & Norm   & Center & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
PT+MAP~\cite{pt_map}*   & -      & -      & -      & 48.57\ci{0.81}      & 75.67\ci{0.82}      & 49.67\ci{0.77}      & 88.32\ci{0.50}      \\ 
\tb{\ours (ours)}       & -      & -      & -      & \textit{74.09}      & \textit{81.58}       & \textit{86.54}     & \textit{90.17}                    \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch    & -      & -      & 44.13\ci{0.56}      & 80.58\ci{0.44}      & 21.84\ci{0.58}      & 78.81\ci{1.43}      \\ 
\tb{\ours (ours)}       & \ch    & -      & -      & \tb{68.01}\ci{0.89}      & \tb{80.89}\ci{0.49}&  78.00\ci{0.91} & 89.40 \ci{0.49}           \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch    & \ch    & -      & 73.41\ci{0.64}      & 84.86\ci{0.42}      & 83.88\ci{0.69}      & 90.48\ci{0.42}      \\ 
\tb{\ours (ours)}       & \ch    & \ch    &        & -                   & -                   &                     &                     \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch    &    -   & \ch    & 80.60\ci{0.81}      & 87.42\ci{0.43}      & 86.50\ci{0.77}      &  91.11\ci{0.46}     \\ 
\tb{\ours (ours)}       & \ch    &   -    & \ch    & -                   & -                   & -                   &                     \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch    & \ch    & \ch    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      \\
\tb{\ours (ours)}       & \ch    & \ch    & \ch    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Robustness comparison our method against~\cite{pt_map} for WRN-28-10 on \emph{mini}ImageNet and \emph{tiered}ImageNet. *: our reproduction with official code on our datasets.}
\label{tab:ab-pt}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength\tabcolsep{2pt}
\begin{tabular}{lccccc}
\toprule
\Th{Method}                & \mc{2}{\Th{\emph{mini}ImageNet}} & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ \midrule 
                           & 1-shot         & 5-shot          & 1-shot         & 5-shot            \\ \midrule
MCT (instance)~\cite{mct}  & 78.55\ci{0.86} & 86.03\ci{0.42}  & 82.32\ci{0.81} & 87.36\ci{0.50}    \\
MCT (instance)~\cite{mct}* & 77.10\ci{0.88} & 86.19\ci{0.40}  & -              & -                 \\
\tb{\ours (ours)}          & \tb{-}         & \tb{-}          & -              & \tb{-}            \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transducive few-shot learning comparison with MCT~\cite{mct} using ResNet-12B. *: our reproduction with official code on our datasets.}
\label{tab:trans-mct}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Transductive inference}
\label{sec:trans}

\autoref{tab:trans-pre} compares our method with LR+ICI~\cite{lrici} and PT+MAP~\cite{pt_map} on all four datasets. The truly fair comparison is with our reproductions, indicated by *. We compare our method against the other two using the backbone that each work based its experimental results. Since WRN-28-10 provides more expressive features, we compare our method against ~\cite{lric} by using WRN-28-10 backbone as well.  \alert{Our method is superior or on par with competitors, except CUB 1-shot where the difference with~\cite{pt_map}is very small THIS CAN BE REMOVED WE ARE A BIT BETTER/EQUAL HERE}. The gain over~\cite{lrici} is 1-2\%. most notably 3\% on \emph{mini}ImageNet 1-shot. The gain over PT+MAP~\cite{pt_map} is around 0.5\%. 

Because the gain over~\cite{pt_map} is small, we perform comparison under two additional settings. The first is 10-shot, using more labeled support examples. As shown in \autoref{tab:trans-10shot}, the gain is again around 0.5\%. The second is using more unlabeled queries, that is, 50 queries per class or $M=250$ in total. As shown in \autoref{tab:trans-50q}, the gain now increases to 1-2\%, even 3\% on \emph{mini}ImageNet 1-shot. This can be attributed to the fact that PT+MAP~\cite{pt_map} operates on Euclidean space, while our method captures the manifold structure, which manifests itself in the presence of more data.

\alert{As a robustness test, we compare the two methods by a robustness ablation study, removing completely or using different combinations of the pre-processing part as well as removing the balancing with the raised exponent $\tau$. It can be clearly seen from table \autoref{tab:ab-pt} that our method is much more robust in every experimented scenario. Without this exact processing regime, PT+MAP can be just as bad as random sampling as it can be seen in the 1-shot setting of tieredImageNet. These results highlight the generality of our method as it is much more robust to pre-processing schemes and can be used effective without much deterioration in performance.}

\alert{\autoref{tab:trans-mct} compares our method with MCT~\cite{mct}.}

%------------------------------------------------------------------------------
%\begin{table*}
%\small
%\centering
%\begin{tabular}{lccccccccc}
%\toprule
%\Th{Method}                               & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}  & \mc{2}{\Th{\emph{tiered}ImageNet}} & \mc{2}{\Th{Cifar-FS}}           & \mc{2}{\Th{CUB}}                \\ 
%                                          &              & 1-shot           & 5-shot         & 1-shot         & 5-shot            & 1-shot         & 5-shot         & 1-shot         & 5-shot         \\ \midrule
%PT+MAP (no-pre)~\cite{pt_map}*            & WRN-28-10    & 48.57\ci{0.81}   & 75.67\ci{0.82} & 49.67\ci{0.77} & 88.32\ci{0.50}    & 20.16\ci{0.04} & 20.77\ci{0.08} & 62.99\ci{1.23} & 85.94\ci{0.85} \\
%\tb{\ours (ours, no-pre)}                 & WRN-28-10    & \tb{-}           & \tb{-}         & -              & \tb{-}            & \tb{-}         & \tb{-}         & -              & \tb{-}         \\ \midrule
%PT+MAP (no-sink)~\cite{pt_map}*           & WRN-28-10    & 81.12\ci{0.71}   & 87.66\ci{0.40} & 87.62\ci{0.64} & 91.27\ci{0.40}    & 85.28\ci{0.71} & 89.34\ci{0.47} & 89.89\ci{0.60} & 92.55\ci{0.31} \\
%\tb{\ours (ours)}                         & WRN-28-10    & \tb{-}           & \tb{-}         & -              & \tb{-}            & \tb{-}         & \tb{-}         & -              & \tb{-}         \\ \midrule
%PT+MAP (no-sink/no-$\tau$)~\cite{pt_map}* & WRN-28-10    & 70.09\ci{0.61}   & 83.89\ci{0.41} & 78.48\ci{0.63} & 89.25\ci{0.42}    & 77.27+0.63     & 87.68\ci{0.48} & 82.97\ci{0.59} & 91.45\ci{0.35} \\
%\tb{\ours (ours, no-bal/no-$\tau$)}       & WRN-28-10    & \tb{-}           & \tb{-}         & -              & \tb{-}            & \tb{-}         & \tb{-}         & -              & \tb{-}         \\
%\bottomrule
%\end{tabular}
%\vspace{6pt}
%\caption{Ablation on robustness of our algorithm in comparison to the best state-of-the-Art method}
%\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{4.5pt}
\begin{tabular}{lcccccccccc}
\toprule
\Th{Method}            & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                & \mc{2}{\Th{CUB}}                \\ 
                       &              &            & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot         & 5-shot              & 1-shot              & 5-shot    \\ \midrule
LR+ICI~\cite{lrici}    & ResNet-12A   & 30/50      & 69.66\cip           & 80.11\cip           & 84.01\cip           & 89.00\cip           & 76.51\cip      & 84.32\cip           & 89.58\cip           & 92.48\cip \\
LR+ICI~\cite{lrici}*   & ResNet-12A   & 30/50      & 67.64\ci{0.95}      & 80.00\ci{0.55}      & 83.20\ci{0.89}      & 89.15\ci{0.48}      & 76.57\ci{0.96} & 84.11\ci{0.60}      & 88.36\ci{0.71}      & -         \\
\tb{\ours (ours)}      & ResNet-12A   & 30/50      & \tb{70.67}\ci{0.98} & \tb{81.48}\ci{0.53} & 83.49\ci{0.80}      & 88.65\ci{0.45}      & 76.46\ci{0.88} & \tb{85.06}\ci{0.56} & \tb{89.92}\ci{0.63} & -         \\ 
\tb{\ours$\dagger$}    & ResNet-12A   & 30/50      & \tb{72.36}\ci{0.93} & \tb{81.23}\ci{0.51} & \tb{84.34}\ci{0.77} & \tb{89.66}\ci{0.49} & -              & -                   & -                   & -         \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised inductive few-shot learning methods comparison with same pre-trained backbones. * represents our re-implementation based on the original code and our datasets, $\dagger$ represents unormalized features}
\label{tab:semi_pre}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Semi-supervised learning}
We compare our method against ~\cite{lrici} in the semi-supervised few-shot learning scenario. As it can be seen from table \autoref{tab:semi_pre} our method is superior in all investigated settings from ~\cite{lrici} by even wider margin than from the transductive setting highlighted by the ~4.5\% difference in \emph{mini}ImageNet. 
\label{sec:semi}

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lcccccc}
\toprule
\Th{Method}                             & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}     & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ 
                                        &              &            & 1-shot         & 5-shot              & 1-shot         & 5-shot            \\ \midrule
%TPN$_{SSL}$\cite{tpn}                  & CONV-4       & 20/20      & 52.78          & 66.42               & 55.74          & 71.01             \\
%k-means$_{masked, soft}$~\cite{ssmeta} & CONV-4       & 20/20      & 50.41          & 64.39               & -              & -                 \\
%\tb{\ours (ours)}                      & CONV-4       & 20/20      &                &                     &                &                   \\ \midrule
LST~\cite{learning2selftrain}           & ResNet-12    & 30/50      & 70.10\ci{1.90} & 78.70\ci{0.80}      & 77.70\ci{1.60} & 85.20\ci{0.80}    \\
LR+ICI~\cite{lrici}                     & ResNet-12    & 30/50      & 69.66\cip      & 80.11\cip           & 84.01\cip      & 89.00\cip         \\
MCT (instance)~\cite{mct}               & ResNet-12    & 30/50      & 73.80\ci{0.70} & 84.40\ci{0.50}      & 76.90\ci{0.70} & 86.30\ci{0.50}    \\
\tb{\ours (ours)}                       & ResNet-12    & 30/50      &                &                     &                &                   \\ \midrule
%LR+ICI~\cite{lrici}                    & ResNet-12    & 80/80      & 71.41          & 81.12               & 85.44          & 89.12             \\
%\tb{\ours (ours)}                      & ResNet-12    & 80/80      &                &                     &                &                   \\ \midrule
*k-means$_{masked, soft}$~\cite{ssmeta} & WRN-28-10    & 100/100    & 52.35\ci{0.89} & 67.67\ci{0.65}      & -              & -                 \\
TransMatch~\cite{transmatch}            & WRN-28-10    & 100/100    & 63.02\ci{1.07} & 81.06\ci{0.59}      & -              & -                 \\
\tb{\ours (ours)}                       & WRN-28-10    & 100/100    &                & \tb{87.73}\ci{0.37} &   -            &  -                \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised inductive few-shot learning methods comparison. *Re-implemented~\cite{transmatch}}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}                             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}         & \mc{2}{\Th{\emph{tiered}ImageNet}}       & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                                        &              & 1-shot              & 5-shot             & 1-shot              & 5-shot             & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
LR+ICI~\cite{lrici}                     & ResNet-12A   & 66.80\cip           & 79.26\cip          & 80.79\cip           & 87.92\cip          & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
LR+ICI~\cite{lrici}*                    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}     & 82.40\ci{0.84}      & 88.80\ci{0.50}     & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
CAN+Top-\emph{k}~\cite{crossattention}  & ResNet-12    & 67.19\ci{0.55}      & 80.64\ci{0.35}     & 73.21\ci{0.58}      & 84.93 \ci{0.38}    & -                   & -                   & -                   & -                   \\
DPGN~\cite{DPGN}                        & ResNet-12    & 67.77\ci{0.32}      & 84.60\ci{0.43}     & 72.45\ci{0.51}      & 87.24\ci{0.39}     & 77.90\ci{0.50}      & 90.20\ci{0.40}      & 75.71\ci{0.47}      & 91.48\ci{0.33}      \\
EP~\cite{embeddingpropagation}          & ResNet-12    & 66.50\ci{0.89}      & 81.06\ci{0.60}     & 76.53\ci{0.87}      & 87.32\ci{0.64}     & -                   & -                   & -                   & -                   \\
MCT (Instance)~\cite{mct}               & ResNet-12    & 78.55\ci{0.86}      & 86.03\ci{0.42}     & 82.32\ci{0.81}      & 87.36\ci{0.50}     & 85.61\ci{0.69}      & 90.03\ci{0.46}      & -                   & -                   \\
MCT (Pair)~\cite{mct}                   & ResNet-12    & 76.16\ci{0.89}      & 85.22\ci{0.42}     & 80.68\ci{0.89}      & 86.63\ci{0.89}     & 87.28\ci{0.70}      & 90.50\ci{0.43}      & -                   & -                   \\
\tb{\ours (ours)}                       & ResNet-12A   & \tb{69.79}\ci{0.99} &\tb{79.58}\ci{0.55} & \tb{83.49}\ci{0.88} &\tb{89.48}\ci{0.47} & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\ \midrule
PT+MAP~\cite{pt_map}                    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}     & -                   & -                  & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
PT+MAP~\cite{pt_map}*                   & WRN-28-10    & 82.88\ci{0.73}      & 88.78\ci{0.40}     & 88.15\ci{0.71}      & 92.32\ci{0.40}     & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
Fine-tuning~\cite{baseline_ft}          & WRN-28-10    & 65.73\ci{0.68}      & 78.40\ci{0.52}     & 73.34\ci{0.71}      & 85.50\ci{0.50}     & 76.58\ci{0.68}      & 85.79\ci{0.50}      & -                   & -                   \\
EP~\cite{embeddingpropagation}          & WRN-28-10    & 70.74\ci{0.85}      & 84.34\ci{0.53}     & 78.50\ci{0.91}      & 88.36\ci{0.57}     & -                   & -                   & -                   & -                   \\
SIB~\cite{SIB}                          & WRN-28-10    & 70.00\ci{0.60}      & 79.20\ci{0.40}     & 72.90$\dagger$      & 82.80$\dagger$     & 80.00\ci{0.60}      & 85.3\ci{0.40}       & -                   & -                   \\
DPGN~\cite{DPGN}                        & WRN-28-10    & 67.24\ci{0.51}      & 83.72\ci{0.44}     & -                   & -                  & -                   & -                   & -                   & -                   \\
SIB+E$^3$BM~\cite{ensemblefsl}          & WRN-28-10    & 71.40\ci{0.50}      & 81.20\ci{0.4}      & 75.60\ci{0.6}       & 84.30\ci{0.4}      & -                   & -                   & -                   & -                   \\
\tb{\ours (ours)}                       & WRN-28-10     & \tb{83.43}\ci{0.79}& \tb{89.10}\ci{0.42}   & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78}      & \tb{91.26}\ci{0.46}      & 91.53\ci{0.59}      & \tb{94.27}\ci{0.30} \\ \bottomrule
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive few-shot learning methods comparison with all state-of-the-Art. * represents our re-implementation based on the original code and our datasets, $\dagger$ implementation carried out by~\cite{ensemblefsl}}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Flaws in evaluation}
\label{sec:flaws}
Throughout our investigations we noted that comparisons that are not under the same settings have commonly been published. For example comparisons have been made between transductive and inductive methods without indication that one method leverages the full unlabeled query set while the other does not. In semi-supervised specifically, comparisons between different methods has been made without consideration of the number of available data used in each work thus making it hard to understand the value of contribution of each work. Also, unless the novelty of the work lies in the training regime, it is unfair to compare methods that have been trained using different training regimes or different backbone architectures. It has also been noted that some works use bounding boxes to crop the images, such as in CUB, while others do not.

We encourage the community to compare works against the same settings and if otherwise state clearly in an attempt to move to an unbiased direction and solbe the few-shot learning problem. As a way to contribute towards a fairer comparison regime, we are planning to make our code publicly available along with the pre-trained networks used in this work for everyone to use.


%------------------------------------------------------------------------------

\subsection{Comparison with the state of the art}
\label{sec:soa}



==> tex/experiments-3.tex <==
\section{Experiments}
\label{sec:experiments}

%------------------------------------------------------------------------------
\extdata{fig/data/sample}
%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
%------------------------------------------------------------------------------

% We evaluate and compare our proposed method with the state-of-the-art methods in trasnductive and semi-supervised few-shot learning on the four most commonly used databases, \emph{mini}ImageNet~\cite{ravilstm, matchingNets}, \emph{tiered}ImageNet~\cite{ssmeta}, \emph{cifar-FS} and \emph{CUB}. 

%------------------------------------------------------------------------------

\subsection{Datasets}
\label{sec:data}

\paragraph{\emph{mini}ImageNet}

This is a widely used few-shot image classification dataset~\cite{matchingNets, ravilstm}. It contains 100 randomly sampled classes from ImageNet~\cite{imagenet}. These 100 classes are split into 64 training (base) classes, 16 validation (novel) classes and 20 test (novel) classes. Each class contains 600 examples (images). We follow the commonly used split proposed in~\cite{ravilstm}. All images are resized to $84 \times 84$.

\paragraph{\emph{tiered}ImageNet}

This dataset is also sampled from the ImageNet~\cite{imagenet}. However, rather than randomly sampling classes as in \emph{mini}ImageNet, it follows a hierarchical structure where the sampled classes are partitioned into 34 categories, which are organized into 20 training, 6 validation and 8 test categories, containing 351, 97 and 160 classes, respectively. This hierarchical partitioning strategy ensures that the training classes are semantically distinct from the test classes, making it a more realistic few-shot classification problem. We follow the commonly used split proposed in~\cite{sslmeta}. Again, all images are resized to $84 \times 84$.

\paragraph{CUB}

This is a fine-grained classification dataset consisting of 200 classes, each corresponding to a bird species. We follow the split defined by~\cite{closerlook, fewshotCUB}, with 100 training, 50 validation and 50 test classes. To compare fairly with competitors, we \emph{use} bounding boxes on ResNet features following~\cite{fewshotCUBbounding} to compare with~\cite{lrici} but we \emph{do not use} bounding boxes on WRN features to compare with~\cite{pt_map}.

\paragraph{CIFAR-FS}

This dataset is derived from CIFAR-100~\cite{cifar100db}, consisting of 100 classes with 600 examples per class. We follow the split provided by~\cite{closerlook}, with 64 training, 16 validation and 20 test classes. To compare fairly with competitors, we use the original image resolution of $32 \times 32$ on WRN features to compare with~\cite{pt_map} but we resize images to $84 \times 84$ on ResNet features to compare with~\cite{lrici}.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lcccccccccc}
\toprule
\Th{Inference}          & \mc{5}{\Th{Components}}            & \mc{2}{\Th{ResNet-12}}             & \mc{2}{\Th{WRN-28-10}}             \\ 
                        & \lp & \bal & \ilc & \cp & \iprob & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
Inductive               &     &      &      &     &        & 56.30\ci{0.62}      & 75.59\ci{0.47}      & 60.04\ci{0.64}      & 81.35\ci{0.43}      \\ 
Transductive            & \ch &      &      &     &        & 61.09\ci{0.70}      & 75.32\ci{0.50}      & 74.35\ci{0.68}      & 84.84\cim           \\ 
Transductive            & \ch & \ch  &      &     &        & 65.04\ci{0.75}      & 76.82\ci{0.50}      & 79.21\ci{0.72}      & 88.00\ci{0.41}      \\ 
Transductive            & \ch & \ch  & \ch  &     &        & \tb{69.79}\ci{0.99} & \tb{79.58}\ci{0.55} & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} \\ 
Transductive            & \ch & \ch  &      &     & \ch    & 58.27\ci{0.91}      & 74.11\ci{0.56}      & 72.28\ci{0.90}          & 85.88\ci{0.46}      \\ 
Transductive            &     & \ch  & \ch  & \ch &        & -                   & -                   & -                   & -                   \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Ablation study of algorithmic components of our method on \emph{mini}ImageNet. Inductive: baseline using only support examples. \lp: label propagation. \bal: class balancing~\eq{balance}. \ilc: iterative label cleaning, without which we just output predictions~\eq{argmax}. \cp: linear classifier used for prediction instead of \lp, as in~\cite{lrici}, with balancing still applied on output probabilities. \iprob: iterative selection of top examples per class directly as column-wise maxima of $P$~\eq{sub} instead of \ilc.}
\label{tab:ab-comp}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{figure}
\input{fig/hist/distributions}
\caption{(a,b) Distributions of loss values~\eq{loss} for correctly and incorrectly labeled examples, normalized independently. Uniform label noise: (a) 20\%, (b) 40\%. Pseudo-labels predicted by label propagation and balancing~\eq{argmax} for two different tasks (c,d).}
\label{fig:hist}
\end{figure}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot       & 5-shot                     \\ \midrule
LR+ICI~\cite{lrici}     & ResNet-12A   & 66.80\cip           & 79.26\cip           & 80.79\cip           & 87.92\cip           & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
LR+ICI~\cite{lrici}*    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
\tb{\ours (ours)}       & ResNet-12A   & \tb{69.79}\ci{0.99} & \tb{79.58}\ci{0.55} & \tb{83.49}\ci{0.88} & \tb{89.48}\ci{0.47} & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\ \midrule
PT+MAP~\cite{pt_map}    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}      & -                   & -                   & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
PT+MAP~\cite{pt_map}*   & WRN-28-10    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
LR+ICI~\cite{lrici}*    & WRN-28-10    & 80.61\ci{0.80}      & 87.93\ci{0.44}      & 86.79\ci{0.76}      & 91.73\ci{0.40}      & 84.88\ci{0.79}      &  89.75\ci{0.48}     & 90.18\ci{0.65}      & 93.35\ci{0.30}      \\
\tb{\ours (ours)}       & WRN-28-10    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78} & \tb{91.26}\ci{0.46} & \tb{91.53}\ci{0.59} & \tb{94.27}\ci{0.30} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive few-shot learning methods comparison with same pre-trained backbones. *: our reproduction with official code on our datasets.}
\label{tab:trans-pre}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Setup}
\label{sec:setup}

\paragraph{Tasks}

We consider $N$-way, $K$-shot classification tasks with $N = 5$ randomly sampled novel classes and $K \in \{1, 5\}$ randomly selected examples per class for support set $S$, that is, $L = 5K$ examples in total. For the query set $Q$, we randomly sample $15$ additional examples per class, that is, $M = 75$ examples in total, which is the most common choice in transductive and semi-supervised few shot learning~\cite{tpn, learning2selftrain, transmatch}. 

In the semi-supervised setting, the unlabeled set $U$ contains an additional number of randomly sampled examples per novel class. This number depends on $K$. We use two settings, namely 30/50 and 100/100, where the first number (30 or 100) refers to 1-shot and the second (50 or 100) to 5-shot. Again, these are the two most common choices in semi-supervised few shot learning~\cite{learning2selftrain,lrici,mct,ssmeta,transmatch}.

Unless otherwise stated, we use 1000 tasks and report mean accuracy and 95\% confidence interval on the test set.

\paragraph{Competitors}

As discussed in the supplementary material, there are number of flaws in experimental evaluation in the bibliography, including the use of different networks, different training settings, different versions of datasets, different dimenionalities and pre-processing of features. As a result, it is impossible to provide fair comparisons with the state of the art, unless one uses public code to reproduce results under exactly the same setup.

In this work, we do provide completely fair comparisons with such reproduced results of three state-of-the-art methods: LR+ICI~\cite{lrici}, PT+MAP~\cite{pt_map} and MCT~\cite{mct}. To our knowledge, these methods outperform all other state of the art. Importantly, only~\cite{lrici} is published, while the other two are pre-prints. We compare with these methods in \autoref{sec:trans} (transductive) and \autoref{sec:semi} (semi-supervised), then with other state of the art in \autoref{sec:soa}.

\paragraph{Networks}

We use publicly available pre-trained backbone convolutional neural networks that are trained on the base-class training set. We experiment with two popular networks, namely, the residual network ResNet-12~\cite{tadam} and the wide residual network (WRN-28-10)~\cite{LEO}.

In particular, to compare with~\cite{lrici}, we use pre-trained weights of the ResNet-12 provided by~\cite{lrici}, which we call ResNet-12A, as well as official public code\footnote{\url{https://github.com/Yikai-Wang/ICI-FSL}} for testing. To compare with~\cite{pt_map}, we use pre-trained weights of a WRN-28-10 provided by~\cite{manifoldmixup}\footnote{\url{https://github.com/nupurkmr9/S2M2_fewshot}}, which are the same used by~\cite{pt_map}, as well as official public code\footnote{\url{https://github.com/yhu01/PT-MAP}} for testing. To compare with~\cite{mct}, we use official public code\footnote{\url{https://github.com/seongmin-kye/MCT}} to train from scratch another version of ResNet-12 used by~\cite{mct}, which we call ResNet-12B, as well as the same code for testing.

\paragraph{Feature pre-processing}

Each method uses its own feature pre-processing choices. For instance, LR+ICI~\cite{lrici} uses $\ell_2$-normalization and PCA to reduce ResNet-12A to 5 dimensions. PR+MAP~\cite{pt_map} uses element-wise power transform, $\ell_2$-normalization and centering of WRN-28-10 features. MCT~\cite{mct} uses flattening of the output tensor of ResNet-12B rather than global spatial pooling, hence dimensionality is in the thousands. By default, we use the same choices as~\cite{pt_map,mct} for WRN-28-10 and ResNet-12B. For ResNet-12A however, we use $\ell_2$-normalization only on transductive inference and we do not use any dimensionality reduction. We ablate these options in \autoref{sec:trans}.

\paragraph{Implementation details}

We use PyTorch~\cite{pytorch}, FAISS \cite{faiss} and scikit-learn~\cite{sklearn}. Label cleaning is based on a linear classifier on top of embedding $f$, initialized by imprinting the average of support features per class and then trained using~\eq{loss}. We use SGD with momentum 0.9 and weight decay 0.0005. Following~\cite{o2u}, we use a cyclical schedule of 10 cycles with 20 iterations per cycle for the learning rate, which linearly decreases from a maximum rate to zero. For inductive (resp. semi-supervised) learning, we use logistic regression on support (resp. as well as pseudo-labeled) examples, learned using scikit-learn like~\cite{lrici}. The row-wise sum $\vp$~\eq{sink-row} is either fixed to 1 for all examples or set to a weight in $[0,1]$ according to entropy, following~\cite{semilpavrithis}.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}          & \mc{2}{\Th{Cifar-FS}}                     \\ 
                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot                & 1-shot              & 5-shot              \\ \midrule
PT+MAP~\cite{pt_map}*   & WRN-28-10    & 83.79\ci{0.71}      & 88.94\ci{0.33}      & 88.87\ci{0.64}      & 92.01\ci{0.36}        & 87.63\ci{0.66}      & 90.15\ci{0.46}      \\
\tb{\ours (ours)}       & WRN-28-10    & \tb{86.30}\ci{0.71} & \tb{89.99}\ci{0.32} & \tb{90.60}\ci{0.64} &\tb{92.97}\ci{0.38}    & \tb{88.51}\ci{0.69} & \tb{91.23}\ci{0.44} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive few-shot 50-queries comparison. *: our reproduction with official code on our datasets.}
\label{tab:trans-50q}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength\tabcolsep{4pt}
\begin{tabular}{lccccc}
\toprule
\Th{Method}             & \Th{\emph{m}IN}     & \Th{\emph{t}IN}     & \Th{Cifar-FS}       & \Th{CUB}            \\ \midrule
PT+MAP~\cite{pt_map}*   & 89.97\ci{0.34}      & 93.33\ci{0.34}      & 91.30\ci{0.45}      & 94.24\ci{0.28}      \\
\tb{\ours (ours)}       & \tb{90.51}\ci{0.35} & \tb{93.61}\ci{0.38} & \tb{91.59}\ci{0.44} & \tb{94.75}\ci{0.26} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive 10-shot comparison with PT+MAP~\cite{pt_map} using WRN-28-10. \emph{m}IN: \emph{mini}ImageNet. \emph{t}IN: \emph{tiered}ImageNet. *: our reproduction with official code on our datasets.}
\label{tab:trans-10shot}
\end{table}

%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Ablation study}
\label{sec:ablation}

\paragraph{Hyperparameters}

We optimize all hyperparameters on the validation set of every dataset. This includes hyperparameters $\gamma$ and $k$ used in the nearest neighbor graph~\eq{affinity}, $\alpha$ used in label propagation~\eq{lp} and $\tau$ used in balancing~\eq{balance}.

\alert{We set $\tau=3$.}

\paragraph{Algorithmic components}

\autoref{tab:ab-comp} ablates the performance of our method in the presence or not of individual components, as well as using alternatives to our components. The use of queries with label propagation immediately gives a strong gain of transductive over inductive inference, especially in 1-shot.


First of all it can be seen than leveraging the manifold structure of the data through label propagation provides better results in comparison to using just a classifier to predict the pseudolabels as it it the case in the inductive section. Furthermore, it can be seen that using our balancing module, the performance is enhanced even more, especially in the 1-shot setting where performance is increased by ~4\%. The most profound result can be seen by comparing our iterative cleaning module, \ilc, to just using the maximum probability of each pseudolabel per class. Using only the probability as a comparative measure to sort the pseudolabels and carry out iterative label propagation, the performance deteriorates while in direct contrast using \ilc the performance improves yet again by around ~4\% in both networks. Lastly the difference between our cleaning module and sorting by probability is ~10\% on the 1-shot setting and ~5\% on the 5-shot setting.

%------------------------------------------------------------------------------

\subsection{Label cleaning: loss distribution}
\label{sec:hist}

To illustrate the effectiveness of our label cleaning, we conduct two experiments with different label noise and we show the distribution of the loss value~\eq{loss} for correctly and incorrectly labeled examples. In the first experiment, shown in \autoref{fig:hist}(a,b), we collect 500 correctly labeled examples and inject label noise uniformly at random to the 20\%~(a) and 40\%~(b) of the data. The correctly and incorrectly labeled examples have very different loss distributions. Importantly, while previous work on label cleaning~\cite{ArazoOAOM19,o2u,robustonfly} attempts to detect clean examples by applying an optimal threshold on the loss value, due to the iterative nature of our algorithm we only need to find few clean examples at a time. It is clear that the examples with minimal loss value are clean.

The second experiment is on two novel \alert{5-way 5-shot} tasks in the transductive setting, as shown in \autoref{fig:hist}(c,d). We use 50 additional unlabeled novel-class queries in each task and we predict pseudo-labels using label propagation and balancing, according to~\eq{argmax}. In this case, label cleaning is more challenging because the distributions of correctly and incorrectly labeled examples are more overlapping. This is natural because predictions are more informed than uniform, even if incorrect. Still, a large proportion of clean examples have less loss than the minimal value of noisy ones.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\Th{Method}             & \mc{3}{\Th{Components}}  & \mc{2}{\emph{mini}ImageNet}               & \mc{2}{\emph{tiered}ImageNet}             \\ 
                        & PT     & Norm   & Center & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
PT+MAP~\cite{pt_map}*   & -      & -      & -      & 48.57\ci{0.81}      & 75.67\ci{0.82}      & 49.67\ci{0.77}      & 88.32\ci{0.50}      \\ 
\tb{\ours (ours)}       & -      & -      & -      & 78.89\ci{0.90}      & 86.80\ci{0.46}      & 86.52\ci{0.47}      & 91.07\ci{0.47}                    \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch    & -      & -      & 44.13\ci{0.56}      & 80.58\ci{0.44}      & 21.84\ci{0.58}      & 78.81\ci{1.43}      \\ 
\tb{\ours (ours)}       & \ch    & -      & -      & 68.01\ci{0.89}      & 80.89\ci{0.49}      & 78.00\ci{0.91}      & 89.40 \ci{0.49}           \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch    & \ch    & -      & 73.41\ci{0.64}      & 84.86\ci{0.42}      & 83.88\ci{0.69}      & 90.48\ci{0.42}      \\ 
\tb{\ours (ours)}       & \ch    & \ch    &        & 68.02\ci{0.89}      & 80.88\ci{0.49}      & 78.00\ci{0.91}      & 89.40\ci{0.49}                   \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch    &    -   & \ch    & 80.60\ci{0.81}      & 87.42\ci{0.43}      & 86.50\ci{0.77}      & 91.11\ci{0.46}     \\ 
\tb{\ours (ours)}       & \ch    &   -    & \ch    & 68.86\ci{0.93}      & 79.94\ci{0.55}     & 78.36\ci{0.93}      &                     \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch    & \ch    & \ch    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      \\
\tb{\ours (ours)}       & \ch    & \ch    & \ch    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Robustness comparison our method against~\cite{pt_map} for WRN-28-10 on \emph{mini}ImageNet and \emph{tiered}ImageNet. *: our reproduction with official code on our datasets.}
\label{tab:ab-pt}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength\tabcolsep{2pt}
\begin{tabular}{lccccc}
\toprule
\Th{Method}                & \mc{2}{\Th{\emph{mini}ImageNet}} & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ \midrule 
                           & 1-shot         & 5-shot          & 1-shot         & 5-shot            \\ \midrule
MCT (instance)~\cite{mct}  & 78.55\ci{0.86} & 86.03\ci{0.42}  & 82.32\ci{0.81} & 87.36\ci{0.50}    \\
MCT (instance)~\cite{mct}* & 77.10\ci{0.88} & 86.19\ci{0.40}  & -              & -                 \\
\tb{\ours (ours)}          & \tb{-}         & \tb{-}          & -              & \tb{-}            \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transducive few-shot learning comparison with MCT~\cite{mct} using ResNet-12B. *: our reproduction with official code on our datasets.}
\label{tab:trans-mct}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Transductive inference}
\label{sec:trans}

\autoref{tab:trans-pre} compares our method with LR+ICI~\cite{lrici} and PT+MAP~\cite{pt_map} on all four datasets. The truly fair comparison is with our reproductions, indicated by *. We compare our method against the other two using the backbone that each work based its experimental results. Since WRN-28-10 provides more expressive features, we compare our method against~\cite{lrici} by using WRN-28-10 backbone as well. Our method is superior or on par with competitors. The gain over~\cite{lrici} is 1-2\%. most notably 3\% on \emph{mini}ImageNet 1-shot. The gain over PT+MAP~\cite{pt_map} is around 0.5\%. 

Because the gain over~\cite{pt_map} is small, we perform comparison under two additional settings. The first is 10-shot, using more labeled support examples. As shown in \autoref{tab:trans-10shot}, the gain is again around 0.5\%. The second is using more unlabeled queries, that is, 50 queries per class or $M=250$ in total. As shown in \autoref{tab:trans-50q}, the gain now increases to 1-2\%, even 3\% on \emph{mini}ImageNet 1-shot. This can be attributed to the fact that PT+MAP~\cite{pt_map} operates on Euclidean space, while our method captures the manifold structure, which manifests itself in the presence of more data.

\alert{As a robustness test, we compare the two methods by a robustness ablation study, removing completely or using different combinations of the pre-processing part as well as removing the balancing with the raised exponent $\tau$. It can be clearly seen from table \autoref{tab:ab-pt} that our method is much more robust in every experimented scenario. Without this exact processing regime, PT+MAP can be just as bad as random sampling as it can be seen in the 1-shot setting of tieredImageNet. These results highlight the generality of our method as it is much more robust to pre-processing schemes and can be used effective without much deterioration in performance.}

\alert{\autoref{tab:trans-mct} compares our method with MCT~\cite{mct}.}

%------------------------------------------------------------------------------
%\begin{table*}
%\small
%\centering
%\begin{tabular}{lccccccccc}
%\toprule
%\Th{Method}                               & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}  & \mc{2}{\Th{\emph{tiered}ImageNet}} & \mc{2}{\Th{Cifar-FS}}           & \mc{2}{\Th{CUB}}                \\ 
%                                          &              & 1-shot           & 5-shot         & 1-shot         & 5-shot            & 1-shot         & 5-shot         & 1-shot         & 5-shot         \\ \midrule
%PT+MAP (no-pre)~\cite{pt_map}*            & WRN-28-10    & 48.57\ci{0.81}   & 75.67\ci{0.82} & 49.67\ci{0.77} & 88.32\ci{0.50}    & 20.16\ci{0.04} & 20.77\ci{0.08} & 62.99\ci{1.23} & 85.94\ci{0.85} \\
%\tb{\ours (ours, no-pre)}                 & WRN-28-10    & \tb{-}           & \tb{-}         & -              & \tb{-}            & \tb{-}         & \tb{-}         & -              & \tb{-}         \\ \midrule
%PT+MAP (no-sink)~\cite{pt_map}*           & WRN-28-10    & 81.12\ci{0.71}   & 87.66\ci{0.40} & 87.62\ci{0.64} & 91.27\ci{0.40}    & 85.28\ci{0.71} & 89.34\ci{0.47} & 89.89\ci{0.60} & 92.55\ci{0.31} \\
%\tb{\ours (ours)}                         & WRN-28-10    & \tb{-}           & \tb{-}         & -              & \tb{-}            & \tb{-}         & \tb{-}         & -              & \tb{-}         \\ \midrule
%PT+MAP (no-sink/no-$\tau$)~\cite{pt_map}* & WRN-28-10    & 70.09\ci{0.61}   & 83.89\ci{0.41} & 78.48\ci{0.63} & 89.25\ci{0.42}    & 77.27+0.63     & 87.68\ci{0.48} & 82.97\ci{0.59} & 91.45\ci{0.35} \\
%\tb{\ours (ours, no-bal/no-$\tau$)}       & WRN-28-10    & \tb{-}           & \tb{-}         & -              & \tb{-}            & \tb{-}         & \tb{-}         & -              & \tb{-}         \\
%\bottomrule
%\end{tabular}
%\vspace{6pt}
%\caption{Ablation on robustness of our algorithm in comparison to the best state-of-the-Art method}
%\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{4.5pt}
\begin{tabular}{lcccccccccc}
\toprule
\Th{Method}            & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                & \mc{2}{\Th{CUB}}                \\ 
                       &              &            & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot         & 5-shot              & 1-shot              & 5-shot    \\ \midrule
LR+ICI~\cite{lrici}    & ResNet-12A   & 30/50      & 69.66\cip           & 80.11\cip           & 84.01\cip           & 89.00\cip           & 76.51\cip      & 84.32\cip           & 89.58\cip           & 92.48\cip \\
LR+ICI~\cite{lrici}*   & ResNet-12A   & 30/50      & 67.64\ci{0.95}      & 80.00\ci{0.55}      & 83.20\ci{0.89}      & 89.15\ci{0.48}      & 76.57\ci{0.96} & 84.11\ci{0.60}      & 88.36\ci{0.71}      & -         \\
\tb{\ours (ours)}      & ResNet-12A   & 30/50      & \tb{70.67}\ci{0.98} & \tb{81.48}\ci{0.53} & 83.49\ci{0.80}      & 88.65\ci{0.45}      & 76.46\ci{0.88} & \tb{85.06}\ci{0.56} & \tb{89.92}\ci{0.63} & -         \\ 
\tb{\ours$\dagger$}    & ResNet-12A   & 30/50      & \tb{72.36}\ci{0.93} & \tb{81.23}\ci{0.51} & \tb{84.34}\ci{0.77} & \tb{89.66}\ci{0.49} & -              & -                   & -                   & -         \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised inductive few-shot learning methods comparison with same pre-trained backbones. * represents our re-implementation based on the original code and our datasets, $\dagger$ represents unormalized features}
\label{tab:semi_pre}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Semi-supervised learning}
We compare our method against ~\cite{lrici} in the semi-supervised few-shot learning scenario. As it can be seen from table \autoref{tab:semi_pre} our method is superior in all investigated settings from ~\cite{lrici} by even wider margin than from the transductive setting highlighted by the ~4.5\% difference in \emph{mini}ImageNet. 
\label{sec:semi}

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lcccccc}
\toprule
\Th{Method}                             & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}     & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ 
                                        &              &            & 1-shot         & 5-shot              & 1-shot         & 5-shot            \\ \midrule
%TPN$_{SSL}$\cite{tpn}                  & CONV-4       & 20/20      & 52.78          & 66.42               & 55.74          & 71.01             \\
%k-means$_{masked, soft}$~\cite{ssmeta} & CONV-4       & 20/20      & 50.41          & 64.39               & -              & -                 \\
%\tb{\ours (ours)}                      & CONV-4       & 20/20      &                &                     &                &                   \\ \midrule
LST~\cite{learning2selftrain}           & ResNet-12    & 30/50      & 70.10\ci{1.90} & 78.70\ci{0.80}      & 77.70\ci{1.60} & 85.20\ci{0.80}    \\
LR+ICI~\cite{lrici}                     & ResNet-12A   & 30/50      & 69.66\cip      & 80.11\cip           & 84.01\cip      & 89.00\cip         \\
MCT (instance)~\cite{mct}               & ResNet-12B   & 30/50      & 73.80\ci{0.70} & 84.40\ci{0.50}      & 76.90\ci{0.70} & 86.30\ci{0.50}    \\
\tb{\ours (ours)}                       & ResNet-12A   & 30/50      &                &                     &                &                   \\ \midrule
%LR+ICI~\cite{lrici}                    & ResNet-12    & 80/80      & 71.41          & 81.12               & 85.44          & 89.12             \\
%\tb{\ours (ours)}                      & ResNet-12    & 80/80      &                &                     &                &                   \\ \midrule
*k-means$_{masked, soft}$~\cite{ssmeta} & WRN-28-10    & 100/100    & 52.35\ci{0.89} & 67.67\ci{0.65}      & -              & -                 \\
TransMatch~\cite{transmatch}            & WRN-28-10    & 100/100    & 63.02\ci{1.07} & 81.06\ci{0.59}      & -              & -                 \\
\tb{\ours (ours)}                       & WRN-28-10    & 100/100    & 83.98\ci{0.78} & \tb{87.73}\ci{0.37} &   -            &  -                \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised inductive few-shot learning methods comparison. *Re-implemented~\cite{transmatch}}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}                             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}         & \mc{2}{\Th{\emph{tiered}ImageNet}}       & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                                        &              & 1-shot              & 5-shot             & 1-shot              & 5-shot             & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
LR+ICI~\cite{lrici}                     & ResNet-12A   & 66.80\cip           & 79.26\cip          & 80.79\cip           & 87.92\cip          & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
LR+ICI~\cite{lrici}*                    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}     & 82.40\ci{0.84}      & 88.80\ci{0.50}     & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
CAN+Top-\emph{k}~\cite{crossattention}  & ResNet-12    & 67.19\ci{0.55}      & 80.64\ci{0.35}     & 73.21\ci{0.58}      & 84.93 \ci{0.38}    & -                   & -                   & -                   & -                   \\
DPGN~\cite{DPGN}                        & ResNet-12    & 67.77\ci{0.32}      & 84.60\ci{0.43}     & 72.45\ci{0.51}      & 87.24\ci{0.39}     & 77.90\ci{0.50}      & 90.20\ci{0.40}      & 75.71\ci{0.47}      & 91.48\ci{0.33}      \\
EP~\cite{embeddingpropagation}          & ResNet-12    & 66.50\ci{0.89}      & 81.06\ci{0.60}     & 76.53\ci{0.87}      & 87.32\ci{0.64}     & -                   & -                   & -                   & -                   \\
MCT (Instance)~\cite{mct}               & ResNet-12B   & 78.55\ci{0.86}      & 86.03\ci{0.42}     & 82.32\ci{0.81}      & 87.36\ci{0.50}     & 85.61\ci{0.69}      & 90.03\ci{0.46}      & -                   & -                   \\
MCT (Pair)~\cite{mct}                   & ResNet-12B   & 76.16\ci{0.89}      & 85.22\ci{0.42}     & 80.68\ci{0.89}      & 86.63\ci{0.89}     & 87.28\ci{0.70}      & 90.50\ci{0.43}      & -                   & -                   \\
\tb{\ours (ours)}                       & ResNet-12A   & \tb{69.79}\ci{0.99} &\tb{79.58}\ci{0.55} & \tb{83.49}\ci{0.88} &\tb{89.48}\ci{0.47} & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\ \midrule
PT+MAP~\cite{pt_map}                    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}     & -                   & -                  & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
PT+MAP~\cite{pt_map}*                   & WRN-28-10    & 82.88\ci{0.73}      & 88.78\ci{0.40}     & 88.15\ci{0.71}      & 92.32\ci{0.40}     & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
Fine-tuning~\cite{baseline_ft}          & WRN-28-10    & 65.73\ci{0.68}      & 78.40\ci{0.52}     & 73.34\ci{0.71}      & 85.50\ci{0.50}     & 76.58\ci{0.68}      & 85.79\ci{0.50}      & -                   & -                   \\
EP~\cite{embeddingpropagation}          & WRN-28-10    & 70.74\ci{0.85}      & 84.34\ci{0.53}     & 78.50\ci{0.91}      & 88.36\ci{0.57}     & -                   & -                   & -                   & -                   \\
SIB~\cite{SIB}                          & WRN-28-10    & 70.00\ci{0.60}      & 79.20\ci{0.40}     & 72.90$\dagger$      & 82.80$\dagger$     & 80.00\ci{0.60}      & 85.3\ci{0.40}       & -                   & -                   \\
DPGN~\cite{DPGN}                        & WRN-28-10    & 67.24\ci{0.51}      & 83.72\ci{0.44}     & -                   & -                  & -                   & -                   & -                   & -                   \\
SIB+E$^3$BM~\cite{ensemblefsl}          & WRN-28-10    & 71.40\ci{0.50}      & 81.20\ci{0.4}      & 75.60\ci{0.6}       & 84.30\ci{0.4}      & -                   & -                   & -                   & -                   \\
\tb{\ours (ours)}                       & WRN-28-10    & \tb{83.43}\ci{0.79}& \tb{89.10}\ci{0.42}   & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78}      & \tb{91.26}\ci{0.46}      & 91.53\ci{0.59}      & \tb{94.27}\ci{0.30} \\ \bottomrule
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive few-shot learning methods comparison with all state-of-the-Art. * represents our re-implementation based on the original code and our datasets, $\dagger$ implementation carried out by~\cite{ensemblefsl}}
\end{table*}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{4.5pt}
\begin{tabular}{lcccccccc}
\toprule
\Th{Method}                     & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                & \mc{2}{\Th{CUB}}                \\ \midrule
\mc{9}   {WRN-28-10} \\\midrule
                                & 1-shot    & 5-shot    & 1-shot    & 5-shot    & 1-shot    & 5-shot    & 1-shot    & 5-shot    \\ \midrule
$\alpha$                        &           &           &           &           &           &           &           &  \\
$K$                             &           &           &           &           &           &           &           & -         \\
$\tau$                          &           &           &           &           &           &           &           & -         \\ 
cleaning max lr                 &           &           &           &           & -         & -         & -         & -         \\ \midrule
\mc{9}   {ResNet-12A} \\\midrule
$\alpha$                        &           &           &           &           &           &           &           &  \\
$K$                             &           &           &           &           &           &           &           & -         \\
$\tau$                          &           &           &           &           &           &           &           & -         \\ 
cleaning max lr                 &           &           &           &           & -         & -         & -         & -         \\ \midrule
\end{tabular}
\vspace{6pt}
\caption{Selected hyper-parameters}
\label{tab:semi_pre}
\end{table*}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------

\subsection{Comparison with the state of the art}
\label{sec:soa}



==> tex/experiments-4.tex <==
\section{Experiments}
\label{sec:experiments}

%------------------------------------------------------------------------------
\extdata{fig/data/sample}
%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
%------------------------------------------------------------------------------

% We evaluate and compare our proposed method with the state-of-the-art methods in trasnductive and semi-supervised few-shot learning on the four most commonly used databases, \emph{mini}ImageNet~\cite{ravilstm, matchingNets}, \emph{tiered}ImageNet~\cite{ssmeta}, \emph{cifar-FS} and \emph{CUB}. 

%------------------------------------------------------------------------------

\subsection{Datasets}
\label{sec:data}

\paragraph{\emph{mini}ImageNet}

This is a widely used few-shot image classification dataset~\cite{matchingNets, ravilstm}. It contains 100 randomly sampled classes from ImageNet~\cite{imagenet}. These 100 classes are split into 64 training (base) classes, 16 validation (novel) classes and 20 test (novel) classes. Each class contains 600 examples (images). We follow the commonly used split proposed in~\cite{ravilstm}. All images are resized to $84 \times 84$.

\paragraph{\emph{tiered}ImageNet}

This dataset is also sampled from the ImageNet~\cite{imagenet}. However, rather than randomly sampling classes as in \emph{mini}ImageNet, it follows a hierarchical structure where the sampled classes are partitioned into 34 categories, which are organized into 20 training, 6 validation and 8 test categories, containing 351, 97 and 160 classes, respectively. This hierarchical partitioning strategy ensures that the training classes are semantically distinct from the test classes, making it a more realistic few-shot classification problem. We follow the commonly used split proposed in~\cite{sslmeta}. Again, all images are resized to $84 \times 84$.

\paragraph{CUB}

This is a fine-grained classification dataset consisting of 200 classes, each corresponding to a bird species. We follow the split defined by~\cite{closerlook, fewshotCUB}, with 100 training, 50 validation and 50 test classes. To compare fairly with competitors, we \emph{use} bounding boxes on ResNet features following~\cite{fewshotCUBbounding} to compare with~\cite{lrici} but we \emph{do not use} bounding boxes on WRN features to compare with~\cite{pt_map}.

\paragraph{CIFAR-FS}

This dataset is derived from CIFAR-100~\cite{cifar100db}, consisting of 100 classes with 600 examples per class. We follow the split provided by~\cite{closerlook}, with 64 training, 16 validation and 20 test classes. To compare fairly with competitors, we use the original image resolution of $32 \times 32$ on WRN features to compare with~\cite{pt_map} but we resize images to $84 \times 84$ on ResNet features to compare with~\cite{lrici}.

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{tabular}{lcccccccc}
\toprule
\Th{Param} & \mc{2}{\Th{\emph{m}IN}} & \mc{2}{\Th{\emph{t}IN}} & \mc{2}{\Th{CFS}} & \mc{2}{\Th{CUB}} \\ \midrule
$K$ (shot)        & 1   & 5   & 1   & 5   & 1   & 5   & 1   & 5   \\ \midrule
\mc{9}{ResNet-12A}                                                \\ \midrule
$k$~\eq{affinity} & 15  & 25  & 15  & 15  & 15  & 15  & 15  & 8   \\ 
$\alpha$~\eq{lp}  & 0.8 & 0.4 & 0.5 & 0.2 & 0.8 & 0.4 & 0.2 & 0.6 \\ \midrule
\mc{9}{WRN-28-10}                                                 \\ \midrule
$k$~\eq{affinity} & 20  & 30  & 20  & 20  & 20  & 25  & 20  & 25  \\ 
$\alpha$~\eq{lp}  & 0.8 & 0.2 & 0.8 & 0.8 & 0.4 & 0.5 & 0.5 & 0.8 \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Selected hyper-parameters. \emph{m}IN: \emph{mini}ImageNet. \emph{t}IN: \emph{tiered}ImageNet. CFS: CIFAR-FS.}
\label{tab:param}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lcccccccccc}
\toprule
\Th{Inference}          & \mc{5}{\Th{Components}}            & \mc{2}{\Th{ResNet-12}}             & \mc{2}{\Th{WRN-28-10}}             \\ 
                        & \lp & \bal & \ilc & \iprob & \cp & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
Inductive               &     &      &      &        &     & 56.30\ci{0.62}      & 75.59\ci{0.47}      & 60.04\ci{0.64}      & 81.35\ci{0.43}      \\ 
Transductive            & \ch &      &      &        &     & 61.09\ci{0.70}      & 75.32\ci{0.50}      & 74.35\ci{0.68}      & 84.84\cim           \\ 
Transductive            & \ch & \ch  &      &        &     & 65.04\ci{0.75}      & 76.82\ci{0.50}      & 79.21\ci{0.72}      & 88.00\ci{0.41}      \\ 
Transductive$\dagger$   & \ch & \ch  & \ch  &        &     & \tb{69.79}\ci{0.99} & \tb{79.58}\ci{0.55} & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} \\ 
Transductive            & \ch & \ch  &      & \ch    &     & 58.27\ci{0.91}      & 74.11\ci{0.56}      & 72.28\ci{0.90}          & 85.88\ci{0.46}      \\ 
Transductive            &     & \ch  & \ch  &        & \ch & -                   & -                   & -                   & -                   \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Ablation study of algorithmic components of our method on \emph{mini}ImageNet. Inductive: baseline using only support examples. \lp: label propagation. \bal: class balancing~\eq{balance}. \ilc: iterative label cleaning, without which we just output predictions~\eq{argmax}. \iprob: iterative selection of top examples per class directly as column-wise maxima of $P$~\eq{sub} instead of \ilc. \cp: linear classifier used for prediction instead of \lp, as in~\cite{lrici}, with balancing still applied on output probabilities. $\dagger$: default setting of \ours.}
\label{tab:ab-comp}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{figure}
\input{fig/hist/distributions}
\caption{(a,b) Distributions of loss values~\eq{loss} for correctly and incorrectly labeled examples, normalized independently. Uniform label noise: (a) 20\%, (b) 40\%. Pseudo-labels predicted by label propagation and balancing~\eq{argmax} for two different tasks (c,d).}
\label{fig:hist}
\end{figure}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot       & 5-shot                     \\ \midrule
LR+ICI~\cite{lrici}     & ResNet-12A   & 66.80\cip           & 79.26\cip           & 80.79\cip           & 87.92\cip           & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
LR+ICI~\cite{lrici}*    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
\tb{\ours (ours)}       & ResNet-12A   & \tb{69.79}\ci{0.99} & \tb{79.58}\ci{0.55} & \tb{83.49}\ci{0.88} & \tb{89.48}\ci{0.47} & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\ \midrule
PT+MAP~\cite{pt_map}    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}      & -                   & -                   & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
PT+MAP~\cite{pt_map}*   & WRN-28-10    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
LR+ICI~\cite{lrici}*    & WRN-28-10    & 80.61\ci{0.80}      & 87.93\ci{0.44}      & 86.79\ci{0.76}      & 91.73\ci{0.40}      & 84.88\ci{0.79}      &  89.75\ci{0.48}     & 90.18\ci{0.65}      & 93.35\ci{0.30}      \\
\tb{\ours (ours)}       & WRN-28-10    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78} & \tb{91.26}\ci{0.46} & \tb{91.53}\ci{0.59} & \tb{94.27}\ci{0.30} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive inference, comparison with LR+ICI~\cite{lrici} and PT+MAP~\cite{pt_map}. *: our reproduction with official code on our datasets.}
\label{tab:trans-pre}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}          & \mc{2}{\Th{Cifar-FS}}                     \\ 
                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot                & 1-shot              & 5-shot              \\ \midrule
PT+MAP~\cite{pt_map}*   & WRN-28-10    & 83.79\ci{0.71}      & 88.94\ci{0.33}      & 88.87\ci{0.64}      & 92.01\ci{0.36}        & 87.63\ci{0.66}      & 90.15\ci{0.46}      \\
\tb{\ours (ours)}       & WRN-28-10    & \tb{86.30}\ci{0.71} & \tb{89.99}\ci{0.32} & \tb{90.60}\ci{0.64} &\tb{92.97}\ci{0.38}    & \tb{88.51}\ci{0.69} & \tb{91.23}\ci{0.44} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive inference, 50 queries per class. *: our reproduction with official code on our datasets.}
\label{tab:trans-50q}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength\tabcolsep{2pt}
\begin{tabular}{lccccc}
\toprule
\Th{Method}             & \Th{Pre} & \mc{2}{\emph{mini}ImageNet}               & \mc{2}{\emph{tiered}ImageNet}             \\ 
                        &          & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
PT+MAP~\cite{pt_map}*   &          & 48.57\ci{0.81}      & 75.67\ci{0.82}      & 49.67\ci{0.77}      & 88.32\ci{0.50}      \\ 
\tb{\ours (ours)}       &          & 78.89\ci{0.90}      & 86.80\ci{0.46}      & 86.52\ci{0.47}      & 91.07\ci{0.47}      \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch      & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      \\
\tb{\ours (ours)}       & \ch      & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive inference, ablation of PT+MAP~\cite{pt_map} pre-processing. \Th{PRE}: power transform, normalization, centering. *: our reproduction with official code on our datasets.}
\label{tab:ab-pt}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength\tabcolsep{1.5pt}
\begin{tabular}{lccccc}
\toprule
\Th{Method}                             & \mc{2}{\Th{\emph{mini}ImageNet}} & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ \midrule 
                                        & 1-shot         & 5-shot          & 1-shot         & 5-shot            \\ \midrule
MCT (instance)~\cite{mct}               & 78.55\ci{0.86} & 86.03\ci{0.42}  & 82.32\ci{0.81} & 87.36\ci{0.50}    \\
MCT (instance)~\cite{mct}*              & 77.10\ci{0.88} & 86.19\ci{0.40}  &                & -                 \\
\tb{\ours (ours)}                       & \tb{-}         & \tb{-}          & -              & \tb{-}            \\ \midrule
MCT (instance)~\cite{mct}*$\dagger$     & 67.39\ci{0.62} & 81.93\ci{0.45}  & -              & -                 \\
\tb{\ours (ours)}                       & \tb{-}         & \tb{-}          & -              & \tb{-}            \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive inference, comparison with MCT~\cite{mct} using ResNet-12B. *: our reproduction with official code on our datasets. $\dagger$: no scaling.}
\label{tab:trans-mct}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Setup}
\label{sec:setup}

\paragraph{Tasks}

We consider $N$-way, $K$-shot classification tasks with $N = 5$ randomly sampled novel classes and $K \in \{1, 5\}$ randomly selected examples per class for support set $S$, that is, $L = 5K$ examples in total. For the query set $Q$, we randomly sample $15$ additional examples per class, that is, $M = 75$ examples in total, which is the most common choice in transductive and semi-supervised few shot learning~\cite{tpn, learning2selftrain, transmatch}. 

In the semi-supervised setting, the unlabeled set $U$ contains an additional number of randomly sampled examples per novel class. This number depends on $K$. We use two settings, namely 30/50 and 100/100, where the first number (30 or 100) refers to 1-shot and the second (50 or 100) to 5-shot. Again, these are the two most common choices in semi-supervised few shot learning~\cite{learning2selftrain,lrici,mct,ssmeta,transmatch}.

Unless otherwise stated, we use 1000 tasks and report mean accuracy and 95\% confidence interval on the test set.

\paragraph{Competitors}

As discussed in the supplementary material, there are number of flaws in experimental evaluation in the bibliography, including the use of different networks, different training settings, different versions of datasets, different dimenionalities and pre-processing of features. As a result, it is impossible to provide fair comparisons with the state of the art, unless one uses public code to reproduce results under exactly the same setup.

In this work, we do provide completely fair comparisons with such reproduced results of three state-of-the-art methods: LR+ICI~\cite{lrici}, PT+MAP~\cite{pt_map} and MCT~\cite{mct}. To our knowledge, these methods outperform all other state of the art. Importantly, only~\cite{lrici} is published, while the other two are pre-prints. We compare with these methods in \autoref{sec:trans} (transductive) and \autoref{sec:semi} (semi-supervised), then with other state of the art in \autoref{sec:soa}.

\paragraph{Networks}

We use publicly available pre-trained backbone convolutional neural networks that are trained on the base-class training set. We experiment with two popular networks, namely, the residual network ResNet-12~\cite{tadam} and the wide residual network (WRN-28-10)~\cite{LEO}.

In particular, to compare with~\cite{lrici}, we use pre-trained weights of the ResNet-12 provided by~\cite{lrici}, which we call ResNet-12A, as well as official public code\footnote{\url{https://github.com/Yikai-Wang/ICI-FSL}} for testing. To compare with~\cite{pt_map}, we use pre-trained weights of a WRN-28-10 provided by~\cite{manifoldmixup}\footnote{\url{https://github.com/nupurkmr9/S2M2_fewshot}}, which are the same used by~\cite{pt_map}, as well as official public code\footnote{\url{https://github.com/yhu01/PT-MAP}} for testing. To compare with~\cite{mct}, we use official public code\footnote{\url{https://github.com/seongmin-kye/MCT}} to train from scratch another version of ResNet-12 used by~\cite{mct}, which we call ResNet-12B, as well as the same code for testing.

\paragraph{Feature pre-processing}

Each method uses its own feature pre-processing choices. For instance, LR+ICI~\cite{lrici} uses $\ell_2$-normalization and PCA to reduce ResNet-12A to 5 dimensions. PR+MAP~\cite{pt_map} uses element-wise power transform, $\ell_2$-normalization and centering of WRN-28-10 features. MCT~\cite{mct} uses flattening of the output tensor of ResNet-12B rather than global spatial pooling, hence dimensionality is in the thousands. By default, we use the same choices as~\cite{pt_map,mct} for WRN-28-10 and ResNet-12B. For ResNet-12A however, we use $\ell_2$-normalization only on transductive inference and we do not use any dimensionality reduction. We ablate these options in \autoref{sec:trans}.

\paragraph{Implementation details}

We use PyTorch~\cite{pytorch}, FAISS \cite{faiss} and scikit-learn~\cite{sklearn}. Label cleaning is based on a linear classifier on top of embedding $f$, initialized by imprinting the average of support features per class and then trained using~\eq{loss}. We use SGD with momentum 0.9 and weight decay 0.0005. Following~\cite{o2u}, we use a cyclical schedule of 10 cycles with 20 iterations per cycle for the learning rate, which linearly decreases from a maximum $\eta_{\max}$ to zero. For inductive (resp. semi-supervised) learning, we use logistic regression on support (resp. as well as pseudo-labeled) examples, learned using scikit-learn like~\cite{lrici}. The row-wise sum $\vp$~\eq{sink-row} is either fixed to 1 for all examples or set to a weight in $[0,1]$ according to entropy, following~\cite{semilpavrithis}.

%------------------------------------------------------------------------------

\subsection{Ablation study}
\label{sec:ablation}

\paragraph{Hyperparameters}

We optimize hyperparameters on the validation set of every dataset. This includes hyperparameters $\gamma$ and $k$ used in the nearest neighbor graph~\eq{affinity}, $\alpha$ in label propagation~\eq{lp} $\tau$ in balancing~\eq{balance} and the maximum learning rate $\eta_{\max}$ of label cleaning. \autoref{tab:param} shows the choices for $k, \alpha$. We always set $\gamma = 3$, $\tau = 3$ and $\eta_{\max} = 0.1$. More details are given in the supplementary material.

\paragraph{Algorithmic components}

\autoref{tab:ab-comp} ablates the performance of our method in the presence or not of individual components, as well as using alternatives to our components. The use of queries with label propagation immediately gives a gain of transductive over inductive inference, up to 14\% in 1-shot. Balancing and iterative label cleaning each bring another gain of 4-5\%, especially in 1-shot. Iterative label cleaning is very important because selecting examples based on $P$ instead is even worse than baseline transductive inference. Label propagation is also very important because using a linear classifier instead fails too.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{4.5pt}
\begin{tabular}{lcccccccccc}
\toprule
\Th{Method}                & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                & \mc{2}{\Th{CUB}}                \\ 
                           &              &            & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot         & 5-shot              & 1-shot              & 5-shot    \\ \midrule
LR+ICI~\cite{lrici}        & ResNet-12A   & 30/50      & 69.66\cip           & 80.11\cip           & 84.01\cip           & 89.00\cip           & 76.51\cip      & 84.32\cip           & 89.58\cip           & 92.48\cip \\
LR+ICI~\cite{lrici}*       & ResNet-12A   & 30/50      & 67.64\ci{0.95}      & 80.00\ci{0.55}      & 83.20\ci{0.89}      & 89.15\ci{0.48}      & 76.57\ci{0.96} & 84.11\ci{0.60}      & 88.36\ci{0.71}      & -         \\
\tb{\ours (ours)}          & ResNet-12A   & 30/50      & \tb{70.67}\ci{0.98} & \tb{81.48}\ci{0.53} & 83.49\ci{0.80}      & 88.65\ci{0.45}      & 76.46\ci{0.88} & \tb{85.06}\ci{0.56} & \tb{89.92}\ci{0.63} & -         \\ 
\tb{\ours (ours)$\dagger$} & ResNet-12A   & 30/50      & \tb{72.36}\ci{0.93} & \tb{81.23}\ci{0.51} & \tb{84.34}\ci{0.77} & \tb{89.66}\ci{0.49} & -              & -                   & -                   & -         \\ \midrule
PT+MAP~\cite{pt_map}*      & WRN-28-10    & 30/50      & 83.47\ci{0.68}      & 89.15\ci{0.38}      & 88.67\ci{0.68}      & 92.44\ci{0.38}      & -              & -                   & -                   & -         \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised few-shot learning, comparison with LR+ICI~\cite{lrici} and PT+MAP~\cite{pt_map}. *: our reproduction with official code on our datasets.  $\dagger$: un-normalized features}
\label{tab:semi_pre}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}                             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
LR+ICI~\cite{lrici}                     & ResNet-12A   & 66.80\cip           & 79.26\cip           & 80.79\cip           & 87.92\cip           & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
LR+ICI~\cite{lrici}*                    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
CAN+Top-\emph{k}~\cite{crossattention}  & ResNet-12    & 67.19\ci{0.55}      & 80.64\ci{0.35}      & 73.21\ci{0.58}      & 84.93 \ci{0.38}     & -                   & -                   & -                   & -                   \\
DPGN~\cite{DPGN}                        & ResNet-12    & 67.77\ci{0.32}      & 84.60\ci{0.43}      & 72.45\ci{0.51}      & 87.24\ci{0.39}      & 77.90\ci{0.50}      & 90.20\ci{0.40}      & 75.71\ci{0.47}      & 91.48\ci{0.33}      \\
EP~\cite{embeddingpropagation}          & ResNet-12    & 66.50\ci{0.89}      & 81.06\ci{0.60}      & 76.53\ci{0.87}      & 87.32\ci{0.64}      & -                   & -                   & -                   & -                   \\
MCT (Instance)~\cite{mct}               & ResNet-12B   & 78.55\ci{0.86}      & 86.03\ci{0.42}      & 82.32\ci{0.81}      & 87.36\ci{0.50}      & 85.61\ci{0.69}      & 90.03\ci{0.46}      & -                   & -                   \\
MCT (Pair)~\cite{mct}                   & ResNet-12B   & 76.16\ci{0.89}      & 85.22\ci{0.42}      & 80.68\ci{0.89}      & 86.63\ci{0.89}      & 87.28\ci{0.70}      & 90.50\ci{0.43}      & -                   & -                   \\
\tb{\ours (ours)}                       & ResNet-12A   & \tb{69.79}\ci{0.99} &\tb{79.58}\ci{0.55}  & \tb{83.49}\ci{0.88} &\tb{89.48}\ci{0.47}  & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\ \midrule
PT+MAP~\cite{pt_map}                    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}      & -                   & -                   & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
PT+MAP~\cite{pt_map}*                   & WRN-28-10    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
Fine-tuning~\cite{baseline_ft}          & WRN-28-10    & 65.73\ci{0.68}      & 78.40\ci{0.52}      & 73.34\ci{0.71}      & 85.50\ci{0.50}      & 76.58\ci{0.68}      & 85.79\ci{0.50}      & -                   & -                   \\
EP~\cite{embeddingpropagation}          & WRN-28-10    & 70.74\ci{0.85}      & 84.34\ci{0.53}      & 78.50\ci{0.91}      & 88.36\ci{0.57}      & -                   & -                   & -                   & -                   \\
SIB~\cite{SIB}$\dagger$                 & WRN-28-10    & 70.00\ci{0.60}      & 79.20\ci{0.40}      & 72.90\cip           & 82.80\cip           & 80.00\ci{0.60}      & 85.3\ci{0.40}       & -                   & -                   \\
DPGN~\cite{DPGN}                        & WRN-28-10    & 67.24\ci{0.51}      & 83.72\ci{0.44}      & -                   & -                   & -                   & -                   & -                   & -                   \\
SIB+E$^3$BM~\cite{ensemblefsl}          & WRN-28-10    & 71.40\ci{0.50}      & 81.20\ci{0.4}       & 75.60\ci{0.6}       & 84.30\ci{0.4}       & -                   & -                   & -                   & -                   \\
\tb{\ours (ours)}                       & WRN-28-10    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78} & \tb{91.26}\ci{0.46} & 91.53\ci{0.59}      & \tb{94.27}\ci{0.30} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive few-shot learning state of the art. *: our reproduction with official code on our datasets. $\dagger$: \emph{tiered}ImageNet results as reported by~\cite{ensemblefsl}}
\label{tab:SOTA}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lcccccc}
\toprule
\Th{Method}                                        & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}     & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ 
                                                   &              &            & 1-shot         & 5-shot              & 1-shot         & 5-shot            \\ \midrule
%TPN$_{SSL}$\cite{tpn}                             & CONV-4       & 20/20      & 52.78          & 66.42               & 55.74          & 71.01             \\
%$k$-means$_{\masked,\soft}$~\cite{ssmeta}         & CONV-4       & 20/20      & 50.41          & 64.39               & -              & -                 \\
%\tb{\ours (ours)}                                 & CONV-4       & 20/20      &                &                     &                &                   \\ \midrule
LST~\cite{learning2selftrain}                      & ResNet-12    & 30/50      & 70.10\ci{1.90} & 78.70\ci{0.80}      & 77.70\ci{1.60} & 85.20\ci{0.80}    \\
LR+ICI~\cite{lrici}                                & ResNet-12A   & 30/50      & 69.66\cip      & 80.11\cip           & 84.01\cip      & 89.00\cip         \\
MCT (instance)~\cite{mct}                          & ResNet-12B   & 30/50      & 73.80\ci{0.70} & 84.40\ci{0.50}      & 76.90\ci{0.70} & 86.30\ci{0.50}    \\
\tb{\ours (ours)}                                  & ResNet-12A   & 30/50      &                &                     &                &                   \\ \midrule
%LR+ICI~\cite{lrici}                               & ResNet-12    & 80/80      & 71.41          & 81.12               & 85.44          & 89.12             \\
%\tb{\ours (ours)}                                 & ResNet-12    & 80/80      &                &                     &                &                   \\ \midrule
$k$-means$_{\masked,\soft}$~\cite{ssmeta}$\dagger$ & WRN-28-10    & 100/100    & 52.35\ci{0.89} & 67.67\ci{0.65}      & -              & -                 \\
TransMatch~\cite{transmatch}                       & WRN-28-10    & 100/100    & 63.02\ci{1.07} & 81.06\ci{0.59}      & -              & -                 \\
\tb{\ours (ours)}                                  & WRN-28-10    & 100/100    & 83.98\ci{0.78} & \tb{87.73}\ci{0.37} &   -            &  -                \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised few-shot learning state of the art. $\dagger$: as reported by~\cite{transmatch}}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Label cleaning: loss distribution}
\label{sec:hist}

To illustrate the effectiveness of our label cleaning, we conduct two experiments, showing the distribution of the loss value~\eq{loss} for correctly and incorrectly labeled examples. In the first experiment, shown in \autoref{fig:hist}(a,b), we collect 500 correctly labeled examples and inject label noise uniformly at random to the 20\%~(a) and 40\%~(b) of the data. The correctly and incorrectly labeled examples have very different loss distributions. Importantly, while previous work on label cleaning~\cite{ArazoOAOM19,o2u,robustonfly} attempts to detect clean examples by applying an optimal threshold on the loss value, we only need to find few clean examples at each iteration. The examples with minimal loss value are clean.

The second experiment is on two novel \alert{5-way 5-shot} tasks in the transductive setting, shown in \autoref{fig:hist}(c,d). We use 50 additional unlabeled novel-class queries in each task and we predict pseudo-labels using label propagation and balancing, according to~\eq{argmax}. In this case, label cleaning is more challenging because the two distributions are more overlapping. This is natural because predictions are more informed than uniform, even if incorrect. Still, a large proportion of clean examples have less loss than the minimal value of noisy ones.

%------------------------------------------------------------------------------

\subsection{Transductive inference}
\label{sec:trans}

\autoref{tab:trans-pre} compares our \ours with LR+ICI~\cite{lrici} and PT+MAP~\cite{pt_map} on all four datasets. The truly fair comparison is with our reproductions, indicated by *. Apart from the default networks, we also use WRN-28-10 with LR+ICI~\cite{lrici}, since it is more powerful. Our \ours is superior or on par with competitors. The gain over~\cite{lrici} is 1-2\%. most notably 3\% on \emph{mini}ImageNet 1-shot. The gain over PT+MAP~\cite{pt_map} is around 0.5\%. 

Because the gain over~\cite{pt_map} is small, we also experiment with 50 unlabeled queries per class, or $M=250$ in total. As shown in \autoref{tab:trans-50q}, the gain now increases to 1-2\%, even 3\% on \emph{mini}ImageNet 1-shot. This can be attributed to the fact that PT+MAP~\cite{pt_map} operates on Euclidean space, while our method captures the manifold structure, which manifests itself in the presence of more data. An experiment on 10-shot is also included in the supplementary material. 

\autoref{tab:ab-pt} shows that PT+MAP~\cite{pt_map} is very sensitive to feature pre-processing, losing up to 30\% or 40\% in the absence of its default settings, while our \ours more robust, losing only up to 5\%.

\alert{\autoref{tab:trans-mct} compares our \ours with MCT~\cite{mct}.}

%------------------------------------------------------------------------------

\subsection{Semi-supervised learning}
\label{sec:semi}

We compare our \ours against ~\cite{lrici} \alert{and ~\cite{pt_map}}in the semi-supervised few-shot learning scenario. As it can be seen from table \autoref{tab:semi_pre}, \ours is superior in all investigated settings from ~\cite{lrici} by even wider margin than from the transductive setting highlighted by the ~4.5\% difference in \emph{mini}ImageNet. This can be be attributed to both the use of the manifold structure of the data through label propagation as well as through the use of our label cleaning module. \alert{We adapt the same semi-supervised few-shot learning setting to ~\cite{pt_map} and use the WRN-28-10 backbone as it was the main backbone used in ~\cite{pt_map}. Again we can see the generality and superiority of our method in the semisupervised setting as it also outperforms \cite{pt_map} by a respectable margin.}

%------------------------------------------------------------------------------

\subsection{Comparison with the state of the art}
\label{sec:soa}
We acknowledge that making completely objective comparisons to every state-of-the-Art method that tackles the transductive and semi-supervised few-shot learning problem. Despite these technical difficulties we can still claim, to the best of our knowledge, that our method surpasses current state-of-the-Art results and is the current state-of-the-Art method in the four benchmark datasets when compared against the best versions of every other method regardless of training regime or backbone architecture. Our results and our competitors can be seen analytically in tables \autoref{tab:SOTA} and \autoref{tab:SOTA_semi}. We chose the model of each competitor that achieves the best results in the benchmark datasets regardless of training regime and backbone. 




==> tex/experiments-5.tex <==
\section{Experiments}
\label{sec:experiments}

%------------------------------------------------------------------------------
\extdata{fig/data/sample}
%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
%------------------------------------------------------------------------------

% We evaluate and compare our proposed method with the state-of-the-art methods in trasnductive and semi-supervised few-shot learning on the four most commonly used databases, \emph{mini}ImageNet~\cite{ravilstm, matchingNets}, \emph{tiered}ImageNet~\cite{ssmeta}, \emph{cifar-FS} and \emph{CUB}. 

%------------------------------------------------------------------------------

\subsection{Datasets}
\label{sec:data}

\paragraph{\emph{mini}ImageNet}

This is a widely used few-shot image classification dataset~\cite{matchingNets, ravilstm}. It contains 100 randomly sampled classes from ImageNet~\cite{imagenet}. These 100 classes are split into 64 training (base) classes, 16 validation (novel) classes and 20 test (novel) classes. Each class contains 600 examples (images). We follow the commonly used split proposed in~\cite{ravilstm}. All images are resized to $84 \times 84$.

\paragraph{\emph{tiered}ImageNet}

This is also sampled from ImageNet~\cite{imagenet} but has a hierarchical structure. Classes are partitioned into 34 categories, organized into 20 training, 6 validation and 8 test categories, containing 351, 97 and 160 classes, respectively. This ensures that training classes are semantically distinct from test classes, which is more realistic. We follow the common split of~\cite{sslmeta}. Again, all images are $84 \times 84$.

\paragraph{CUB}

This is a fine-grained classification dataset consisting of 200 classes, each corresponding to a bird species. We follow the split defined by~\cite{closerlook, fewshotCUB}, with 100 training, 50 validation and 50 test classes. To compare fairly with competitors, we \emph{use} bounding boxes on ResNet features following~\cite{fewshotCUBbounding} to compare with~\cite{lrici} but we \emph{do not use} bounding boxes on WRN~\cite{LEO} features to compare with~\cite{pt_map}.

\paragraph{CIFAR-FS}

This dataset is derived from CIFAR-100~\cite{cifar100db}, consisting of 100 classes with 600 examples per class. We follow the split provided by~\cite{closerlook}, with 64 training, 16 validation and 20 test classes. To compare fairly with competitors, we use the original image resolution of $32 \times 32$ on WRN features to compare with~\cite{pt_map} but we resize images to $84 \times 84$ on ResNet features to compare with~\cite{lrici}.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lcccccccccc}
\toprule
\Th{Inference}          & \mc{5}{\Th{Components}}            & \mc{2}{\Th{ResNet-12}}             & \mc{2}{\Th{WRN-28-10}}             \\ 
                        & \lp & \bal & \ilc & \iprob & \cp & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
Inductive               &     &      &      &        &     & 56.30\ci{0.62}      & 75.59\ci{0.47}      & 60.04\ci{0.64}      & 81.35\ci{0.43}      \\ 
Transductive            & \ch &      &      &        &     & 61.09\ci{0.70}      & 75.32\ci{0.50}      & 74.35\ci{0.68}      & 84.76 \ci{0.42}          \\ 
Transductive            & \ch & \ch  &      &        &     & 65.04\ci{0.75}      & 76.82\ci{0.50}      & 79.21\ci{0.72}      & 88.00\ci{0.41}      \\ 
Transductive$\dagger$   & \ch & \ch  & \ch  &        &     & \tb{69.79}\ci{0.99} & \tb{79.58}\ci{0.55} & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} \\ 
Transductive            & \ch & \ch  &      & \ch    &     & 58.27\ci{0.91}      & 74.11\ci{0.56}      & 72.28\ci{0.90}      & 85.88\ci{0.46}      \\ 
Transductive            &     & \ch  & \ch  &        & \ch &                     &                     & 82.01\ci{0.85}      &                     \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Ablation study of algorithmic components of our method \ours on \emph{mini}ImageNet. Inductive: baseline using only support examples. \lp: label propagation. \bal: class balancing~\eq{balance}. \ilc: iterative label cleaning, without which we just output predictions~\eq{argmax}. \iprob: iterative selection of top examples per class directly as column-wise maxima of $P$~\eq{sub} instead of \ilc. \cp: linear classifier used for prediction instead of \lp, as in~\cite{lrici}, with balancing still applied on output probabilities. $\dagger$: default setting of \ours.}
\label{tab:ab-comp}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{figure}
\input{fig/hist/distributions}
\caption{(a,b) Distributions of loss values~\eq{loss} for correctly and incorrectly labeled examples, normalized independently. Uniform label noise: (a) 20\%, (b) 40\%. Pseudo-labels predicted by~\eq{argmax} for two different 1-shot transductive \emph{mini}ImageNet tasks (c,d).}
\label{fig:hist}
\end{figure}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot       & 5-shot                     \\ \midrule
LR+ICI~\cite{lrici}     & ResNet-12A   & 66.80\cip           & 79.26\cip           & 80.79\cip           & 87.92\cip           & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
LR+ICI~\cite{lrici}*    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
\tb{\ours (ours)}       & ResNet-12A   & \tb{69.79}\ci{0.99} & \tb{79.58}\ci{0.55} & \tb{83.49}\ci{0.88} & \tb{89.48}\ci{0.47} & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\ \midrule
PT+MAP~\cite{pt_map}    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}      & -                   & -                   & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
PT+MAP~\cite{pt_map}*   & WRN-28-10    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
LR+ICI~\cite{lrici}*    & WRN-28-10    & 80.61\ci{0.80}      & 87.93\ci{0.44}      & 86.79\ci{0.76}      & 91.73\ci{0.40}      & 84.88\ci{0.79}      &  89.75\ci{0.48}     & 90.18\ci{0.65}      & 93.35\ci{0.30}      \\
\tb{\ours (ours)}       & WRN-28-10    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78} & \tb{91.26}\ci{0.46} & \tb{91.53}\ci{0.59} & \tb{94.27}\ci{0.30} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive inference, comparison with LR+ICI~\cite{lrici} and PT+MAP~\cite{pt_map}. *: our reproduction with official code on our datasets.}
\label{tab:trans-pre}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{tabular}{lccccccc}
\toprule
\Th{Method}             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}          & \mc{2}{\Th{Cifar-FS}}                     \\ 
                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot                & 1-shot              & 5-shot              \\ \midrule
PT+MAP~\cite{pt_map}*   & WRN-28-10    & 83.79\ci{0.71}      & 88.94\ci{0.33}      & 88.87\ci{0.64}      & 92.01\ci{0.36}        & 87.63\ci{0.66}      & 90.15\ci{0.46}      \\
\tb{\ours (ours)}       & WRN-28-10    & \tb{86.30}\ci{0.71} & \tb{89.99}\ci{0.32} & \tb{90.60}\ci{0.64} &\tb{92.97}\ci{0.38}    & \tb{88.51}\ci{0.69} & \tb{91.23}\ci{0.44} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive inference, 50 queries per class. *: our reproduction with official code on our datasets.}
\label{tab:trans-50q}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength\tabcolsep{2pt}
\begin{tabular}{lccccc}
\toprule
\Th{Method}             & \Th{Pre} & \mc{2}{\emph{mini}ImageNet}               & \mc{2}{\emph{tiered}ImageNet}             \\ 
                        &          & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
PT+MAP~\cite{pt_map}*   &          & 48.57\ci{0.81}      & 75.67\ci{0.82}      & 49.67\ci{0.77}      & 88.32\ci{0.50}      \\ 
\tb{\ours (ours)}       &          & 78.89\ci{0.90}      & 86.80\ci{0.46}      & 86.52\ci{0.47}      & 91.07\ci{0.47}      \\ \midrule
PT+MAP~\cite{pt_map}*   & \ch      & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      \\
\tb{\ours (ours)}       & \ch      & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive inference, ablation over PT+MAP~\cite{pt_map} pre-processing. \Th{PRE}: power transform, normalization, centering. *: our reproduction with official code on our datasets.}
\label{tab:ab-pt}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{figure}
\extfig{pca}
{
\begin{tikzpicture}
\begin{axis}[
	width=\linewidth,
	height=0.5\linewidth,
	font=\small,
	xlabel={dimensions},
	ylabel={mean accuracy},
	legend pos={south west},
]
\addplot[blue] table[x=d,y=ours] \pcadims; \leg{\ours (ours)}
\addplot[red]  table[x=d,y=ici]  \pcadims; \leg{LR+ICI}
\end{axis}
\end{tikzpicture}
}
\caption{1-shot trasductive inference on \emph{mini}ImageNet, ablation over LR+ICI~\cite{lrici} pre-processing: dimension reduction by PCA.}
\label{fig:pca}
\end{figure}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength\tabcolsep{1pt}
\begin{tabular}{lccccc}
\toprule
\Th{Method}                             & \mc{2}{\Th{\emph{mini}ImageNet}} & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ \midrule 
                                        & 1-shot         & 5-shot          & 1-shot         & 5-shot            \\ \midrule
MCT (instance,flip)~\cite{mct}          & 78.55\ci{0.86} & 86.03\ci{0.42}  & 82.32\ci{0.81} & 87.36\ci{0.50}    \\
MCT (instance)~\cite{mct}*              & 76.83\ci{0.85} & 85.36\ci{0.44}  &                &                   \\
\tb{\ours (ours)}                       & 75.63\ci{0.87}      & 81.42\ci{0.53}       &                &                   \\ \midrule
MCT (no scale)~\cite{mct}*$\dagger$     & 67.26\ci{0.60} & 81.90\ci{0.43}  &                &                   \\
\tb{\ours (ours)}                       & 75.58\ci{1.16} & 81.58\ci{0.50}  &                &                   \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive inference, comparison with MCT~\cite{mct} using ResNet-12B. *: our reproduction with official code on our datasets. $\dagger$: no scaling.}
\label{tab:trans-mct}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Setup}
\label{sec:setup}

\paragraph{Tasks}

We consider $N$-way, $K$-shot classification tasks with $N = 5$ randomly sampled novel classes and $K \in \{1, 5\}$ randomly selected examples per class for support set $S$, that is, $L = 5K$ examples in total. For the query set $Q$, we randomly sample $15$ additional examples per class, that is, $M = 75$ examples in total, which is the most common choice in the literature~\cite{tpn, learning2selftrain, transmatch}. 

In the semi-supervised setting, the unlabeled set $U$ contains an additional number of randomly sampled examples per novel class. This number depends on $K$. We use two settings, namely 30/50 and 100/100, where the first number (30 or 100) refers to 1-shot and the second (50 or 100) to 5-shot. Again, these are the two most common choices in semi-supervised few shot learning~\cite{learning2selftrain,lrici,mct,ssmeta,transmatch}.

Unless otherwise stated, we use 1000 tasks and report mean accuracy and 95\% confidence interval on the test set.

\paragraph{Competitors}

As discussed in the supplementary material, there are several flaws in experimental evaluation in the literature, like the use of different networks, training, versions of datasets, dimensionality and feature pre-processing. Fair comparison is impossible, unless one uses public code to reproduce results under exactly the same setup.

In this work, we do provide completely fair comparisons with such reproduced results of three state-of-the-art methods: LR+ICI~\cite{lrici}, PT+MAP~\cite{pt_map} and MCT~\cite{mct}. 
% To our knowledge, these methods outperform all other state of the art. 
Only~\cite{lrici} is published, while the other two are pre-prints. 
% We compare with these methods in \autoref{sec:trans} (transductive) and \autoref{sec:semi} (semi-supervised), then with other state of the art in \autoref{sec:soa}.

\paragraph{Networks}

We use publicly available pre-trained backbone convolutional neural networks that are trained on the base-class training set. We experiment with two popular networks, namely, the residual network ResNet-12~\cite{tadam} and the wide residual network WRN-28-10~\cite{LEO}.

In particular, to compare with~\cite{lrici}, we use pre-trained weights of the ResNet-12 provided by~\cite{lrici}, which we call ResNet-12A, as well as official public code\footnote{\url{https://github.com/Yikai-Wang/ICI-FSL}} for testing. To compare with~\cite{pt_map}, we use pre-trained weights of a WRN-28-10 provided by~\cite{manifoldmixup}\footnote{\url{https://github.com/nupurkmr9/S2M2_fewshot}}, which are the same used by~\cite{pt_map}, as well as official public code\footnote{\url{https://github.com/yhu01/PT-MAP}} for testing. To compare with~\cite{mct}, we use official public code\footnote{\url{https://github.com/seongmin-kye/MCT}} to train from scratch another version of ResNet-12 used by~\cite{mct}, which we call ResNet-12B, as well as the same code for testing.

\paragraph{Feature pre-processing}

Each method uses its own feature pre-processing. LR+ICI~\cite{lrici} uses $\ell_2$-normalization and PCA to reduce ResNet-12A to 5 dimensions. PR+MAP~\cite{pt_map} uses element-wise power transform, $\ell_2$-normalization and centering of WRN-28-10 features. MCT~\cite{mct} uses flattening of the output tensor of ResNet-12B rather than spatial pooling.
% , hence dimensionality is in the thousands. 
By default, we use the same choices as~\cite{pt_map,mct} for WRN-28-10 and ResNet-12B. For ResNet-12A however, we use $\ell_2$-normalization only on transductive inference and we do not use any dimensionality reduction.
% We ablate these options in \autoref{sec:trans}.

\paragraph{Implementation details}

We use PyTorch~\cite{pytorch}
% , FAISS \cite{faiss} 
and scikit-learn~\cite{sklearn}. Label cleaning is based on a linear classifier on top of $f$, initialized by imprinting the average of support features per class and then trained using~\eq{loss}. We use SGD with momentum 0.9 and weight decay 0.0005. Following~\cite{o2u}, we use a cyclical schedule of 10 cycles with 20 iterations per cycle for the learning rate, which linearly decreases from a maximum $\eta_{\max}$ to zero. For inductive (resp. semi-supervised) learning, we use logistic regression on support (resp. also pseudo-labeled) examples, learned using scikit-learn~\cite{lrici}. The row-wise sum $\vp$~\eq{sink-row} is fixed to 1. The supplementary material includes more choices.
% an ablation with weights in $[0,1]$ according to entropy, following~\cite{semilpavrithis}.

%------------------------------------------------------------------------------

\subsection{Ablation study}
\label{sec:ablation}

\paragraph{Hyperparameters}

Our hyperparameters include $\gamma$ and $k$ used in the nearest neighbor graph~\eq{affinity}, $\alpha$ in label propagation~\eq{lp}, $\tau$ in balancing~\eq{balance} and the maximum learning rate $\eta_{\max}$ of label cleaning. We optimize them on the validation set of every dataset. Common choices for $k$ and $\alpha$ are in $[15,20]$ and in $[0.5,0.8]$, respectively. We set $\gamma = 3$, $\tau = 3$ and $\eta_{\max} = 0.1$. More details and precise choices per dataset are given in the supplementary material.

\paragraph{Algorithmic components}

\autoref{tab:ab-comp} ablates the performance of our method in the presence or not of individual components, as well as using alternatives to our components. The use of queries with label propagation immediately gives a gain of transductive over inductive inference, up to 14\% in 1-shot. Balancing and iterative label cleaning each bring another gain of 4-5\%, especially in 1-shot. Iterative label cleaning is very important because selecting examples based on $P$ instead is even worse than baseline transductive inference. Label propagation is also very important because using a linear classifier instead fails too.

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{4.5pt}
\begin{tabular}{lcccccccccc}
\toprule
\Th{Method}                    & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                 \\ 
                               &              &            & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot               & 5-shot    \\ \midrule
LR+ICI~\cite{lrici}            & ResNet-12A   & 30/50      & 69.66\cip           & 80.11\cip           & 84.01\cip           & 89.00\cip           & 76.51\cip           & 84.32\cip           & 89.58\cip            & 92.48     \\
LR+ICI~\cite{lrici}*           & ResNet-12A   & 30/50      & 67.64\ci{0.95}      & 80.00\ci{0.55}      & 83.20\ci{0.89}      & 89.15\ci{0.48}      & 76.57\ci{0.96}      & 84.11\ci{0.60}      & 88.36\ci{0.71}       & -         \\
% \tb{\ours (ours)}              & ResNet-12A   & 30/50      & \tb{70.67}\ci{0.98} & \tb{81.48}\ci{0.53} & 83.49\ci{0.80}      & 88.65\ci{0.45}      & 76.46\ci{0.88}      & \tb{85.06}\ci{0.56} & \tb{89.92}\ci{0.63}  & -         \\ 
\tb{\ours (ours)}              & ResNet-12A   & 30/50      & \tb{72.36}\ci{0.93} & \tb{81.23}\ci{0.51} & \tb{84.34}\ci{0.77} & \tb{89.66}\ci{0.49} & 78.44\ci{0.89}      & \tb{85.69}\ci{0.50} & \tb{ 89.44}\ci{0.62} & -         \\ \midrule
LR+ICI~\cite{lrici}*           & WRN-28-10    & 30/50      & 81.77\ci{0.81}      & 88.53\ci{0.44}      & 87.96\ci{0.75}      & 92.11\ci{0.41}      & 86.41\ci{0.77}      & 89.90\ci{0.53}      & 91.29\ci{0.59}       & -         \\
PT+MAP~\cite{pt_map}$\dagger$  & WRN-28-10    & 30/50      & 83.47\ci{0.68}      & 89.15\ci{0.38}      & 88.67\ci{0.68}      & 92.44\ci{0.38}      & 87.71\ci{0.67}      & 90.38\ci{0.45}      & 92.05\ci{0.52}       & -         \\
\tb{\ours (ours)}              & WRN-28-10    & 30/50      & \tb{84.00}\ci{0.74} & \tb{89.68}\ci{0.37} & \tb{88.87}\ci{0.73} & \tb{92.66}\ci{0.40} & \tb{87.78}\ci{0.69} & \tb{90.58}\ci{0.50} & \tb{92.35}\ci{0.52}  & -         \\
\bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised few-shot learning, comparison with LR+ICI~\cite{lrici} and PT+MAP~\cite{pt_map}. *: our reproduction with official code on our datasets. $\dagger$: our adaptation to semi-supervised, based on official code. CUB 5-shot omitted: no class has the required 70 examples.}
\label{tab:semi_pre}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{lccccccccc}
\toprule
\Th{Method}                             & \Th{Network} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}}        & \mc{2}{\Th{Cifar-FS}}                     & \mc{2}{\Th{CUB}}                          \\ 
                                        &              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
% LR+ICI~\cite{lrici}                     & ResNet-12A   & 66.80\cip           & 79.26\cip           & 80.79\cip           & 87.92\cip           & 73.97\cip           & 84.13\cip           & 88.06\cip           & 92.53\cip           \\
LR+ICI~\cite{lrici}*                    & ResNet-12A   & 66.85\ci{0.92}      & 78.89\ci{0.55}      & 82.40\ci{0.84}      & 88.80\ci{0.50}      & 75.36\ci{0.97}      & 84.57\ci{0.57}      & 86.53\ci{0.79}      & 92.11\ci{0.35}      \\
CAN+Top-\emph{k}~\cite{crossattention}  & ResNet-12    & 67.19\ci{0.55}      & 80.64\ci{0.35}      & 73.21\ci{0.58}      & 84.93 \ci{0.38}     & -                   & -                   & -                   & -                   \\
DPGN~\cite{DPGN}                        & ResNet-12    & 67.77\ci{0.32}      & 84.60\ci{0.43}      & 72.45\ci{0.51}      & 87.24\ci{0.39}      & 77.90\ci{0.50}      & 90.20\ci{0.40}      & 75.71\ci{0.47}      & 91.48\ci{0.33}      \\
% EP~\cite{embeddingpropagation}          & ResNet-12    & 66.50\ci{0.89}      & 81.06\ci{0.60}      & 76.53\ci{0.87}      & 87.32\ci{0.64}      & -                   & -                   & -                   & -                   \\
MCT (instance)~\cite{mct}               & ResNet-12B   & 78.55\ci{0.86}      & 86.03\ci{0.42}      & 82.32\ci{0.81}      & 87.36\ci{0.50}      & 85.61\ci{0.69}      & 90.03\ci{0.46}      & -                   & -                   \\
% MCT (Pair)~\cite{mct}                   & ResNet-12B   & 76.16\ci{0.89}      & 85.22\ci{0.42}      & 80.68\ci{0.89}      & 86.63\ci{0.89}      & 87.28\ci{0.70}      & 90.50\ci{0.43}      & -                   & -                   \\
% \tb{\ours (ours)}                       & ResNet-12A   & \tb{69.79}\ci{0.99} &\tb{79.58}\ci{0.55}  & \tb{83.49}\ci{0.88} &\tb{89.48}\ci{0.47}  & \tb{77.14}\ci{0.95} & \tb{85.23}\ci{0.55} & \tb{88.75}\ci{0.68} & \tb{92.74}\ci{0.35} \\
\midrule
% PT+MAP~\cite{pt_map}                    & WRN-28-10    & 82.92\ci{0.26}      & 88.82\ci{0.13}      & -                   & -                   & 87.69\ci{0.23}      & 90.68\ci{0.15}      & 91.55\ci{0.19}      & 93.99\ci{0.10}      \\
PT+MAP~\cite{pt_map}*                   & WRN-28-10    & 82.88\ci{0.73}      & 88.78\ci{0.40}      & 88.15\ci{0.71}      & 92.32\ci{0.40}      & 86.91\ci{0.72}      & 90.50\ci{0.49}      & 91.37\ci{0.61}      & 93.93\ci{0.32}      \\
Fine-tuning~\cite{baseline_ft}          & WRN-28-10    & 65.73\ci{0.68}      & 78.40\ci{0.52}      & 73.34\ci{0.71}      & 85.50\ci{0.50}      & 76.58\ci{0.68}      & 85.79\ci{0.50}      & -                   & -                   \\
EP~\cite{embeddingpropagation}          & WRN-28-10    & 70.74\ci{0.85}      & 84.34\ci{0.53}      & 78.50\ci{0.91}      & 88.36\ci{0.57}      & -                   & -                   & -                   & -                   \\
SIB~\cite{SIB}$\dagger$                 & WRN-28-10    & 70.00\ci{0.60}      & 79.20\ci{0.40}      & 72.90\cip           & 82.80\cip           & 80.00\ci{0.60}      & 85.3\ci{0.40}       & -                   & -                   \\
% DPGN~\cite{DPGN}                        & WRN-28-10    & 67.24\ci{0.51}      & 83.72\ci{0.44}      & -                   & -                   & -                   & -                   & -                   & -                   \\
SIB+E$^3$BM~\cite{ensemblefsl}          & WRN-28-10    & 71.40\ci{0.50}      & 81.20\ci{0.40}      & 75.60\ci{0.60}       & 84.30\ci{0.40}       & -                   & -                   & -                   & -                   \\
\tb{\ours (ours)}                       & WRN-28-10    & \tb{83.43}\ci{0.79} & \tb{89.10}\ci{0.42} & \tb{88.50}\ci{0.77} & \tb{92.99}\ci{0.42} & \tb{87.57}\ci{0.78} & \tb{91.26}\ci{0.46} & \tb{91.53}\ci{0.59} & \tb{94.27}\ci{0.30} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Transductive inference state of the art. *: our reproduction with official code on our datasets. $\dagger$: \emph{tiered}ImageNet as reported by~\cite{ensemblefsl}.}
\label{tab:soa-trans}
\end{table*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\setlength\tabcolsep{2pt}
\begin{tabular}{lcccccc}
\toprule
\Th{Method}                                        & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}          \\ 
                                                   &              &            & 1-shot              & 5-shot              \\ \midrule
% TPN$_{SSL}$\cite{tpn}                              & CONV-4       & 20/20      & 52.78               & 66.42               \\
% $k$-means~\cite{ssmeta}                            & CONV-4       & 20/20      & 50.41               & 64.39               \\
% \tb{\ours (ours)}                                  & CONV-4       & 20/20      &                     &                     \\ \midrule
LST~\cite{learning2selftrain}                      & ResNet-12    & 30/50      & 70.10\ci{1.90}      & 78.70\ci{0.80}      \\
LR+ICI~\cite{lrici}                                & ResNet-12A   & 30/50      & 69.66\cip           & 80.11\cip           \\
MCT (instance)~\cite{mct}                          & ResNet-12B   & 30/50      & 73.80\ci{0.70}      & 84.40\ci{0.50}      \\
% \tb{\ours (ours)}                                  & ResNet-12A   & 30/50      &                     &                     \\ 
\midrule                                                                                            
% LR+ICI~\cite{lrici}                                & ResNet-12A   & 80/80      & 71.41               & 81.12               \\
% \tb{\ours (ours)}                                  & ResNet-12A   & 80/80      &                     &                     \\ \midrule
$k$-means~\cite{ssmeta}$\dagger$                   & WRN-28-10    & 100/100    & 52.35\ci{0.89}      & 67.67\ci{0.65}      \\
TransMatch~\cite{transmatch}                       & WRN-28-10    & 100/100    & 63.02\ci{1.07}      & 81.06\ci{0.59}      \\
\tb{\ours (ours)}                                  & WRN-28-10    & 100/100    & \tb{87.62}\ci{0.67}      & \tb{90.51}\ci{0.36} \\ \bottomrule
\end{tabular}
\vspace{6pt}
\caption{Semi-supervised few-shot learning state of the art. $\dagger$: as reported by~\cite{transmatch}}
\label{tab:soa-semi}
\end{table}
%------------------------------------------------------------------------------

% %------------------------------------------------------------------------------
% \begin{table*}
% \small
% \centering
% \begin{tabular}{lcccccc}
% \toprule
% \Th{Method}                                        & \Th{Network} & \Th{Split} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{\emph{tiered}ImageNet}} \\ 
%                                                    &              &            & 1-shot              & 5-shot              & 1-shot         & 5-shot            \\ \midrule
% % TPN$_{SSL}$\cite{tpn}                              & CONV-4       & 20/20      & 52.78               & 66.42               & 55.74          & 71.01             \\
% % $k$-means$_{\masked,\soft}$~\cite{ssmeta}          & CONV-4       & 20/20      & 50.41               & 64.39               & -              & -                 \\
% % \tb{\ours (ours)}                                  & CONV-4       & 20/20      &                     &                     &                &                   \\ \midrule
% LST~\cite{learning2selftrain}                      & ResNet-12    & 30/50      & 70.10\ci{1.90}      & 78.70\ci{0.80}      & 77.70\ci{1.60} & 85.20\ci{0.80}    \\
% LR+ICI~\cite{lrici}                                & ResNet-12A   & 30/50      & 69.66\cip           & 80.11\cip           & 84.01\cip      & 89.00\cip         \\
% MCT (instance)~\cite{mct}                          & ResNet-12B   & 30/50      & 73.80\ci{0.70}      & 84.40\ci{0.50}      & 76.90\ci{0.70} & 86.30\ci{0.50}    \\
% % \tb{\ours (ours)}                                  & ResNet-12A   & 30/50      &                     &                     &                &                   \\ 
% \midrule                                                                                            
% % LR+ICI~\cite{lrici}                                & ResNet-12A   & 80/80      & 71.41               & 81.12               & 85.44          & 89.12             \\
% % \tb{\ours (ours)}                                  & ResNet-12A   & 80/80      &                     &                     &                &                   \\ \midrule
% $k$-means$_{\masked,\soft}$~\cite{ssmeta}$\dagger$ & WRN-28-10    & 100/100    & 52.35\ci{0.89}      & 67.67\ci{0.65}      & -              & -                 \\
% TransMatch~\cite{transmatch}                       & WRN-28-10    & 100/100    & 63.02\ci{1.07}      & 81.06\ci{0.59}      & -              & -                 \\
% \tb{\ours (ours)}                                  & WRN-28-10    & 100/100    & \tb{83.98}\ci{0.78} & \tb{87.73}\ci{0.37} &                &                   \\ \bottomrule
% \end{tabular}
% \vspace{6pt}
% \caption{Semi-supervised few-shot learning state of the art. $\dagger$: as reported by~\cite{transmatch}}
% \label{tab:soa-semi}
% \end{table*}
% %------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Label cleaning: loss distribution}
\label{sec:hist}

To illustrate our label cleaning, we conduct two experiments, showing the distribution of the loss value~\eq{loss}. In the first, shown in \autoref{fig:hist}(a,b), we inject label noise uniformly at random to the 20\%~(a) and 40\%~(b) of 500 labeled examples. The correctly and incorrectly labeled examples have very different loss distributions. Importantly, while previous work on noisy labels~\cite{ArazoOAOM19,o2u,robustonfly} attempts to detect clean examples by an optimal threshold on the loss value, we only need few clean examples per iteration. Examples with minimal loss value are clean.

The second experiment is on two novel 1-shot transductive tasks, shown in \autoref{fig:hist}(c,d). We use 50 unlabeled queries per class and we predict pseudo-labels according to~\eq{argmax}. Label cleaning is more challenging here because the two distributions are more overlapping. This is natural because predictions are more informed than uniform, even if incorrect. Still, a large proportion of clean examples have less loss than the minimal value of noisy ones.

%------------------------------------------------------------------------------

\subsection{Transductive inference}
\label{sec:trans}

\autoref{tab:trans-pre} compares our \ours with LR+ICI~\cite{lrici} and PT+MAP~\cite{pt_map}.
% on all four datasets. 
The truly fair comparison is with our reproductions, indicated by *. Apart from the default networks, we also use WRN-28-10 with LR+ICI~\cite{lrici}, since it is more powerful. Our \ours is superior or on par with competitors. The gain over~\cite{lrici} up to 3\% on \emph{mini}ImageNet 1-shot. The gain over PT+MAP~\cite{pt_map} is around 0.5\%. 

% Because the gain over~\cite{pt_map} is small, we 
We also experiment with 50 unlabeled queries per class, or $M=250$ in total. As shown in \autoref{tab:trans-50q}, the gain increases up to 3\% on \emph{mini}ImageNet 1-shot. This can be attributed to the fact that PT+MAP~\cite{pt_map} operates on Euclidean space, while we capture the manifold structure, which manifests itself in the presence of more data. An 10-shot experiment is also included in the supplementary material. 

\autoref{tab:ab-pt} shows that PT+MAP~\cite{pt_map} is very sensitive to feature pre-processing, losing up to 40\% without it, while our \ours more robust, losing only up to 5\%. Similarly, \autoref{fig:pca} shows that LR+ICI~\cite{lrici} is sensitive to dimension reduction, working best at only 5 dimensions. By contrast, our \ours is very stable and only fails at 2 dimensions.

\alert{\autoref{tab:trans-mct} compares our \ours with MCT~\cite{mct}. In order to have more fair comparisons between state-of-the-art methods and their pre-trained backbones, we trained from scratch the resNet-12 used in ~\cite{mct} using the meta-learning training procedure that \cite{mct} uses. We compare ~\cite{mct} and our method without using any model data augmentations such as flipping the images as is used in the ~\cite{mct} works so that the performance of each method can be solely attributed on the merits of each method. Also we do not use the meta-learnt scaled function that is used in ~\cite{mct} since our aim was to investigate whether our method and ~\cite{mct} are comparable using solely the same backbone. Since our method is solely based on the testing procedure of the transductive few-shot setting, it would be unfair to compare our method and ~\cite{mct} using the scaled function that was learnt during training, therefore we test the performance merits of each method assuming access to only the pre-trained backbone that is pre-trained using meta-learning.}

%------------------------------------------------------------------------------

\subsection{Semi-supervised learning}
\label{sec:semi}

As shown in \autoref{tab:semi_pre}, \ours is superior to LR+ICI~\cite{lrici} in all settings by an even larger margin than in transductive inference, \eg by nearly 5\% in \emph{mini}ImageNet 1-shot. This can be be attributed to capturing the manifold structure of the data, since there is more unlabeled data in this case. Because PT+MAP~\cite{pt_map} does not experiment with semi-supervised learning, we adapt it in the same way as ours, using the default WRN-28-10, again outperforming it.

%------------------------------------------------------------------------------

\subsection{Comparison with the state of the art}
\label{sec:soa}

\autoref{tab:soa-trans} and \autoref{tab:soa-semi} compare our \ours with a larger collection of recent methods on the tranductive and semi-supervised settings, respectively. Even when the network and data split appears to be the same, we acknowledge that our results are not directly comparable with any method other than our reproductions. As discussed in the supplementary material, this is due to the very diverse choices made in the bibliography, \eg versions of network, training settings, versions of datasets, or pre-processing. For instance, ResNet-12 is different than either ResNet-12A or ResNet-12B.

For this reason, we focus on the best result by each method, including ours. Necessarily, methods experimenting with WRN-28-10 have an advantage. Still, at least among those, \ours performs best by a large margin in both settings, with the closest second best being PT+MAP~\cite{pt_map}.




==> tex/plots-none.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/plots.tex <==
%------------------------------------------------------------------------------
% hack for CVPR style
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,shapes,calc,matrix,fit,positioning,backgrounds,decorations.markings}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.9}
\usepackage{xstring}

%------------------------------------------------------------------------------
% externalization: requires defining \finalcopy first

\usepgfplotslibrary{external}
% \tikzexternalize[prefix=fig/extern/]
\newcommand{\extfig}[2]{\tikzsetnextfilename{#1}{#2}}
\newcommand{\noextfig}[1]{\tikzset{external/export next={false}}{#1}}
\newcommand{\extdata}[1]{\input{#1}}
\IfBeginWith*{\jobname}{fig/extern/}{\finalcopy}{}

%-----------------------------------------------------------------------------
% tikz styles

\tikzstyle{every picture}+=[
	remember picture,
	every text node part/.style={align=center},
	every matrix/.append style={ampersand replacement=\&},
]
\tikzstyle{tight} = [inner sep=0pt,outer sep=0pt]
\tikzstyle{node}  = [draw,circle,tight,minimum size=12pt,anchor=center]
\tikzstyle{op}    = [draw,circle,tight]
\tikzstyle{dot}   = [fill,draw,circle,inner sep=1pt,outer sep=0]
\tikzstyle{pt}    = [fill,draw,circle,inner sep=1.5pt,outer sep=.2pt]
\tikzstyle{box}   = [draw,thick,rectangle,inner sep=3pt]
\tikzstyle{high}  = [black!60]
\tikzstyle{group} = [high,box,opacity=.5]
\tikzstyle{rectc} = [tight,transform shape]
\tikzstyle{rect}  = [rectc,anchor=south west]

%-----------------------------------------------------------------------------
% framed figures

\newcommand{\framed}[3][1]{\extfig{#2}{\tikz{
	\node[tight](a){\fig[#1]{#3}};
	\node[tight,draw=gray,fit=(a)]{};
}}}

%-----------------------------------------------------------------------------
% pgfplots general options

\newcommand{\leg}[1]{\addlegendentry{#1}}

\tikzset{every mark/.append style={solid}}
\pgfplotsset{%smooth,
	grid=both, width=\columnwidth, try min ticks=5,
	every axis/.append style={font=\small},
	every axis plot/.append style={thick,mark=none,mark size=1.8,tension=0.18},
	legend cell align=left, legend style={fill opacity=0.8},
	xticklabel={\pgfmathprintnumber[assume math mode=true]{\tick}},
	yticklabel={\pgfmathprintnumber[assume math mode=true]{\tick}},
	nodes near coords math/.style={
		nodes near coords={\pgfmathprintnumber[assume math mode=true]{\pgfplotspointmeta}},
	},
}

\pgfplotsset{
	dash/.style={mark=o,dashed,opacity=0.6},
	dott/.style={mark=o,dotted,opacity=0.6},
	nolim/.style={enlargelimits=false},
	plain/.style={every axis plot/.append style={},nolim,grid=none},
}
\newcommand{\kilo}[1]{\thisrow{#1}/1000}



==> tex/related-1.tex <==
\section{Related work}
\label{sec:related}
In this section we will describe the main lines of research that attempted to tackle the few-shot learning challenge. Then we will focus in the transductive and semi-supervised few-shot learning methodologies that leverage the use of unlabelled data which is more related to our work.
\subsection{Few-shot learning}
One of the main lines of research tackling the few-shot learning challenge is the approach of meta-learning \cite{MAML, siamese, prototypical, SNAIL, matchingNets}. This approach generally partitions the dataset into multiple different so-called episodes with a few labelled examples, the support set $S$, of $K$ examples from $N$ different classes while the rest of the examples being unlabelled, the query set $Q$. The purpose of meta-learning is to learn a model such that when a novel task sampled from unseen classes is presented to the model, the model can adapt and make accurate predictions. Typically meta-learning methods can be classified into gradient-based methods, model-based methods and metric-based methods. Gradient-based methods \cite{MAML, iMAML, CAVIA, ravilstm, reptile, metaoptnet, bertinetto} attempt to learn model parameters that are capable to adapt fast in novel tasks. Metric-based methods \cite{prototypical, siamese, relationnet, matchingNets} attempt to learn a good vector representation where similarity comparison between different samples can be done. Model-based methods \cite{SNAIL, santoro, metaNet} rely on the properties of specific model architectures, such as Recurrent Neural Networks, LSTMs and memory augmented neural network to aid learning from few samples.
\\
\\
Besides meta-learning methodologies other methods that tackle the few-shot learning challenge include predicting classifier weights \cite{gidarisFSL, imprintedweights, activationweights}. In \cite{gidarisFSL} a few-shot classification weight generator was designed that is fed examples of a novel category along with already pre-trained weightvectors and generates a representative weight vector for the novel class. In \cite{imprintedweights} the idea is to leverage the novel examples of each class by using their average vector as the classifier weights for every class. Another line of research revolves around hallucination based approaches \cite{lowshot, lowshot2, dataAG}. These methods attempt to learn how to generate new training data, hallucinate, and use the data for improving the few-shot training regime.\\
\\
In recent years the most commonly used line of research addressing the few-shot learning challenge is the transfer based approaches \cite{rfs, manifoldmixup, closerlook}. In contrast to meta-learning methodologies, transfer learning methods focus on pre-training a feature extractor on the whole dataset rather than sampling few-shot training episodes. In \cite{manifoldmixup} it has been shown that self-supervised and regularization techniques can be used to learn robust feature representations and surpass the performance of meta-learning methods. In a similar note \cite{rfs} showed that training with knowledge distillation can boost the performance of few-shot learning by learning more representative features. In \cite{closerlook} the authors showed that transfer learning methods that learn a representative feature embedding can be as accurate as meta-learning methods.
\subsection{Transductive and Semi-supervised Few-shot Learning} Leveraging the use of unlabelled data along with labelled data has been of interest in many practical applications due to the ease and efficiency of obtaining unlabelled data. A common line of research that leverages the use of unlabelled data in the few-shot setting is the transductive few-shot learning \cite{tpn, tafssl, transductiveEA, exploitingUI, pt_map, embeddingpropagation}. In this setting the assumption is that all the query samples are available for prediction at inference time and they can be used as a source of unlabelled data to improve the performance of the few-shot learning algorithm. In \cite{embeddingpropagation}, embedding propagation is used and applied on the support and query samples to improve the feature embedding of all samples. In \cite{tpn}, rather than using heuristic label-propagation methods, the authors propose to learn to propagate labels for samples of novel classes. In \cite{tafssl}, a task-specific feature sub-space that is highly discriminant for different tasks is identified through the use of dimensionality reduction techniques. In \cite{crossattention}, the authors propose a cross attention module that generates cross attention maps for each pair of class features and query sample features, highlighting the target object region in the process. In this work the authors also leverage the available query samples by iteratively classifying the queries and choosing the top $k$ queries at every iteration to re-calculate the class feature map before re-classifying the queries.\\
\\
In the semi-supervised few-shot learning, access to an extra unlabelled set besides the query sample is assumed that can be used for training purposes \cite{ssmeta, lrici, transmatch}. The samples from the unlabelled set can be the same as the support set or they can include examples from distractor classes as well. One of the first works to use this setting was \cite{ssmeta}, in which they proposed the use the unlabelled examples in order to improve the prototypical networks \cite{prototypical} algorithm by fining more representative class prototypes while at the same time identifying whether a sample belongs to a "distractor" class. Another work that attempts to tackle the semi-supervised few-shot learning problem is \cite{transmatch}, where the authors proposed to adapt the well known semi-supervised method MixMatch \cite{mixmatch} to the semi-supervised Few-shot learning setting. In \cite{learning2selftrain}, the authors proposed to learn how to self-train by first predicting the pseudolabels of the unlabelled data and then learn how to cherry pick the best pseudolabels to re-train the model and improve its performance. \cite{lrici} proposed to predict pseudolabels using a linear layer and then apply a so called instance credibility inference module that provides a score for the credibility of each pseudolabel. Based on that score the best pseudolabels are used to augment the support set and repeat the same procedure until all the unlabelled samples are added to the support set. In \cite{adaptivesubspace}, the authors leverage the unlabelled data to learn a feature extractor that genereates class specific subspaces. A class specific projection matrix is defined from the support and unlabelled data and the classification of the query is based on the shortest distance between the query and to its projection its projection to a class specific subspace.
